Design of secure and robust cognitive system for malware detection

Machine learning based malware detection techniques rely on grayscale images of malware and tends to classify malware based on the distribution of textures in graycale images. Albeit the advancement and promising results shown by machine learning techniques, attackers can exploit the vulnerabilities by generating adversarial samples. Adversarial samples are generated by intelligently crafting and adding perturbations to the input samples. There exists majority of the software based adversarial attacks and defenses. To defend against the adversaries, the existing malware detection based on machine learning and grayscale images needs a preprocessing for the adversarial data. This can cause an additional overhead and can prolong the real-time malware detection. So, as an alternative to this, we explore RRAM (Resistive Random Access Memory) based defense against adversaries. Therefore, the aim of this thesis is to address the above mentioned critical system security issues. The above mentioned challenges are addressed by demonstrating proposed techniques to design a secure and robust cognitive system. First, a novel technique to detect stealthy malware is proposed. The technique uses malware binary images and then extract different features from the same and then employ different ML-classifiers on the dataset thus obtained. Results demonstrate that this technique is successful in differentiating classes of malware based on the features extracted. Secondly, I demonstrate the effects of adversarial attacks on a reconfigurable RRAM-neuromorphic architecture with different learning algorithms and device characteristics. I also propose an integrated solution for mitigating the effects of the adversarial attack using the reconfigurable RRAM architecture.

==> ChapterFour.tex <==
\chapter[Survey Paper]{Survey of ML-based Techniques and Hardware Implementations}
\paragraph*{Abstract}
Advancements in technology and smart devices demand incubation of advanced learning methodologies to learn or capture the underlying patterns in the data and further utilize and analyze the extracted patterns for different purposes such as anomaly detection, face recognition, and data prediction.
There are many techniques for learning and analyzing data patterns, each of which has different complexity and performance. Two important kinds of data analyzed in the current day technology are the time-series signals and the images (computer vision). In this work,
we outline diverse machine learning techniques and 
their applicability for pattern analysis in the aforementioned kind of applications.
This survey is motivated by the increasing need to analyze time-series signals and image processing 
in resource-constrained, embedded devices for a large variety of applications, including autonomous driving.
First, we provide a comprehensive review of techniques for analyzing the signals based on numerous stochastic, traditional machine learning, deep neural networks, and other hybrid approaches. For all the prominent families of techniques,  
we discuss their use in prediction, anomaly detection, and classification. 
Moreover, we consider their algorithmic complexity and review their 
hardware implementations. 
Further, we compare and analyze the involved trade-offs among 
different techniques (including hardware requirements), and its suitability for analyzing various data sets such as image classification, recognition, and time-series analysis.

\section{Introduction} \label{sec:intro}
Data analysis is a challenge faced by modern computing systems with the amounts of data collected by embedded electronic devices reaching the Exa-scale. Time-series 
data is one of the main categories of data captured by the current devices for many purposes. 

Time-series is an ordered sequence of values of the variable(s) 
monitored or measured at regular time intervals. 
Time-series signals are widely employed for various purposes. 
Processing and analysis of time-series signals are of 
equal importance in simple and portable electronic devices as well as in  
large data centers, and are employed for various applications 
ranging from simple forecasting to complex operations. Time-series analysis 
is applied for anomaly detection \cite{Strauss'01,Mohamad'13}, prediction \cite{Kong'04,Dalvi'16,Yu'15}, 
and classification~\cite{Prathibhamol'16,Ye'12}, and also in different purposes 
such as Quality-of-Service (QoS) management \cite{SMPD_DAC'13,SMPD_ICCAD'14, SMPD_TC'15}, and security in embedded systems \cite{ Shukla_1, Shukla_2, Shukla_3, Abhijitt_1}. 
Time-series analysis involves challenges such as the need for real-time processing, low complexity, and high-accuracy, depending on the data size, performance requirements, 
and the complexity of the application.   

As the data analysis can incur large amounts of data, and 
repetitive operations, automating the data analysis is needed to  
enhance the efficiency of processing. 
There exists a large and diverse body of 
techniques ranging from statistical methods to deep learning 
that has been used for 
pattern recognition, signal analysis, and anomaly detection in time-series signals.

% There exists numerous techniques to perform this automated 
% data analysis ranging from stochastic techniques 
% to complex machine learning techniques. 
%Signal analysis or data analysis can be automated to make the analysis  more efficient and faster with the aid of machine learning techniques. 
% Machine learning is about making the computing systems modify or adapt their actions  based on their experience or 
% training, so that the operation becomes more accurate, where the accuracy is measured in comparison to ideally correct actions~\cite{Marsland'09}. 
% Machine learning could be classified broadly into four categories: supervised, unsupervised, 
% reinforcement and evolutionary learning. For supervised learning, the system 
% is provided with data and the correct responses. For unsupervised learning, the system is provided 
% with data, but does not know what is the correct response. It explores similarities in inputs, classifies the input data patterns, and detects changes and anomalies. 
% Reinforcement learning is a combination of supervised and unsupervised learning. The system is provided with feedback when its output is incorrect, but it is not provided with 
% clues how to correct it and what is the correct output. Evolutionary learning is similar to biological 
% learning, where the organisms adapt to improve their survival rates. 

% Furthermore, there exists a large and diverse body of 
% techniques ranging from statistical methods to deep learning 
% that has been used for 
% pattern recognition, signal analysis, and anomaly detection in time-series signals.
%The most widely used learning technique is supervised learning. 
%Neural networks \cite{Lipmann'87} are 
%inspired by the mammalian brain architecture from the brain-based implementation strategy. 
%
%There exists a large number of methods that are developed for time-series analysis.
However, each of these techniques has its pros and cons. 
Despite numerous works on data analysis, 
there has been no methodology or hard-coded rule that facilitates selecting an optimal analysis technique for a given application and data inputs; this is a significant challenge for devising/choosing data analysis techniques. Furthermore, with miniature computing systems' proliferation, some data analysis designs are moving towards resource-efficient hardware. This process adds one more level of complexity in choosing the appropriate data analysis technique, from the processing perspective and the hardware implementation costs and overheads. 
We first present different data analysis methods ranging from statistical methods to highly sophisticated machine learning methods in this work. This is followed by a review of existing hardware implementations available on different platforms such as FPGAs, ASICs, and GPUs. Lastly, an analysis of the complexity and suitability of other techniques to hardware, application
requirements, and performance is proposed. 
%To the best of our knowledge, this is the first work that 
This work presents a wide spectrum of data analysis techniques, discusses the 
hardware implementations analyze their complexity and provide 
valuable insights. 
This work focuses on time-series analysis for embedded systems broadly, and any other techniques described are to make it comprehensive.

%  on time-series analysis. 
%not only considering the performance, but also the computational complexity and hardware implementations relevant to the application to be processed. 
% A traditional neural network comprises of three layers: input layer, hidden layer, 
% and output layer. 
% %Multiple number of hidden layers could be 
% %possible in deep learning, depending on the necessity and design. 
% Each layer is 
% built with nodes. Each node has inputs, outputs and 
% performs one operation based on its activation function, e.g. a threshold function. Inputs are  given weights to signify their relative importance. Learning in 
% neural networks could be seen as adaptation of weights between layers and 
% updating of activation functions. Many different variants 
% of neural networks have been studied in the literature, a few of which will be investigated along with some other lightweight techniques for signal analysis in this project. 
% Analysis of different techniques will be presented along with a 
% road-map that leads to efficient utilization of machine learning 
% techniques with features of lightweight, low resource utilization, 
% accurate and fast.

% The rest of the paper is organized as follows. 
% Different techniques 
% that are employed for time-series analysis ranging from 
% statistical metrics based methods to deep learning approaches 
% are presented
% in Section \ref{sec:tech_tsa}. %, and how they are applied in 
% %the context of signal analysis and different variants of 
% %techniques are presented in Section \ref{sec:use_tech}. 
% Hardware implementations of different time-series analysis 
% techniques are presented in Section \ref{sec:hw_impl} 
% with complexity analysis discussion in 
% Section \ref{sec:cmplx}. Based on the complexity analysis 
% and existing 
% hardware implementations, analysis on suitability of 
% different time-series analysis techniques to different 
% application is derived in Section \ref{sec:analysis}. 
% Lastly, the conclusions of this study are drawn in Section \ref{sec:conc}.








%\section{Introduction}
%\label{sec:intro}
%Time-series is an ordered sequence of values of variable(s) 
%monitored or measured at regular time intervals. 
%Time-series signals are widely employed in our society. 
%Processing and analysis of time-series signals is of 
%equal importance in simple, portable electronic devices as well as in  
%large data centers, and is employed for various applications 
%ranging from simple forecasting to complex operations. Time-series analysis 
%is applied for anomaly detection \cite{Strauss'01,Mohamad'13}, prediction \cite{Kong'04,Dalvi'16,Yu'15}, 
%and classification~\cite{Prathibhamol'16,Ye'12}. 
%Time-series analysis involves challenges such as need for real-time processing, low complexity, and high-accuracy, depending on the data size, performance requirements, 
%and the complexity of the application.   
%
%Signal analysis or data analysis can be automated to make the analysis 
%more efficient and faster with the aid of machine learning techniques. 
%Machine learning is about making the computers or systems modify or adapt their  
%actions  based on their experience or 
%training, so that the operation becomes more accurate, where the accuracy is 
%measured in comparison to ideally correct actions~\cite{Marsland'09}. 
%% Machine learning could be classified broadly into four categories: supervised, unsupervised, 
%% reinforcement and evolutionary learning. For supervised learning, the system 
%% is provided with data and the correct responses. For unsupervised learning, the system is provided 
%% with data, but does not know what is the correct response. It explores similarities in inputs, classifies the input data patterns, and detects changes and anomalies. 
%% Reinforcement learning is a combination of supervised and unsupervised learning. The system is provided with feedback when its output is incorrect, but it is not provided with 
%% clues how to correct it and what is the correct output. Evolutionary learning is similar to biological 
%% learning, where the organisms adapt to improve their survival rates. 
%
%There exists a large and diverse body of techniques ranging from statistical methods to deep learning 
%that has been used for 
%pattern recognition, signal analysis and anomaly detection in time series signals.
%%The most widely used learning technique is supervised learning. 
%%Neural networks \cite{Lipmann'87} are 
%%inspired by the mammalian brain architecture from the brain-based implementation strategy. 
%%
%%There exists a large number of methods that are developed for time-series analysis.
%However, each of the techniques 
%have their own pros and cons. 
%Despite the existence of numerous works on time-series analysis, 
%there exists no methodology or hard-coded rules that facilitates to 
%select an optimal analysis technique for a given application and data inputs. This is one of the basic challenges for devising/choosing
%time-series analysis techniques. Furthermore, 
%with the proliferation of miniature 
%computing systems, the focus in some of the time-series analysis 
%designs moving towards hardware efficiency. This adds one more level 
%of complexity in choosing the appropriate time-series analysis technique, 
%not only from processing perspective, but also from hardware implementation 
%costs and overheads. 
%As such, in this work we first present different existing time-series analysis methods ranging from statistical methods to machine learning methods. This is followed by existing hardware 
%implementations available on different platforms such as FPGAs, ASICs, and GPUs. An analysis on complexity, and suitability of 
%different techniques to hardware, application requirements, and 
%performance is finally analyzed. 
%
%
%
%
%To the best of our knowledge, this is the first work that 
%presents a wide spectrum of time-series analysis, discusses the 
%hardware implementations, analyzes the complexity, and provide 
%insights on time-series analysis not only considering performance, but also the computational complexity, hardware implementations, 
%relevance to the application. 
%% A traditional neural network comprises of three layers: input layer, hidden layer, 
%% and output layer. 
%% %Multiple number of hidden layers could be 
%% %possible in deep learning, depending on the necessity and design. 
%% Each layer is 
%% built with nodes. Each node has inputs, outputs and 
%% performs one operation based on its activation function, e.g. a threshold function. Inputs are  given weights to signify their relative importance. Learning in 
%% neural networks could be seen as adaptation of weights between layers and 
%% updating of activation functions. Many different variants 
%% of neural networks have been studied in the literature, a few of which will be investigated along with some other lightweight techniques for signal analysis in this project. 
%% Analysis of different techniques will be presented along with a 
%% road-map that leads to efficient utilization of machine learning 
%% techniques with features of lightweight, low resource utilization, 
%% accurate and fast.
%
%The rest of the paper is organized as follows. 
%Different techniques 
%that are employed for time-series analysis ranging from 
%statistical metrics based methods to deep learning approaches 
%are presented
%in Section \ref{sec:tech_tsa}. %, and how they are applied in 
%%the context of signal analysis and different variants of 
%%techniques are presented in Section \ref{sec:use_tech}. 
%Hardware implementations of different time-series analysis 
%techniques are presented in Section \ref{sec:hw_impl} 
%with complexity analysis discussion in 
%Section \ref{sec:cmplx}. Based on the complexity analysis 
%and existing 
%hardware implementations, analysis on suitability of 
%different time-series analysis techniques to different 
%application is derived in Section \ref{sec:analysis}. 
%The conclusions are drawn in Section \ref{sec:conc}

% \textcolor{red}{Revise whole paper to make sure the message is clear that we are talking about time-series signals and not image processing. You can mention this survey is specific to time-series analysis on embedded systems, not generic analysis. Also, feel free to cut section 2 further to fit into 8 pages. Do a grammarly check. Tomorrow night 11:59ET is deadline for final version. Send me a version by 6pm.
% \textcolor{red}{Also, cite my CSUR paper and may be another 2-3 relevant ones. You can remove some others' references to save space.}

%\vspace{-0.5em}
\section{Techniques for Time-series Analysis}
\label{sec:tech_tsa}
%\vspace{-0.5em}
Time-series can be analyzed either in time-domain or frequency-domain. When analyzing the series in time-domain, 
characteristics of the signal, such as periodicity, variance, amplitude, and other raw information, are utilized.  
Similarly, time-series can be analyzed in the frequency domain. The series is converted into a frequency-domain signal, and the respective characteristics such as energy and power spectrum density (PSD) must be taken into account for evaluation.  
As such, we discuss some of the widely used techniques for analyzing 
time-series signals with the aid of extracted characteristics below. 


\subsection{Time-Series Analysis using Statistical Metrics} \label{subs:con_met}
The time-series characteristics refer to time-series' inherent properties such as periodicity, amplitude, variance, etc.
Statistical metrics derived or signal characteristics 
such as variance, mean, median, and mode can be employed further to perform the time-series analysis. 
% As mentioned earlier, these statistical metrics can be applied on both time-domain or frequency-domain characteristics of the signal for analysis. 
%extracted from
%the raw signal or by converting the signal into frequency domain and further
%derive these metrics to analyze the signal. 
We include several commonly used %important
statistical metrics based on the signal characteristics employed for 
time-series analysis here  \cite{Guidelines'96, SMPD_CSUR}.
% It needs to be note that the metrics defined below are widely used in a vast number of applications. 
% \textcolor{red}{even in this section, the metrics (e.g., mean, variance, autocorrelation, power spectral density etc) are rather trivial and generic.}


% \textcolor{red}{In the interest of space, I recommend commenting out tables 1 and 2. Also, see if you can fit table 9 into 1 column. }

\subsubsection{Time-Domain Characteristics}% Based Analysis}
\label{subsubs:tdm} 
Time-domain characteristics-based analysis refers to employing the derived statistical metrics on the time-domain characteristics  
of the raw signal for analysis, 
%The analysis is carried out
%based on the characteristics derived from the raw signal 
%i.e., in time-domain, 
such as time period, time-series motif, 
construction of density function of time periods, etc.
% For most of the signals, periodicity or the motif can be found by 
%are periodic and the periodicity could be found by 
% auto-correlation. The motif in a time-series represents a repeating pattern % in the series. A time-series might have multiple motifs. 
%\caj{This assumes a periodicity of the signal. Can this always be assumed? Or do we only cover periodic signals?}
%\cpd{Motif is for aperiodic signals, motif represents the repeating patterns}
% One of the major challenges to determine the time-domain characteristics is 
% the presence of noise in the measured or observed signals. 
% Noise
% and other unwanted effects have to be filtered out 
% from the input signal for an efficient signal analysis, which calls for a
% pre-processing stage.
% Throughout this article, we use the term \emph{component} rather than general to denote an identifiable part or element
% whose characteristics, like the amplitude, time period, and so on, can be utilized for analyzing the signal. For instance, it may be a periodically recurring maximum or minimum. 
%\caj{Do we also mean components derived from principal component analysis?}
%\cpd{It can also be}
% The time-domain characteristics widely used for signal analysis are: 
% time period, rate-norm (rate-norm indicates the percentage of components 
% having period higher than a threshold compared to normal period)
% %\cajb{What is meant by rate-norm?}
% for component(s),
% root-mean square difference between intervals of components, mode of the component, and 
% standard deviation. For instance, a component can be a 
% periodic maxima or minima characterized by period and amplitude, which however, may vary significantly. 
% Table \ref{tbl:td_metrics} 
% presents some of the commonly used statistical metrics on the time-domain characteristics for analyzing the 
% signal. 
However, the time-domain characteristics-based analysis's fundamental drawback is that the characteristics are derived from the signal's original state space. The dimensionality is often high, and
some of the derived features may be irrelevant for the classification and signal analysis \cite{Strauss'01}. As such, the time-domain analysis incurs large processing overheads. 
%\cpd{Component could be seen as a 
%periodic maxima or minima, with slight variations 
%in absolute amplitude and period.}
% We illustrate the use of time-domain characteristics based signal 
% analysis by considering a simple time-series 
% electrocardiogram (ECG) signal shown in 
% Figure \ref{fig:ecg_basic}. 
%The terminology used regarding ECG signal is defined below: 
%\textit{\textbf{Component}}: The components of the ECG signal are the P, Q, R, S and T peaks.
%\textit{\textbf{Feature}}: Features of a component refer to its 
%inherent characteristics such as time period, amplitude, width. For instance, R-R 
%interval can be seen as a feature, similarly the width of the QRS complex, or the amplitude of the R peak.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!htb]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{pics/ecg_mkd}
% 	\caption{A pseudo ECG signal and its components}
% 	\label{fig:ecg_basic}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The represented ECG signal (in time-domain) has mainly 5 components: 
% P, Q, R, S and T. These components are determined based on their 
% morphological structures, amplitude, and periodicity. 
% However, the components can be differently determined for different signals. For instance, in an Electroencephalography (EEG) the components are determined based on the frequency bands such as Alpha, Beta, Gamma, and Delta. 
%\caj{All of the are either minima or maxima; so one would conclude that a component is always a local minimum or a local maximum. If that is so, let's say it explicit.}
% Some of the time-domain characteristics considered to 
% analyze the ECG signal using a component as reference are:  
% \begin{itemize}
% 	\item \textbf{Time period:} Time period of a periodic signal is the time after which the signal repeats.
% 	\item \textbf{$\text{pNN}50$}: It is the percentage of successive 
% 	component intervals which differ more than 50\% in duration. pNN50 
% 	stands for the proportion of intervals higher than 50\%. 
% 	This is given as 
% 	\begin{equation}
% 	\begin{aligned} \label{eq:pnn}
% 	\text{PNN50}(\%)=\frac{C}{N} \times 100
% 	\end{aligned}
% 	\end{equation}
% 	where, $C$ denotes the number of times the distance (in time) 
% 	between two 
% 	successive components differ by more than 50\% of its 
% 	normal value and $N$ is 
% 	the total number of considered components. %samples. 
% 	% \caj{The use of the term "interval" is confusing. Do you mean the time distance between two occurrences of the same component? If so, let's define this explicitly, but I am not sure that interval is the right term (in math interval is the set of numbers between two numbers). Is "delay" or "distance" a better term?
% 	% Is PNN50 only used for time distances between component occurrences? Or also for other metrics like amplitude? 
% 	% What does "PNN"  stand for?}
% 	Consider an ECG signal, with a mean of R-R intervals of  
% 	100ms. If the interval between successive R-R peaks is higher 
% 	than 150ms (50\%), $C$ is incremented by 1 and correspondingly the PNN50 is updated. 
% 	The higher the PNN, the more abnormal the signal is. 
% 	%\caj{I made some changes; please check.}
% 	%As such the number of intervals having more than 
% 	% difference 
% 	% For instance, if the R-R intervals of the ECG signal are $RT_1, RT_2, ..., RT_N$, if $RT_{i+1}-RT_i>50ms$,
% 	% then the value of PNN50 is increased by 1 and corresponding percentage value is
% 	% calculated. 
% 	%\caj{This should be defined more precisely. (What is 50ms here? PNN50 is creased by 1?? PNN50 is a percentage, so is the percentage increased by 1? or the fraction, which is between 0 and 1?. I guess the mean of the interval must be computed first?)}
% 	\item \textbf{Mean:} Mean of a time-series represents the average value of the time-series. For a signal $X=\{x_1,x_2,..., x_N\}$, 
% 	mean is mathematically given as
% 	\begin{equation}
% 	\begin{aligned}
% 	\text{Mean}=\mu=\frac{\sum_{i=1}^{N}x_i}{N}
% 	\end{aligned}
% 	\end{equation}
% 	For time-series analysis, the mean over a time window is used as well. 
% 	%\caj{Is the "running mean" (the mean over a running window) also used?}
% 	\item \textbf{RMSD:} Root mean-square deviation (RMSD)
% 	measures the deviation between predicted or detected values and the normal 
% 	values
% 	%\caj{What is the difference of measured and actual values in our context?} 
% 	%\cpd{It should be deviation between predicted and actual or detected and 
% 	%actual component or value}
% 	in the context of prediction; or the deviation between 
% 	detected and actual components in the context of detection. 
% 	RMSD for a signal
% 	$X=\{x_1,x_2,..., x_N\}$ is given by
% 	\begin{equation}
% 	\begin{aligned}
% 	\text{RMSD}=\sqrt{\frac{\sum_{i=1}^N(x_i-\mu)^2}{N}}
% 	\end{aligned}
% 	\end{equation}
% 	%\caj{What is $0^n$?? }
% 	where $\mu$ represents the mean of the series $X$ 
% 	and $N$ denotes the number of samples.
% 	%\caj{Above we used $S$ to denote the number of samples. Is $n$ here the number of samples? Let's use one symbol for the number of samples, $N$ if you want, and use it throughout all formulas.}
	
% 	% \item \textbf{Mode:} Mode is the value in a sequence that occurs often.
% 	% %\caj{Why is that useful and what is the mode in an ECG signal? Perhaps it is useful only for certain types of signals which are dominated by one or a few values, but not relevant for other signals like ECG?}
% 	% Mode is helpful to have 
% 	% a quantitative analysis of individual components in the signal.
% 	% %For instance, in a series like \{13, 18, 13, 14, 13, 16, 14, 21, 13\},
% 	% %the mode is 13, as it has most often occurrence.
% 	% However, it is possible to have a multi-modal sequences i.e., have multiple
% 	% modes. As such, based on the modes, it is possible to see the distribution of
% 	% different components in the signal and further analyze it.
% 	% Mode can be utilized to analyze a time periodic signals, by carefully observing 
% 	% the histogram of individual mode values (if it is a multi-modal signal). 
	
% 	% For an ECG, the mode can be derived for individual components 
% 	% and depending on their variability the arrhythmias can be 
% 	% diagnosed. For instance, a lower mode for T component indicates 
% 	% Ischemia. The mode based analysis is primarily useful 
% 	% for sequences which have repeating patterns or components. 
% 	%\caj{What is the definition of mode?}
% 	\item \textbf{Standard Deviation:} Standard deviations SD1 
% 	represents the standard deviation of the distance (in time) between components and SD2 represents the standard deviation of the  distance between next consecutive components. The SD1 and SD2 considering an ECG signal as example can be given as 
% 	\begin{equation}
% 	\begin{aligned}
% 	\text{SD1} & =\sqrt{\frac{1}{2}\text{Var}(RR_i - RR_{i+1})}; \ \forall i=1,2,...,N\\
% 	\text{SD2} & =\sqrt{2\sigma^2-\frac{1}{2}\text{SD1}^2}
% 	\end{aligned}
% 	\end{equation}
% 	%\caj{What is SDNN in the equation?}
% 	%\caj{Make sure a symbols appears uniformly everywhere. Now SD1 appears differently in normal text and in an equation $SD1$. The best is to define a new command, which then is used and looks identical in all contexts. }
% 	%\cpd{They considered difference between successive RR intervals with next and put it in a vector i.e., \{$RR_1-RR_2$, $RR_2-RR_3$,...\} 
% 	%and further calculated variance for this differences} 
% 	here $RR_i$ represents the R-R interval of the $i^{th}$ beat, 
% 	$Var()$ represents the variance and $\sigma$ represents the 
% 	standard deviation of the component. As such the vector is 
% 	built with the differences of R-R intervals with the succeeding ones. 
% 	Variance and standard deviation are mathematically given as 
% 	\begin{equation}
% 	\begin{aligned}
% 	\text{Var}(X)=& \sigma^2=\sum_{i=1}^N\frac{(x_i-\mu)^2}{N} \\ 
% 	\sigma=& \sqrt{Var(X)} %=\sigma
% 	\end{aligned}
% 	\end{equation}
% 	Here, $X$ is the input series of length $N$; $\mu$ indicates the mean.
% 	Standard deviation is given by square root of variance.
% 	%\caj{There is some inconsistency. In (4) $Var$ takes one scalar value as argument, but in (5) it takes the whole sample set $X$.}
% 	%\cpd{I will cross check the formula}
% 	%\caj{Let's use standard terminology everywhere: $\sigma$ instead of $SDNN$, $\mu$ instead of $Mean$, etc.}
% 	%\caj{Multi-character symbols in math mode look ugly (e.g. $SDNN$), because Latex typesetting assumes that each of the characters is a separate symbol and these symbols are multiplied. It is better to use e.g. } \verb|$\text{SDNN}$|
% 	%\caj{which becomes $\text{SDNN}$, or}
% 	%\verb|$\mathit{SDNN}$}|
% 	%\caj{which becomes $\mathit{SDNN}$. This can be abbreviated in a command like}
% 	%\verb|\newcommand{\mySymbol}[1]{\ensuremath{\mathit{#1}}}|
	
% 	%\verb|\newcommand{\SDNN}{\mySymbol{SDNN}}|
% 	%\newcommand{\mySymbol}[1]{\ensuremath{\mathit{#1}}}
% 	%\newcommand{\SDNN}{\mySymbol{SDNN}}
% 	%\caj{This can be used inside and outside math mode. It has the advantage that all your symbols will look the same, and it is easy to change the font for all of them later on. It can then be used as }
% 	%\verb|$\SDNN = \sigma$|
% 	%\caj{which will display as $\SDNN = \sigma$.}
% 	\item \textbf{Auto-correlation:} Auto-correlation is one of the parametric methods utilized for
% 	time-series analysis that also estimates the disturbances in the signal.
% 	The auto-correlation {\bf R} of a signal $x$ can be
% 	found as
% 	\begin{equation}
% 	\begin{aligned}
% 	{\bf R}_{xx}(\tau)=\int_{-\infty}^{\infty}x(t)\overline{x(t-\tau)} dt
% 	\end{aligned}
% 	\end{equation}
% 	%\caj{What is §u§?}
% 	where $\tau$ indicates the lag and $x(t)$ indicates the signal on which the
% 	auto-correlation is carried out with $t$ representing the 
% 	time instant. This ACF indicates the energy of the signal.
% 	\item \textcolor{red}{Cross-correlation}
% 	\item Some other time-domain metrics are presented in Table \ref{tbl:td_metrics}.
% \end{itemize}
% %Similarly, calculating RMSD between intervals of component provides the
% %information on the variation of signal components. Lower RMSD indicates more uniform signal.
% %In similar manner, standard deviation of the signal, the standard deviation of mean of intervals
% %could be used for analysis.
% %
% %
% %Mode amplitude corresponds to number of samples in the signal that abide the
% %Mode value. Higher the Mode amplitude, lower the anomaly in the signal.
% %Variation range is a bound set by the user/system on particular metrics i.e., $Value_{Min}\leq Value \leq Value_{Max}$.
% %
% \begin{table}[!t]
% 	\centering
% 	\caption{Time-Domain Metrics}
% 	\label{tbl:td_metrics}
% 	% \caj{Let's be clearer in this table with the terms used:
% 	% What exactly is meant with PNN50?
% 	% What is rate-norm?
% 	% What is an interval? Is it the time between two occurrences of the same component? What then is the difference to period?
% 	% -- Interval is same as period for uni modal series, but there can be series with multi-modal (or multiple motifs) 
% 	% What exactly is Mode? The values that appear most often? Why is that interesting? Why is it called mode?
% 	% }
% 	\scalebox{1}{
% 		\begin{tabular}{|p{1.4cm}|p{6.6cm}|}
% %				\begin{tabular}{|p{3cm}|p{7.5cm}|}
% 			\hline
% 			PNN50(\%) & Rate-norm of a component which differ by more than  a threshold  \\
% 			\hline
% 			RMSD & Root mean square difference between consecutive interval  of a component \\
% 			\hline
% 			$\sigma$ & Standard deviation of average duration intervals \\
% 			\hline
% 			SDANN & Standard deviation of mean of interval length of a  component calculated for every  window (5min for ECG signal)\\
% 			\hline
% 			Mode (Mo) & Mode of a series i.e., most frequently recurring value(s) in a time-series\\ %component, not very different from \\
% 			\hline
% 			%\multirow{2}{*}{Mode amplitude} & Number of intervals corresponding to the mode value, \\
% 			% & in \% to the amount of samples \\
% 			%\hline
% 			Variation range  & Variation of amplitude or interval of the component \\
% 			\hline
% 			SD1/SD2 & Ratio of standard deviations SD1 and SD2 \\
% 			\hline
% 		\end{tabular}
% 	} \vspace{-2em}
% \end{table}


%\begin{table}[!t]
%	\centering
%	\scalebox{1}{
%		\begin{tabular}{|p{2.7cm}|p{2.7cm}|}
%			\hline
%			\multirow{2}{*}{PNN50(\%)} & Rate norm of a component which differ by more than  a threshold  \\
%			\hline
%			\multirow{2}{*}{RMSD} & Root mean square difference between consecutive intervals \\
%			& of a component \\
%			\hline
%			$\sigma$ & Standard deviation of average duration intervals \\
%			\hline
%			\multirow{2}{*}{SDANN} & Standard deviation of mean of interval length of a \\
%			& component calculated for every  window (5min for ECG signal)\\
%			\hline
%			\multirow{2}{*}{Mode (Mo)} & Mode of a series i.e., most frequently recurring value(s) \\ %component, not very different from \\
%			& in a time series \\ % mathematical expectation  \\
%			\hline
%\multirow{2}{*}{Mode amplitude} & Number of intervals corresponding to the mode value, \\
% & in \% to the amount of samples \\
%\hline
%			Variation range  & Variation of amplitude or interval of the component \\
%			\hline
%			SD1/SD2 & Ratio of standard deviations SD1 and SD2 \\
%			\hline
%		\end{tabular}
%	}
%	\caption{Time Domain Metrics}
%	\label{tbl:td_metrics}
%\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Some of the time domain metrics like time period, RMSD, PNN50, SD1, 
%SD2 and so on as described in Section \ref{subsubs:tdm} 
%are used to analyze the time series signals such as ECG. 
% The above mentioned metrics are obtained or calculated from the signal and any deviations from the standard values indicating 
% anomaly. In the Table \ref{tbl:td_metrics}, the interval is 
% same as period for univariate series, but there can be 
% series with multivariate (or multiple motifs) series. 
% %\hl{verified for any deviations and/or pre-defined values}.\cajb{What do you mean?}  
% \textbf{\textit{Example:}} For instance, consider the R component of an ECG signal. % If the time period (R-R interval) is $\sim$100ms, then for 
% each instance of the R component, the time period (R-R interval) is 
% compared against 100ms and any significant deviation indicates an
% irregularity in the ECG signal i.e. arrhythmia. Other metrics can be deployed in a similar manner  
% \cite{Guidelines'96}. Similarly, the consecutive R-R intervals 
% {\tiny }can be used calculate SD1, SD2, and also the pNN50. 
% %\caj{The example is a great idea, but let's compute most or all of the metrics, that we introduced, for one specific ECG signal.}
% Some other variants proposed in the literature that use time-domain metrics include
% minimum-distance classifiers \cite{Chakraborty'14}, and template 
% matching \cite{Robert'89} which uses the obtained time-domain metrics 
% for signal analysis. For instance, an Euclidean distance metric is 
% utilized in \cite{Chakraborty'14} for classification of beats 
% in an ECG signal using the extracted components and the time period. 
% The main advantage of employing time-domain characteristics based analysis is its relative low-complexity for some of the time-domain based metrics such as mean, standard deviation, and pNN.
% %\caj{I guess auto-correlation is fairly complex. Can we give complexity numbers for the algorithms?}
% However, the basic drawback of the time-domain characteristics based analysis is 
% that the characteristics are derived from the signal's original state space,
% where the dimensionality is often high and
% some of the derived characteristics may be irrelevant for the classification 
% and signal analysis \cite{Strauss'01}.
% Consider a sample of ECG signal, 
% which will have 12-channels i.e., 12 different ECG leads generating data, analyzing which 
% altogether will lead to a high-dimensional data. Moreover, it is important to note that 
% all the 12-channels might not be relevant for detecting all arrhythmias. 
%and the quality of the analysis is not high and depends heavily on the impact of noise.

%\caj{Perhaps we should elaborate these points more: why is the dimensionality of the state space a problem? Why are some characteristics irrelevant? Giving examples will illustrate theses things and provide an intuition for the reader.}





\subsubsection{Frequency-Domain Characteristics}% Based Analysis}
\label{subsub:fdm}
%In addition to the time-domain characteristics, frequency-domain characteristics can as well be 
%employed for signal analysis. 
% \textcolor{red}{Fourier Transform: give some statements about the behaviour advantages and drawbacks.}
Fast Fourier Transform (FFT) is widely adopted to transform the signal from the time-domain to the frequency-domain. After converting the signal into frequency-domain, the entire signal's energy, or the energy of different frequency bands, can be extracted. Based on the energy or power spectrum, i.e., by studying the variance in the distribution of energy or power across different frequency regions, 
the analysis of the signal is carried-out \cite{Shah'14}. Some of the most widely used frequency-domain characteristics are the
Power Spectrum Density (PSD) \cite{Acharya'04} and Power Spectral Entropy (PSE). 
% Some of the most common frequency-domain characteristics used for analysis are listed in Table \ref{tbl:fd_metrics}.
%The energy of a signal is obtained and the corresponding 
%spectrum is used for analysis of the signal \cite{Shah'14}. 

% The Fast-Fourier Transform (FFT) is defined as
% \begin{equation}
% \begin{aligned}
% X_k=\sum_{n=0}^{N-1}x_ne^{-i2\pi kn/N}\;\;\;\;0\leq k\leq N-1
% \end{aligned} \label{eq:fft}
% \end{equation}
% where $x_n$ represent the $n^{th}$ element in time-series and $X_k$ represents the
% $k^{th}$ frequency component. $N$ represents the size of input series. The FFT can
% be used to obtain the energy or power spectrum density in specific frequency ranges (by modifying the limits in eq (\ref{eq:fft})). As per the Parseval's theorem \cite{Proakis'07}, %\cajb{Add reference.}
% the energy of a signal can be given by the summation of all frequency components i.e.,
% \begin{equation}
% \begin{aligned}
% E_s=\sum|X_k|^2
% \end{aligned} \label{eq:energy}
% \end{equation}
% where $E_s$ represents the energy of the signal.

% \textcolor{red}{Inverse FFT and its typical effects which must be explained for practitioners (e.g. lattice fence effect) 
% In practice many other transforms are used with are more helpful in SP (e.g. cosine, Hadamard ...). How to handle these?
% }

% \noindent\textbf{Power Spectral Density:} One of the most widely used frequency-domain characteristics is the
% Power Spectrum Density (PSD) \cite{Acharya'04}, which indicates the severity of frequency components in
% different frequency ranges such as very low frequency (VLF), low frequency (LF), high frequency (HF), and very high frequency (VHF).
% As we will show in an example later,  the analysis of the signal is performed based on the power distribution in each or between different frequency 
% bands. Here, the power spectral density $PSD$ for a signal $x(t)$ 
% is defined as 
% \begin{equation}\label{eq:psd}
% \begin{aligned}
% \text{PSD}(\omega)=& \lim_{T\to\infty} \textbf{E}[|\hat{x_T}(\omega)|^2] \\
% \hat{x_T}(\omega)= & \frac{1}{\sqrt{T}} \int_{0}^{T} x(t)e^{-i\omega t} dt
% \end{aligned}
% \end{equation}



% %Furthermore, the power in each of the frequency bands can as well be employed for signal 
% %analysis.

% \noindent\textbf{Spectral Entropy:} Spectral entropy also called as Power Spectral Entropy (PSE) is the entropy 
% of the power spectrum of a signal which is also used for signal analysis. PSE is 
% obtained by calculating the normalized power spectral density of the 
% signal, followed by calculating the corresponding entropy. 
% Spectral entropy is given by 
% \begin{equation}
% \begin{aligned}
% \text{PSE}=& -\sum_{i=1}^Np_i\ln p_i; 
% \end{aligned}
% \end{equation}
% where $p_i$ represents the power spectral density for the input $X$, as in (\ref{eq:psd}). 
% Spectral entropy basically quantifies the complexity of the time-series i.e., a low 
% spectral entropy indicates that the spectral power is concentrated in relatively small
% number of frequency bands. 


% Some of the most common frequency-domain characteristics used for analysis are listed in
% Table \ref{tbl:fd_metrics}. The table consists of the basic frequency-domain characteristics spectral density of the signal, energy, 
% entropy, and etc. %Methods to obtain these metrics are presented in Section \ref{subsub:fdm}.




% \begin{table}[!t]
% 	\centering
% 	\caption{Frequency-Domain Metrics}
% 	\label{tbl:fd_metrics}
% 	\scalebox{1}{
% 		% \begin{tabular}{|p{4cm}|p{8.5cm}|}
% 		\begin{tabular}{|p{0.9cm}|p{7cm}|}
% 			\hline
% 			VLF & Power or energy in the very low frequency range \\
% 			\hline
% 			LF & Power or energy in the low frequency range \\
% 			\hline
% 			HF & Power or energy in the high frequency range \\
% 			\hline
% 			VHF & Power or energy in the very high frequency range \\
% 			\hline
% 			ApEn & Approximate entropy quantifying the unpredictability of fluctuations in a time-series  \cite{Sun'14} \\
% 			\hline
% 			SpEn & Spectral entropy quantifies the complexity of the time-series \\
% 			\hline
% 			C0, C1 & Correlation values without shift and with one shift \\
% 			\hline
% 		\end{tabular}
% 	} \vspace{-2em}
% \end{table}
% VLF, LF and etc. in Table \ref{tbl:fd_metrics} are obtained based on Auto-correlation or FFT-based analysis depending
% on the implemented method.
% The power or energy in different frequency ranges are estimated and based on the characteristics
% of the signal. Based on the energy values in each of the frequency 
% domains signal analysis is performed based on the energy distribution 
% pattern in different frequency bands or by deriving statistical 
% metrics presented in Section \ref{subsubs:tdm}. 
% The frequency-domain characteristics-based signal analysis is 
% described with an example below. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%Consider a simple case of analyzing an ECG signal based on the 
%R component whose time period is 100ms i.e., 10Hz. The energy should be 
%high close to 10Hz range, whereas an high energy for R component 
%at 150Hz (say) indicates an irregularity in the R component in the signal. Similarly, 

% \textbf{\textit{Example:}} Consider an example of signal analysis in a system which is designed as 
% a high pass filter. The output of such a system 
% should have zero or low spectral energy in the 
% lower frequency range. Whereas, the presence of energy at 
% low frequency range indicates 
% malfunction of the designed filter. In a similar manner, for most of the 
% signals, the %characteristics 
% energy density in frequency bands depends on the signal characteristics and
% any abnormal 
% energy distribution is considered as an indication of presence of abnormal behavior. 
% It needs to be noted that, to analyze a signal using time-domain or frequency-domain metrics, 
% pre-processing of the signal is critical to avoid the impact of noise.
% The complexity of different time-domain and frequency-domain analysis are 
% presented in Section \ref{sec:cmplx}.


%\caj{We should give an idea and discuss briefly the complexity of the algorithms used for both the time domain and the frequency domain analysis. Or, alternatively, if we cover this in the later section 4, we just refer there.}

\subsection{Regression Techniques} \label{subs:regression}
% In the previous section, we discussed time-series analysis by deriving statistical metrics. In addition, 
% the signal analysis is performed by exploiting 
% the relationship between the independent
% and dependent variables of the signal. 
% For example,
% in a time varying series, time is an independent variable and the
% value of the series is a dependent variable.
%The number of dependent and independent variables can be different.
% This can be done by performing regression and building the model for the 
% time-series or signal under experimentation. 
Regression exploits the relationship between the dependent and independent variables of the 
signal, based on which the analysis for new inputs 
is carried out and validated whether the relationship holds or not.
Regression is mainly employed to 
forecast and predict the signal by exploiting the 
dependency between dependent and independent variables. 
% Though regression is often considered to be a subset of machine learning techniques, we present the regression as a separate section due to its vast usage in time-series analysis. 
Various regression techniques exist which are employed depending on the application. Some of the widely used regression techniques for time-series signal analysis are Multi-variable Liner Regression \cite{Kumar'16}, Multi-variable  Adaptive  Regression  Splines  (MARS) \cite{Marinho'16}, Autoregressive  Moving  Average  (ARMA) \cite{Barbe'16}, Bayesian linear regression(in short referred as Bayesian regression) \cite{Saha'07}, and Logistic  Regression \cite{Prathibhamol'16,Dalvi'16}. 

% Consider a series with independent variable $X$ and dependent variable
% $Y$ ($X$, $Y$ are matrices or vectors). The regression analysis \cite{Harrell'15,Alpaydin'09,Marsland'09} can be mathematically defined as
% \[
% Y=f(X,\beta)
% \]
% where $\beta$ indicates the set of unknown parameters.

% In general, $\beta$ is calculated based on minimizing the error in
% least-square sense. For a particular case of linear regression, 
% $\beta$ is derived based on the input $X$
% and the output $Y$, and can be given as
% \begin{equation}
% \begin{aligned}
% \beta=(X^TX)^{-1}X^TY
% \end{aligned}\label{eq:beta_reg}
% \end{equation}
% %\cajb{Shouldn't the derivation of $\beta$ depend on $f$?}

% For a multi-variable dependent regression, the function can be given as
% \[
% Y=f(X_1, X_2, ...,X_n, \beta_1, \beta_2,...\beta_n)
% \]
% The function $f(...)$ could be linear or a polynomial, depending on the class of regression considered. This regression analysis is widely
% adopted for interpolation, extrapolation, and prediction of the time-series sequences.  
% %\caj{Please add a good reference for regression techniques.}

% \textbf{\textit{Example:}} For instance, consider a simple prediction in which the output 
% can be given as weighted sum of previous $N$ inputs. Once this regression 
% model is built, any deviation in the output from the model i.e., predicted value can be 
% seen as anomaly or noise. The same regression can be applied to predict the sequence of 
% ECG signal discussed in the previous Subsection. In such a case, the input will be 
% a set of samples obtained from previous time window, which will be weighted to 
% predict the ECG signal at the next time-instant. 
% %\caj{Can we compute the regression for a specific ECG signal, perhaps the same that we used in the section above?}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Various regression techniques exist, which are 
% employed depending on the application. Some of the widely used 
% regression techniques for time-series 
% signal analysis are described below. 

% \subsubsection{Multi-variable Linear Regression}
% The most commonly used linear regression is multi-variable linear 
% regression. Multi-variable linear regression \cite{Kumar'16,Wang'16}, %,MLR1},
% also known as multivariate regression, exploits the relation between 
% dependent and independent variables, with more than 2 independent variables:
% \begin{equation}
% \begin{aligned}
% y=\beta_0+\beta_1x_1+\beta_2x_2+...+\beta_Nx_N
% \end{aligned}
% \end{equation}
% where $y$ is the output i.e., the dependent variable with dependence 
% on $N$ input variables $x_i$, $i=1,2,...,N$. The weights are denoted 
% by $\beta$. 

% \paragraph{Example:} For instance, consider a simple example of predicting the ECG signal 
% w.r.t time. In this case the ECG values are the dependent variables, and other conditions including time, altitude, physical position (standing, running, walking, sitting, and so on) 
% are some of the examples of independent variables. The dependent variable is 
% dependent on each of these variables. 
% %\caj{Can you give an example of multiple independent variables in time series signals?}

% %\textcolor{red}{Swap 2.2.2 and 2.2.3}


% \subsubsection{Multi-variable Adaptive Regression Splines (MARS)}
% Multi-variable Adaptive Regression Splines (MARS) \cite{Marinho'16,Crino'07} 
% is an extension of 
% linear regression, but with added capabilities to effectively 
% capture non-linearities and 
% interactions between dependent and independent variables. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.4\textwidth]{pics/mars} \\
% 	\caption{Regression with: (a) Linear regression; (b) MARS}
% 	\label{fig:mars}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% As a simple example, consider a univariate linear regression with $x$, $x\in R$ being the independent 
% variable and $y$, $y\in R$ being the dependent variable. A linear 
% regression will model the behavior as 
% \[
% \widehat{y}=ax+b
% \]
% where $a$ and $b$ are constants and $\widehat{y}$ is the estimated value of $y$. 
% Figure \ref{fig:mars}(a) shows the solution of a linear regression as a
% line passing through most of the data points (indicated by boxes).
% In contrast to linear regression, MARS builds the model considering the
% non-linearities in the data. As such, a model built with MARS looks like 
% %\cajb{$x$ is not in the equation??}
% \[
% \widehat{y}=a\ \max(0,x-c)+b
% \]
% where $a$, $c$ and $b$ are constants. Note, that this
% formula is a simple example of MARS. However, the hinge function
% $\max(0,x-c)$ could be in a different form or could be the sum of multiple hinge functions, as discussed below. 
% Thus, any deviation from perfect linearities %non-linearities
% are captured effectively, as shown in Figure \ref{fig:mars}(b).
% %\caj{Fig 2b does not really illustrate that a non-linearity is effectively dealt with.}

% In general, the model of a MARS is given as follows:
% \begin{equation}
% \begin{aligned}\label{eq:y_mars}
% \widehat{y}=\sum_{i=1}^k a_iB_i(x)
% \end{aligned}
% \end{equation}
% where $a_i$ is a constant and $B_i(x)$ is a basis function, dependent on $x$. The basis function can be a constant or a hinge 
% function, or it can be a product of two or more hinge functions. A \emph{hinge function} 
% is a function defined by a variable and a knot, and takes the 
% following possible forms: $max(0,x-c)$ or $max(0,c-x)$, where 
% $x$ is the variable and $c$ is a constant called \emph{knot}. 

% This MARS model is built in two steps: forward pass step and 
% backward pass step. In forward pass, the modeling starts with an initial 
% intercept term i.e., a constant (which is the mean of the response values). 
% Further, it keeps adding new basis functions based on the input. New basis 
% functions that give a maximum reduction in sum-of-squares of residual 
% error are often added. This is done in a brute force manner. This forward pass is followed by backward pass step. In order to avoid over-fitting, 
% the least effective basis functions are found and removed from the model. The user can limit 
% the number of terms in the forward pass and the total number of basis 
% functions i.e., $k$ in eq. (\ref{eq:y_mars}). 

% \textbf{\textit{Example:}} In \cite{Marinho'16}, MARS is deployed to explore the non-linear 
% relationships between real and the desired responses (measured time-series) in antenna arrays' received signal. 
% Further, these values are utilized to determine the Direction of Arrival (DoA) of the 
% signal for further signal processing. This method enjoys the benefits of efficient 
% modeling of the non-linear data compared to other methods. However, MARS is computationally 
% expensive compared to other techniques \cite{Marinho'16}. 

% %\caj{At the end of each of these subsections, we could give an example of time series, or discuss briefly, for which kinds of time series this analysis is applied with benefit.}

% \subsubsection{AutoRegressive Moving Average}
% Autoregressive Moving Average (ARMA) \cite{Barbe'16} %,ARMA1}
% models the time-series data to analyze the data and/or predict the future series. 
% ARMA is mostly applied especially when the data is non-stationary (a series whose probability 
% distribution changes when shifted in time). 

% %\Hossein: (This sentence looks redundant here! The ARMA models are built basically from autoregressive (AR) and moving average (MA) models.

% For better understanding, AutoRegressive (AR) and Moving Average (MA)
% models are individually presented here, followed by the ARMA model. 

% \noindent\textbf{AutoRegressive model:} AutoRegressive (AR) models are utilized 
% for predicting 
% %\ HS: or forecasting (redundant?!)  
% univariate time-series 
% data (i.e., one variable, excluding time), purely based on its 
% previous values. An autoregression is expressed as 
% %\cajb{OK?}
% %\cpd{Yes}
% \begin{equation}
% \begin{aligned} \label{eq:ar_model}
% y_{t} & =f(y_{t-1},y_{t-2},...,y_{t-p},\epsilon_t) \\
% & =c+\sum_{i=1}^p\phi_iy_{t-i}+\epsilon_t
% \end{aligned}
% \end{equation}
% where $y_t$ represents value of variable $y$ at time instant $t$;
% $\epsilon_t$ is the prediction error at time instant $t$; 
% $p$ represents the order of AR model and $\phi_i$ represents 
% the AR parameters i.e., weights for the model; 
% %\cajb{WHat is $\phi$; what is $p$?}
% $c$ is a constant and $f(...)$ represents the model that fits the 
% time-series. 

% \noindent\textbf{Moving average:} Moving Average (MA) modeling is another regression technique efficient 
% for univariate time-series or signal prediction. 
% %\cajb{What do you mean?}
% The model for moving average (MA($q$)) regression, with order $q$ is 
% given by 
% %\cajb{Why don't you write this also as a sum as above?}
% \begin{equation}
% \begin{aligned}
% y_{t} & =g(\epsilon_t,\epsilon_{t-1},...,\epsilon_{t-q}) \\
% & =\gamma+\epsilon_t+\sum_{i=1}^q \theta_i\epsilon_{t-i} \\  %+...+\theta_q\epsilon_{t-q} \\
% \end{aligned}
% \end{equation}
% where $\theta_1$, $\theta_{1}$, ..., $\theta_{q}$ are the 
% parameters for the moving average model, $\gamma$ is a constant, $q$ denotes the order
% of the moving average model, and $\epsilon_t$ denotes 
% the error, as in (\ref{eq:ar_model}). The order of the MA model 
% indicates the number of error terms considered from the previous 
% predictions. Thus, moving average 
% can be seen as a linear regression of present 
% and previous error terms. 

% \noindent\textbf{Autoregressive Moving average:} Based on the above presented autoregression and moving average models, 
% ARMA can be given as %ARMA combines AR and MA models and can be given as  
% \begin{equation}
% \begin{aligned}\label{eq:arma_model}
% y_{t} & =\gamma+\epsilon_t+\sum_{i=1}^p \phi_i y_{t-i}+ \sum_{i=1}^q \theta_i \epsilon_{t-i} \\
% \end{aligned}
% \end{equation}
% ARMA is generally represented as ARMA$(p,q)$ with $p$ and 
% $q$ representing the orders of AR and MA, respectively. 
% The main advantage of ARMA is its capability to capture the impacts of 
% noise from previous predictions 
% effectively, resulting in an improved prediction accuracy. 
% This method is useful especially for lower order polynomials. 
% %as the computing time becomes negligible. 
% %\cajb{Why so few?}

% To build ARMA regression, the time-series signal is 
% initially modeled to estimate the AR and MA models based on the 
% previous values and errors, and then 
% %\cajb{Why not in one go?} 
% %\cpd{Individual terms i.e., errors and weights are computed to form the whole model}
% an ARMA model is 
% %\cajb{Don't use "could be"! What would that mean? Under which conditions could it be and under which conditions could it not be? Write "is" instead.} 
% formed. Further, based on the differences in 
% predicted signal and the actual signal, the signal can 
% be evaluated. The major drawback of ARMA is the amount of computation 
% increases proportional with the selected order, though the prediction accuracy might not 
% increase at same scale. 
% %\HS: isn't it better to explicitly mention advantage and disadvantage of ARMA in individual bullets? 

% \textbf{\textit{Example:}} In \cite{Barbe'16}, ARMA is utilized for time-series analysis in fractional 
% order systems. 
% In the presence of a diffusion or dispersion component, the fractional behavior 
% forces the estimated poles and zeros of the ARMA model to form an alternating chain. 
% This chain can be detected and consecutively be compressed to finally result 
% in a fractional order version of the ARMA model. 


% \subsubsection{Bayesian Linear Regression}
% \label{sec:bayesian_lr}
% Bayesian linear regression (in short referred as Bayesian regression) \cite{Saha'07} is a %,BLR1,BLR2} is a
% multivariate linear regression, where the output presents the 
% probability of the regression value for a particular point based on 
% the given data. Other similar approaches such as Maximum Likelihood Estimation (MLE) suffer 
% from over-fitting, especially when the amount of trained data has a large variance and 
% biasing when the variance in the dataset is too less \cite{Montgomery'10}. 
% %\caj{Can this be really state in such general terms? Do you have a reference? }
% The basic principle of Bayesian regression is to provide an 
% inference of how good or bad (in 
% terms of probability) the predicted
% %\ estimated 
% values are. 

% Consider a simple linear regression case, given by 
% \begin{equation}
% \begin{aligned}\label{eq:bay}
% y_i=x_i^T\beta+\epsilon_i
% \end{aligned}
% \end{equation}
% here $x_i$ and $\beta$ are vectors of size $k \times 1$, and output is $y_i$. 
% %The input and output vectors are $x_i$, $y_i$, respectively with 
% $\beta$ represents the model fitting parameter vector. 
% $\epsilon_i$ values are independent and normally distributed random 
% variables i.e., it follows a Gaussian distribution with 0 mean ($\epsilon_i \sim N(0,\sigma^2)$). 
% The likelihood function for the output at an input with a given variance 
% (variance is set by user or already known) is given by 
% \begin{equation}
% \begin{aligned}\label{eq:bays_prob}
% p(\bf{y}|\bf{X},\beta,\sigma^2) \propto (\sigma^2)exp(-\frac{1}{2\sigma^2}(\bf{y}-\bf{X}\beta)^T(\bf{y}-\bf{X}\beta))
% \end{aligned}
% \end{equation}
% where $\bf{X}$ is a $n \times k$ matrix and each row is a vector $x_i^T$. 
% $\bf{y}$ is the column $n$-vector ($[y_1,y_2,...,y_n]^T$) with 
% variance $\sigma$.
% $\beta$, denoting the weights, can be derived similar to that 
% in eq. (\ref{eq:beta_reg}).
% %For more in-depth analysis of how these are derived, please refer to \cite{Wakefield'13}. %,BLR1,BLR2}. 

% In practice, the objective of Bayesian linear regression is to maximize 
% $\beta$ in eq. (\ref{eq:bays_prob}) for the given 
% data. Hence, it is often desired to have higher probability 
% for the estimated 
% output for a given input. % is often desired. % when 
% %the probability to have a particular output is high for given 
% %input is maximum, it indicates it is more likely to have that output 
% %for the input. 
% A low probability indicates that the formed model does not fit the data, 
% hence needs to be further optimized. 

% In case of time-series or signal analysis, consider that a model is 
% formed as given in eq. (\ref{eq:bay}) with output $y_i$. However, it is not known how good 
% the derived model is and how reliable the output is. In such cases, the Bayesian regression analysis 
% is carried out to estimate the quality of the derived model. 
% %The derived value i.e., $y_i$ represents the output value. 
% A low probability to have the $y_i$ based on the given data indicates that 
% the model is not accurate and needs to be improved. 

% \textbf{\textit{Example:}} The work in \cite{Saha'07} proposed management of battery life with the aid of Bayesian linear regression 
% with regression and classification in the form of Relevance Vector Machine (RVM), and to state estimation via Particle Filters (PF).  
% Accurate estimates of 
% the state-of-charge (SOC), the state-of-health (SOH), and state-of-life (SOL) 
% for batteries helps in scheduling and managing the involved operations effectively 
% to improve the overall system performance. 


% % Consider the data $D=\{((x_1,y_1),(x_2,y_2),...,(x_n,y_n)\}$, where 
% % $x_i \in R^d$ and $y_i \in R$. The objective or the output of 
% % Bayesian regression is to obtain $p(Y|X,D)$, where $p()$ represents 
% % probability. The basic assumptions for Bayesian regression is that 
% % the independent variable ($Y$)

% % \begin{itemize}
% % \item What is this and how is this related to previously described technique  in Section \ref{subs:regress_tech}
% % \item Involved complexity
% % \end{itemize}
% \subsubsection{Logistic Regression}
% In contrast to other discussed regression techniques, logistic regression 
% \cite{Prathibhamol'16,Dalvi'16} is used %,LR1,LR2} is used 
% for the purpose of classification only. The underlying basic 
% principle is similar to that of a regression. 
% A dependency among dependent 
% and independent variables are initially exploited, following
% the application of the logistic function (hence the name 
% logistic regression). 
% %\HS: This sentence could be written better .. 

% For a given data $D=\{(X_1,y_1),(X_2,y_2),...,(X_n,y_n)\}$, 
% with $X_i \in R^N$ i.e., $N$-dimensional vector and $y_i$ represents 
% the class to which it belongs i.e., $y_i=\{0,1\}$ for the binary case. 
% The logistic function  
% \begin{equation}
% \begin{aligned}\label{eq:log_reg}
% \sigma(a)=\frac{1}{1+e^{-a}}
% \end{aligned}
% \end{equation}
% has an output between 0 and 1, depending on $a$.
% The logistic regression works for the given data  
% as follows: 
% \begin{eqnarray}
% \begin{aligned}
% Y_i \sim P_r(\sigma(\beta^T \cdot X_i)) \\ 
% \end{aligned}
% \end{eqnarray}
% where $P_r$ denotes the Bernoulli distribution 
% (i.e., $P(X=1)=1-P(X=0)$, where $P$ indicates the probability) and 
% $\beta$ indicates the weight vector, similar to that described in eq. (\ref{eq:beta_reg}). Vectors $\beta$ and $X$ are of the same dimension.
% Based on the probability value, the class to which the input belongs 
% to can be determined. 
% The above mentioned example is for a simple binary classification, but it can be extended for multi-class classification.

% \textbf{\textit{Example:}}
% Logistic regression for a binary classification 
% with a simple example is explained here. 
% %\cajb{where below?} 
% Consider the process of classifying an ECG signal as normal or an anomaly. %\normal what? 
% The process considers different signal metrics such as periodicity ($T_p$), 
% amplitudes of individual components ($A_1$), QRS complex deviations ($Q$). 
% For instance, consider the weighted function is formulated as follows
% \[
% w_0+w_1 T_p+w_2 A_1+w_3 Q= W^T\cdot X 
% \]
% \[
% p(an|X)=\sigma(W^T \cdot X)
% \]
% In the above equation, $X$ is a set of parameters i.e., $X=\{T_p,Q,A_1\}$,
% $W=\{w_0,w_1,w_2,w_3\}$ is the set of weights, and $p(an|X)$
% represents the probability to have an anomaly for the observed $X$ in 
% the ECG signal. In this example, it can be clearly seen that 
% an increase in the QRS complex deviations ($Q$) increases the 
% probability to have anomaly. As such, logistic regression could be 
% implemented for classification purpose. 
% %The logistic regression builds a weighted function based on the above 
% %considered parameters and normalized further. 
% %Based on the parameters, the probability of signal to be normal or 
% %anomaly  derived. 

% %observing In this case, the function can be built using different 
% %metrics such as mean, standard deviation and so on. Further, 
% %the dot product of these metric values 
% %and weights is passed to the logistic function, as in
% %(\ref{eq:log_reg}), the signal is classified into one of the 
% %classes.\cajb{Can you give the equation for this example?}

% \subsection{Motif Discovery}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Machine Learning-based Analysis}
Sometimes, a more efficient approach is to learn the signal characteristics and build a model. The advancement in machine learning has facilitated signal analysis efficiently, even under adverse conditions. 
Neural networks (NN)  \cite{Reed'99,Anderson'95,Lipmann'87} are
inspired by the mammalian brain architecture.
Learning process in
neural networks refers to the adaptation of weights between layers and
the update of activation functions. Other types of Neural Networks are  Back  Propagation  Neural  Network (BPNN) \cite{Marsland'09,Gent'91}, Elman  Neural  Network \cite{Deng'16,Lin'15}, Block-based Neural Networks (BbNN) \cite{Merchant'06,Kong'04},
Probabilistic Neural Network (PNN) \cite{Perera'11} and Wavelet neural networks (WNN) \cite{Alexandridis'13,Pan'08}.
% \cite{Alexandridis'13,Chen'10,Pan'08}
% \subsubsection{Neural Networks}
% Neural networks(NN)  \cite{Reed'99,Anderson'95,Lipmann'87} are
% inspired by the mammalian brain architecture.
% A neural network comprises of at least three layers: an input layer, one or more hidden layers,
% and an output layer. In a fully connected neural network all nodes in a succeeding layer are 
% connected to all the nodes in the preceding layer. 
% Each node has inputs and outputs, and
% performs an operation based on its activation function. 
% Different layers could have different activation functions. 
% Learning process in
% neural networks refers to the adaptation of weights between layers and
% the update of activation functions. 
% A traditional neural network with one % hidden layer is illustrated in 
% Figure \ref{fig:trad_neural}.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{pics/neural} \\
% 	\caption{A single-hidden layer neural network with 2 inputs and 2 outputs}
% 	\label{fig:trad_neural}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The output of a neuron in a hidden or output layer can be given as
% \begin{equation}
% \begin{aligned}
% y_j=g(\sum_{i=1}^nw_ix_i+b_j)
% \end{aligned}
% \end{equation}
% where $y_j$ indicates the output of the $j$-th neuron with $n$ inputs,
% given by $x_i$, and $b_j$ denotes the bias. The activation function
% of the node is given by $g(\cdot)$.

% The main parameters to be tuned in neural networks are:
% %\cajb{Number of hidden layers?}
% % cpd{For traditional neural networks, 1 hidden layer is used}
% \begin{itemize}
% 	\item Number of hidden layers (if number of hidden layers is more than 1, it is usually classified under a deep neural network, otherwise it is classified as a shallow neural network).
% 	\item Number of nodes in input, output and hidden layers.
% 	\item Activation functions in hidden and output layers.
% 	%\caj{Is there never an activation function for the input layer neurons?}
% 	%\cpd{No. There is ideally no input layer, it is just inputs, but for differentiation they use term input layer. But, they do pre-processing in some applications}
% 	\item Update procedure for the weights between different layers (learning methodology).
% \end{itemize}

% The number of nodes in the output layer denotes the number of outputs the
% user expects from the signal analysis. For instance, to classify an input series into one of the five categories, the neural network architecture will have five nodes in the output layer. The used activation functions and 
% the methodology to update the weights in neural network are discussed 
% here. 
% %indicate that the signal can be
% %classified effectively into one among the 5 possible categories.
% %As such, these are application specific.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Activation Functions}
% In neural networks, the activation function can be defined as an abstraction representing the
% rate of action potential
% %\HS: action potential in or for ?!
% firing in the cell, i.e. the activation function
% indicates the effectiveness with which the presented data will be helpful
% in determining final output. Different activation functions are
% used in the literature. Some of the most widely used activation functions in a neural network are presented in Table \ref{tbl:nn_acf}.
% The most widely used activation functions are $tanh(x)$ and step functions.
% In Table \ref{tbl:nn_acf}, $x_0$ is the x-value of sigmoid's midpoint, $L$ is the curve's 
% maximum value and $k$ represents the steepness of the curve. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!htb]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{pics/Activation_Functions} \\
% 	\caption{Activation functions: (a) identity; (b) binary step; (c) sigmoid; (d) hyperbolic tangent; (e) exponential linear unit; (f) soft plus; (g) sinusoid; (h) Gaussian}
% 	\label{fig:act_func}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{table}[!t]
% 	\caption{Activation Functions in a Neural Network}
% 	\centering
% 	\scalebox{1}{
% 		\begin{tabular}{|l|l|}
% 			\hline
% 			Name & Formula \\
% 			\hline
% 			Identity & $f(x)=x$  \\
% 			\hline
% 			Binary step & $f(x)= \begin{cases} 0, & \text{if}\ \text{$x < 0$} \\ 1, & \text{otherwise} \end{cases} $ \\
% 			\hline
% 			Logistic & $f(x)=\frac{L}{1+e^{-k(x-x_0)}}$\\ 
% 			\hline
% 			Sigmoid & $f(x)=\frac{1}{1+e^{-x}}$  \\
% 			\hline
% 			Hyperbolic tangent & $f(x)=\tanh(x)=\frac{2}{1+e^{-2x}}-1$  \\
% 			\hline
% 			ArcTan & $f(x)=\tan^{-1}(x)$ \\
% 			\hline
% 			Softsign & $f(x)=\frac{x}{1+|x|}$ \\
% 			\hline
% 			Exponential linear unit & $f(x)= \begin{cases} \alpha(e^x-1), & \text{if}\ \text{$x < 0$} \\ x, & \text{otherwise} \end{cases} $ \\
% 			\hline
% 			SoftPlus & $f(x)=\ln(1+e^x)$ \\
% 			\hline
% 			Sinusoid & $f(x)=\sin(x)$ \\
% 			\hline
% 			Gaussian & $f(x)=e^{-x^2}$ \\
% 			\hline
% 		\end{tabular}
% 	}
% 	\label{tbl:nn_acf}
% 	%\caj{Should it not be $x\leq 0$?}
% \end{table}


% The graphs for the activation functions presented in Table \ref{tbl:nn_acf} are
% shown in Figure \ref{fig:act_func}. The shapes of logistic and sigmoid functions look 
% similar, except the change in the bounds of the function. Similarly, from the perspective 
% of shapes, the hyperbolic tangent, arctan, and softsign look similar with differences 
% in the slope of the curves and the bounds of the functions. 
% It needs to be noted that the graphs shown are 
% a simpler representation of their corresponding shapes, not drawn to the scale. 

% Activation functions are often the most computationally expensive  part in neural networks. 
% Reducing the implementation complexity of these functions often reduces the overall
% computational complexity. These activation functions could be implemented in 
% different manners, such as using Look-Up-Tables (LUTs), BRAMs, utilizing CORDIC 
% algorithms to compute the hyperbolic and trigonometric functions \cite{Qian'06,Gisthuam'00}, and 
% approximate 
% computations \cite{Bian'14,Liu'08} such as Piecewise-Linear-Approximations (PLAs). 


% \paragraph{Updating of Weights}
% \label{sec:update_nn}
% Weights in a neural network can be updated in multiple ways.
% One of the most widely used rules is the Delta rule \cite{Marsland'09}: % \cite{Wiki_Delta}:
% %\caj{Let's add a reference here; perhaps to the wikipedia page: {https://en.wikipedia.org/wiki/Delta\_rule ?}}

% \begin{equation}
% \begin{aligned}\label{eq:wt_update}
% \Delta w_{ij}=\alpha (t_j-y_j)x_i
% \end{aligned}
% \end{equation}
% where $i$ indicates the index of input $x_i$ and $j$ represents the
% index of the $j$-th neuron with $t_j$ and $y_j$ as target and actual
% outputs. $\alpha$ denotes the learning rate.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % We have described the basic functionality of a neural network in 
% % Section \ref{subs:nn}. In addition to the number of neurons and the type of activation functions, various other architecture parameters influence the functionality and performance 
% % of the neural network. 
% We present some of the popular neural network 
% architectures for signal analysis, targeting resource-constrained systems. 

% \subsubsection{Back Propagation Neural Network}
% \label{sec:bpnn}
% Back propagation means updating the weights in the network architecture. In Back propagation neural networks (BPNN) \cite{Marsland'09,Heerman'92,Gent'91} %,BPNN1,BPNN2}, 
% the input data is fed from the input layer to the hidden layer and then to the output layer. 
% However, the weights are updated in the reverse manner. One popular method to update the 
% weights of individual nodes is the Delta rule (eq. (\ref{eq:wt_update})). 
% The weights between the hidden layer and the output layer are 
% updated first based on the target outputs of the system, followed 
% by updating the weights between the hidden layer and the input layer.  
% The overall architecture is also termed popularly as feed-forward neural network. 
% %\caj{Please give the formula that updates the weights based on the error.}

% \textbf{\textit{Example:}} In \cite{Asl'06}, a combination
% of linear and non-linear features of ECG, especially, Heart-Rate Variability (HRV) is provided
% as input for feed-forward ANN with back propagation for ECG classification. Time-domain and frequency-domain based nonlinear
% methods are applied in \cite{Asl'06} to extract the features of ECG and are fed to an ANN classifier
% for ECG arrhythmia detection. The NN architecture comprises of 11 inputs, one hidden layer with
% 20 neurons and 5 outputs. This indicates that the implementation in \cite{Asl'06} can detect 
% and classify up to 5 arrhythmias. The paper claims that the implementation can be effective even when the 
% training dataset is small.
% % The output at each neuron is a real number in the  interval range [0, 1]. 
% This architecture utilizes the features of the ECG and 
% HRV metrics to 
% derive conclusions on arrhythmias, which makes the system prone to noise, unless the neural network itself  
% offsets the effects of noise. 


% \subsubsection{Elman Neural Network}
% Elman neural networks \cite{Deng'16,Lin'15} have explicit feedback 
% from the succeeding layer i.e., there exists a feedback from the 
% output layer to the hidden layer and from the hidden layer to the 
% input layer. It is a BPNN (as described in Section \ref{sec:bpnn}), but 
% with explicit feedback from output layer to hidden layer. 
% The feedback provides the error, depending on the application. 
% For instance, when the neural network is used for 
% prediction, the prediction error is used as feedback signal. 
% As a result, the Elman neural network learns faster and more efficiently,
% even when the signal quality is poor. 
% However, inconsistent data such as random or noisy signals 
% leads to convergence issues. 

% \textbf{\textit{Example:}} An Elman neural network implementation for ECG anomaly detection is proposed in \cite{Mohamad'13}.
% In \cite{Mohamad'13}, for ECG anomaly detection,
% a three step process: pre-processing, processing, and classification is followed. For pre-processing,
% median filter and moving average filters are used to remove high frequency noises, smooth the signal,
% and eliminate the jagged edges. This is followed by Principal Component Analysis (PCA) for reducing the features
% to save the computation costs. The reduced feature set is provided as input to the Elman neural network,
% which is trained with the data. The results have shown a satisfactory results of more than 95\% accuracy.
% The major bottleneck in the Elman neural networks are the amount of 
% required memory resources, especially when the number of utilized nodes and  
% states in the process are high. 

% \subsubsection{Block-based Neural Network}
% For an efficient hardware implementation, Block-based Neural Networks (BbNN) \cite{Merchant'06,Kong'04,Moon'01}
% are often chosen. Their implementations can be seen as 2 dimensional arrays of blocks.
% Each block is a four input/output feed-forward neural network in which the number of inputs and outputs are configurable.
% Each block connects to its neighboring blocks similar to
% a mesh network. The signal flow uniquely specifies the internal
% configuration of the block as well as the overall network structure.
% The number of inputs and outputs for different blocks do not have to be the same. 
% A feed-forward NN based BbNN can be seen as a data flow from the top block
% to the bottom block in a 2D array. A BbNN
% architecture with inputs provided at the top and outputs at the bottom
% is shown in Figure \ref{fig:trad_Bb}.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{pics/NNs_Bb} \\
% 	\caption{Block based neural network architecture}
% 	\label{fig:trad_Bb}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \textbf{\textit{Example:}} A BbNN with morphological features and temporal properties of ECG 
% i.e., Hermite expansion coefficients and RR intervals
% as inputs is proposed for ECG arrhythmia detection and classification 
% in \cite{Jewajinda'10}. However, in \cite{Jewajinda'10}, an online 
% updating mechanism for weights is incorporated.


% \subsubsection{Probabilistic Neural Networks}
% A Probabilistic Neural Network (PNN) \cite{Perera'11} %,PNN1,PNN2} 
% is a feed-forward neural network \cite{Marsland'09,Alpaydin'09} 
% which uses Bayesian statistics i.e., probabilistic evaluations 
% as described in Section \ref{sec:bayesian_lr}, and Kernels to perform 
% pattern analysis. A PNN comprises of an input layer, a pattern layer, 
% a summation layer, and an output layer.  

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{pics/pnn} \\
% 	\caption{Probabilistic Neural Network Architecture}
% 	\label{fig:trad_pnn}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \textbf{\textit{Example:}}
% The input layer in the probabilistic neural networks 
% normalizes the raw input data, such that the range of input 
% becomes 0 to 1. For instance, consider a series $X=\{4,5,7,6,7\}$ which 
% could be normalized as $X_p=\{0.57,0.71,1.00,0.86,1.00\}$ 
% (all the values are divided by 7). However, it does not need to be divided by the maximum value in series, could also some other 
% function %\HS: This sentence is not clear ..
% which will normalizes the input data to be in the range of 0 
% to 1, such as eq. (\ref{eq:log_reg}). This normalized data will be sent 
% to other layers i.e., passed to pattern layer. 
% %\caj{what is normalized? The number of neurons in the input layer? Or the input signals to the input layer neurons?} 
% %and this is input is given to the 
% %pattern layer. 
% The pattern layer is built based on the number of 
% training samples i.e., %for instance
% if for class A the network is 
% trained with 3 samples, one can see three nodes corresponding to 
% class A. As such, the number of 
% nodes in the pattern layer corresponds to the total number of 
% training samples. 
% In case of larger data sets, an optimal number of data sets 
% that covers most of the cases are considered in which the 
% number of nodes are formed based on that the. 
% %\cajb{Is this scalable to large training sets?} 
% The outputs of nodes that belong to a particular 
% class are summed up in the summation layer. In the output layer, 
% the summed up values received from the 
% summation layer for each class are compared and the class with 
% highest accumulated value is 
% voted as the class to which the input data belongs to. 

% % For instance, consider a simple case of differentiating 3 symbols 
% % i.e., 3 classes, as shown in Figure \ref{fig:trad_pnn}. 
% % The input is initially normalized. The nodes in the pattern layer 
% % are often built for each of the individual training samples. 
% % Further, the outputs from nodes in pattern 
% % layer that belongs to same class are summed (In this example, two training 
% % samples are provided for each class, hence 2 nodes for each class in
% % pattern layer, different colors inside the node indicate different 
% % class). In the
% % output layer, the summed values in the summation layer are compared and the class with the highest 
% % value is considered to be the class to which the input relates to.

% Probabilistic neural networks are more suitable for small %scale
% and 
% medium scale input data based applications. On the other hand, for large 
% and (sometimes) even for medium scale data applications, the input 
% training data needs to be optimized. PNNs are widely used for object 
% recognition, pattern recognition, and so on, especially when the training 
% dataset is smaller. However, PNNs are not preferred particularly on 
% hardware-constrained systems, as the number of nodes in the pattern layer 
% scales up proportionately with the training datasets. 

% %\caj{Please add a sentence about the suitability of this network for hardware implementation. It seems the network is very dynamic with large number of nodes for large training sets, which seems very difficult to accommodate in HW. On the other hand we write that we focus on resource constrained implementations.}


% \subsubsection{Wavelet Neural Networks}
% Wavelet neural networks \cite{Alexandridis'13,Chen'10,Pan'08} %,WNN1} 
% constitute a class of feed-forward neural networks with 
% input, hidden, and output 
% layers with backward propagation for updating the weights, 
% as in Section \ref{sec:bpnn}. 
% However, there is only one neuron in the output layer (Figure \ref{fig:trad_wnn}). 

% Wavelet neural networks make use of wavelet as an activation function. 
% Wavelets have the benefit of high compression ability as well as 
% an updating function that involves only a subset of coefficients. 
% Wavelet is a specific pattern or a mathematical function that is 
% intended to possess certain properties. Some of the widely used 
% wavelet functions are Gaussian derivation, second derivative of 
% Gaussian (also called ``Mexican Hat''), and Morlet wavelet. 
% In eq.~(\ref{eq:wnn}), a multi-dimensional wavelet function $\psi(...)$ is utilized.  
% Multidimensional wavelets are widely used, as they can preserve the 
% ``universal approximation'' property
% %\caj{Can you briefly give an intuition of this property?}
% that characterizes neural networks 
% \cite{Alexandridis'13}. The universal approximation theorem says that the approximation 
% in the neural networks i.e., building the model occurs as a result of neural network architecture rather than the 
% activation functions. The output of the wavelet neural network can be given as 
% follows
% \begin{equation}
% \begin{aligned}\label{eq:wnn}
% y=\sum_{i=1}^m x_iw_i^{[0]}+\sum_{j=1}^k w_j^{[2]}\prod_{i=1}^m\psi(\frac{x_i-w_{ijt}^{[1]}}{w_{ijd}^{[1]}}) +w_{k+1}^{[2]}
% \end{aligned}
% \end{equation}
% Here, $m$ represents the number of inputs, $k$ represents the number 
% of nodes in the hidden layer. The scaling factors (weights) between input 
% layer and output layer is given by $w_i^{[0]}$, $i=1,2,...,m$ and 
% the weights between hidden layer and the output layer is represented as 
% $w_j^{[2]}$, $j=1,2,...,k$. The weight vector between input and 
% hidden layer is given by $w_{ij}^{[1]}=(w_{ijt}^{[1]},w_{ijd}^{[1]})$, 
% $i=1,2,...,m; \ j=1,2,...,k$. Translation and dilation factors are 
% represented by $w_{ijt}^{[1]},w_{ijd}^{[1]}$, respectively. 
% For instance, the ''Mexican Hat'' wavelet function can be given as 
% \begin{equation}
% \begin{aligned}
% \psi(x)=(1-x^2)e^{-\frac{1}{2}x^2}
% \end{aligned}
% \end{equation}
% The main idea of the 
% wavelet neural networks is to adapt the wavelet basis in the 
% hidden layers to the training data.  A simple example is to adapt the 
% variance of the Gaussian function based on the inputs. When testing, 
% any input that does not satisfy the adapted variance can be seen as 
% an outlier to the trained data. 

% \textbf{\textit{Example:}} A Wavelet Neural Network (WNN) is proposed in \cite{Ceylan'11} with wavelets 
% as the activation functions. This work uses
% wavelet functions as activation functions in the hidden layer nodes. Morlet and Mexican
% hat wavelet functions are widely selected for experimenting, and it has been shown that an NN with Mexican hat wavelet
% function outperforms a Morlet activation function based NN, in terms of classification
% accuracy \cite{Ceylan'11}. In \cite{Ceylan'11}, ECG signals are first filtered using low-pass and high-pass
% filters. Further, R peaks are detected. The RR intervals are provided as inputs and
% training data for the NN. This work can classify Bundle Branch Blocks (BBBs) and normal beats.

% %In the hidden layer, the inputs are transformed into dilated and 
% %translated version of the \hl{mother wavelet} 
% %\cajb{What is the mother wavelet?} 
% %used in the nodes in 
% %hidden layer (each node in the hidden layer is also called a hidden unit). Finally, in the output layer, the 
% %approximation of target values are estimated. 
% %\caj{The main idea should be explained better.}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{pics/wnn} \\
% 	\caption{Feed-forward Wavelet Neural Network Architecture}
% 	\label{fig:trad_wnn}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In addition to shallow and deep neural networks, there are other machine learning approaches for signal analysis such as Kernel-based Time-series Analysis \cite{Taylor'04} and Support Vector Machines (SVMs)  \cite{Marsland'09,Vapnik'06}.
% \cite{Marsland'09,Steinwart'08,Vapnik'06}.

% \subsection{Other Signal Analysis Approaches based on Machine Learning}
% In addition to shallow and deep neural networks there are other machine learning approaches for signal analysis are Kernel-based Time-series Analysis \cite{Taylor'04,Bernhard'02}, Support Vector Machines (SVMs) \cite{Marsland'09,Steinwart'08,Vapnik'06}, 

% \subsubsection{Kernel-based Time-series Analysis}

% Kernel methods \cite{Taylor'04,Bernhard'02} are another useful set of techniques for pattern analysis and recognition. In contrast to other described techniques, kernel methods
% make use of user-specified kernels, i.e., similarity functions
% over pairs of data points in a raw distribution.
% The main purpose %\HS: intention
% behind 
% having kernels is to have similar output for similar inputs. 

% One of the most widely used Kernel functions is the Radial Basis%\HS: "widely used" is repeated many times in the text.. 
% Function kernel (RBF, also known as Gaussian Kernel), given by
% \begin{equation}
% K(x,\mu)=e^{-\frac{\|x-\mu\|^2}{2\sigma^2}}
% \end{equation}
% where $x$ represents the variable $x$ at a particular 
% time instant and $\mu$ denotes the mean
% %\cajb{$x'$ denotes the mean? Why not use $\mu$?} 
% of the corresponding series $X$ with a 
% variance of $\sigma$. 
% One can see the Kernel as a simple function correlating with a sequence or a window in 
% a time-series result in detecting the patters, resulting in either detecting anomalies or 
% finding the desired patterns in the time-series. 
% %\caj{Can you give an example how the kernel is used for analyzing the times series signal?}

% Other popular functions include String kernels, Graph kernels,
% Fisher kernels, and polynomial kernel. In a broader sense, the underlying 
% operation is to obtain the similarity metric (distance) of the 
% data to the Kernel. However, different kernels are more specific for 
% particular applications, for instance, String kernels are exploited when performing string or text matching, graph kernels to find the 
% similarity between graphs by calculating the inner products and 
% Fisher kernels for image recognition and classification purposes. 
% %\caj{Add a sentence indicating what are the main differences between different kernels. E.g. Is it a different distance metric, or?}

% Consider a simple example of detecting a pattern which resembles Gaussian distribution curve 
% %\cajb{What is a Gaussian pattern?} 
% in a series of data. Application of a RBF, i.e. multiplying the input 
% series with the RBF kernel will result in a maximum output near the 
% existence of the Gaussian pattern and lower values elsewhere. Based 
% on the output of the kernel, corresponding patterns are identified.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Kernels \cite{Hastie'08,Silverman'86} are generally considered to be 
% a measure of similarity in a sense that the kernel function $K({\bf X}, {\bf Y})$ takes a larger value if ${\bf X}$ and ${\bf Y}$ are 
% similar \cite{Alpaydin'09}. 
% %pre-defined functions \hl{using which the patterns in a 
% %data or series can be analyzed}.\cajb{This is weird formulation which I do not understand.} 
% %As defined in Section \ref{subs:kernel}, 
% Kernels are widely applied for problem solving scenarios such as pattern matching and 
% text recognition. In the case of 
% line detection, a kernel is a model of a line and a correlation  
% over the input data series (a set of input data points) which produces a
% maximum correlation or a minimal Euclidean distance 
% or a dot product that
% indicates the presence of a line at those points
% \cite{Garcia'13,Alpaydin'09,Marsland'09,Cruz'04}. In a similar manner, 
% different kernels are employed to perform pattern analysis. 
% The type of kernel depends on the application. %A kernel can be 
% %some of the 
% %existing standard functions like Gaussian functions depending 
% %on the application. 

% \textbf{\textit{Example:}} For arrhythmia detection in ECG signals, a kernel can be 
% a user defined mathematical model of the QRS complex, as provided in \cite{Amiri'15}. 
% This QRS modeled kernel is used for pattern matching i.e., to match the 
% QRS of the incoming signal with the kernel. In case of any mismatch, the arrhythmia 
% will be signaled to the user. 
% In case of classification, Kernel-based optimization can be seen as 
% a convex optimization problem.

% \paragraph{Different Kernels}
% A variety of pre-defined standard Kernels exists and each of them 
% are utilized depending on the application. A few of the commonly 
% used Kernels are listed below. 

% \begin{table}[ht]
% 	\centering
% 	\caption{Common Kernel Functions}
% 	%\scalebox{1}{
% 	\begin{tabular}{|l|l|}
% 		\hline
% 		Name & Formula \\
% 		\hline
% 		\hline
% 		Uniform & $K(x)= \begin{cases} c, & \text{if}\ |x|\leq a \\ 0, & \text{otherwise} \end{cases} $   \\
% 		\hline
% 		Triangular & $K(x)= \begin{cases} (c-|x|), & \text{if}\ x \leq c \\ 1, & \text{otherwise} \end{cases} $  \\
% 		\hline
% 		Gaussian & $K(x)=\frac{1}{\sqrt{2\pi}}e^{-\frac{x^2}{2}}$ \\
% 		\hline
% 		Logistic & $K(x)=\frac{1}{e^x+2+e^{-x}}$  \\
% 		\hline
% 		Sigmoid & $K(x)=\frac{2}{\pi}\frac{1}{e^x+e^{-x}}$ \\
% 		\hline
% 		String$^1$ & $K({\bf X})= \sum_{i:u=s_i} \lambda^{l(i)}$ \\
% 		\hline
% 		\multirow{2}{*}{Fisher Score$^2$} & $K({\bf X}_i, {\bf X}_j)= U_{{\bf X}_i}^TI^{-1} U_{{\bf X}_j}$\\
% 		& $U_{{\bf X}} = \nabla_\theta log P({\bf X}|\theta) $  \\
% 		\hline
% 		Polynomial$^3$ & $K({\bf X},{\bf Y})=({\bf X}^T{\bf Y}+c)^d$ \\
% 		\hline
% 		Radial Basis Function & $K({\bf X},{\bf Y})=exp(-\frac{||{\bf X}-{\bf Y}||^2}{2\sigma^2})$  \\
% 		\hline
% 	\end{tabular}\\[1ex]
% 	\raggedright
% 	$^1$ $i$ represents the string index, ${\bf X}$ is the string with substring $u$ of length $n$, 
% 	$s$ represents the string with which the input is matched; 
% 	parameter $\lambda$ can be set to any value between 0 
% 	and 1.\\ 
% 	$^2$ ${\bf X}_i$, ${\bf X}_j$ are two matrices, $I$ is the fisher information matrix, $\theta$ represents the set of parameters and 
% 	$P({\bf X}|\theta)$ is the likelihood of the probabilistic model. \\ 
% 	$^3$ $d$ is degree of polynomial. \\
% 	\label{tbl:kernels}
% \end{table}

% In Table \ref{tbl:kernels}, $c$ and $a$ are constants; $x$ is a scalar 
% and $K()$ represents the kernel function. 
% Letters in bold (such as ${\bf X},{\bf Y}$) represent Vectors, 
% unless otherwise specified. % otherwise.
% %\todo{References for each of the kernels}
% Fisher Kernels \cite{Zhu'08,Roth'06} are mainly employed for image classification and
% retrieval applications. Graph kernels \cite{Kim'14,Bleik'13} 
% compute inner products on graphs and are seen as 
% functions that measure the similarity between a pair of graphs. 
% Polynomial kernels \cite{Yaman'13,Meijering'99} are equivalent to polynomial regression models 
% but without any learning or updating. For  
% Radial Basis Function (RBF) Kernel (also called as Gaussian kernel) 
% \cite{Wang2'16,Jayasumana'15}, 
% $\sigma^2$ denotes the allowed variance as determined by the user. 
% A RBF kernel is an interpretation of similarity measure between 
% input vectors, with 1 denoting high similarity. 
% Kernel-based recognition are widely employed in the field of image recognition 
% and classification.  

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %\HS: general comment--> It is good for each ML description to mention that they have been widely used in other domains (power,performance, energy efficiency prediction or security improvement) and give some references for that..before going deep into ML application in the context of signal processing.. 

% \subsubsection{Support Vector Machines}

% Support Vector Machines (SVMs) \cite{Marsland'09,Steinwart'08,Vapnik'06} are used for classification and regression analysis.
% An SVM builds a model based on the input data with labels such
% that it could be classified as clear as possible (as provided in labels). 
% Here the label indicates the class or a group to which the 
% input data belongs to. For example, consider an ECG signal, 
% here the label could be name of the  
% component at a particular time instant. 
% %\cajb{What is a label? An example would illuminate the technique.}
% Every new input is mapped to the corresponding category.
% %SVMs make use of the Kernels to build the models and
% %mapping the input data to the category.
% %\cpd{Kernels are used to see if the data could be modeled as standard kernels based on the distance, but most often models are derived from data.}
% SVMs operate on vectors rather than individual
% points, making them robust. For estimating the
% distances, SVMs make use of dot products.
% %\caj{Isn't a kernel function used as distance metric?}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{pics/svm} \\
% 	\caption{Binary classification with (a) other classifiers; (b) SVM}
% 	\label{fig:svm}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In SVMs, the objective is to find a hyper-plane that could separate 
% the positive and negative samples (considering a simple binary classification) with a clear boundary. Let us assume a sample space with 
% vector $w$ being normal to the hyper-plane that separates the data set and a constant $b$. Then the following equation has to be satisfied
% \[
% t_i(w^T\cdot  x_i+b)\geq 1 \\ 
% \]
% where $x_i$ is a sample, and $t_i$ is the 
% %\caj{what is the target output?} 
% target output i.e., the class to which it should belong. $t_i = +$1 for the sample belonging to positive 
% class and $t_i=-1$ for the sample belonging to negative class. 
% %\caj{What is a positive sample and what is a negative sample?}

% The width of the hyper-plane is given by 

% \[
% max(\frac{1}{\|w\|})
% \]
% where $w$ represents the normal vector to the hyper-plane.

% %\caj{What is "max."? and what is $w$? If max is the Maximum function it should be written as $\max(\frac{1}{\|w\|})$}

% Considering all these assumptions, it boils down to optimizing the following equations which 
% could be performed using Karush-Kuhn-Tucker (KKT) conditions \cite{Boyd'04}. %\cajb{Add reference.} 
% \begin{equation}
% \begin{aligned}\label{eq:svm}
% \lambda_i(1-t_i(w^T\cdot x_i+b)) & = 0 \\
% 1-t_i(w^T \cdot x_i+b) & \leq 0 \\ 
% \lambda_i & \geq 0
% \end{aligned}
% \end{equation}
% where $\lambda_i$ is a Lagrange multiplier. 
% %\cajb{Is the . in the equations (12) the Dot-product? It should be written as $\cdot$.}
% The main objective here is to find $w$ and $b$, such that for any sample, 
% the classification can be carried out. 


% A simple example, explaining this SVM method is shown in Figure \ref{fig:svm}. 
% The goal is to perform classification of new input 
% based on the existing data. In this figure, the positive samples are indicated by circles 
% and negative with squares. We first find the normal vector $w$ to the 
% median of the hyper-plane and the width of the hyper-plane. 
% Further, the hyper-plane is formed and the classification can be 
% easily performed by calculating the distance of the sample to the plane, 
% as given by constraint 1 in eq.~(\ref{eq:svm}). 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Support vector machines (SVMs) \cite{Xue'11}  are employed in classification % ,SVM1,SVM2}
% applications. The main objective of SVM is to compute the 
% hyper-plane based on KKT conditions as given in eq.~(\ref{eq:svm}). %\HS: These few lines are repeated above and look redundant here.. 

% The basic process of SVM starts with 
% training of labeled input data 
% %to basically data along with the labels 
% %\cajb{Not understandable!} 
% (labels represent the class to which the data belongs). 
% Further, based on the training data, 
% the normal vector $w$ is calculated. Once the normal vector is obtained, 
% the position of new input data (test data) relative to the obtained 
% hyper-plane has to be computed and based on the 
% relative position, the 
% class of the new input is determined. 

% %\subsection{Genetic Algorithms}
% %\begin{itemize}
% %\item How to use Genetic Algorithms for signal analysis
% %\item Complexity, advantages and limitations
% %\end{itemize}
% Consider a simple case of binary classification i.e., 
% the input data has two classes. A hyper-plane will 
% be formed in between those two classes. 
% Class A is on the left side of hyper-plane and 
% class B to the right side, similar to that in 
% Figure \ref{fig:svm}. Any new input data 
% whose distance is negative i.e., left side 
% of the hyper-plane belongs to class A and the 
% input data whose distance to the hyper-plane is 
% positive belongs to class B.

% \textbf{\textit{Example:}} Similar to neural networks, ECG morphological features can also be used as inputs for 
% arrhythmia detection for SVMs. An ECG classification method based on dynamics and the morphological features is presented in
% \cite{Ye'12}. It applies wavelet transform and Independent Component Analysis (ICA)
% separately to extract the morphological features. Additionally, RR interval information is
% utilized to compute dynamic information. All this information together is provided to SVM
% with Aadial Basis Function (RBF) to perform classification.
\subsection{Deep Learning-based Approaches}
Previously presented techniques such as 
neural networks, SVMs, and kernels are efficient as long as 
the data set is small and has low levels of noise. But, the presence of 
noise and colossal data sets adversely affect the 
performance of traditional machine learning techniques. 
Deep learning has been introduced to address these issues. Deep learning \cite{Goodfellow'16} can be seen as an extension of traditional machine learning
with abstractions and processing at multiple levels.
Different deep learning architectures \cite{Goodfellow'16,Heaton'15} include convolutional 
neural networks \cite{Chen'16,Lawrence'97}, recursive neural networks \cite{Bianchini'01,Williams'89}, deep stacking networks \cite{Nie'14,Deng'13} 
%\cajb{Add reference. Either a good reference for each of those types, or one reference that covers all types well.}
and so  on are introduced depending on the application, with 
architecture, i.e., the connectivity between and within layers, as the main differentiating factor. Other types of sophisticated NNs are Convolutional Neural Network \cite{Lee'16,Li'16},
Recurrent Neural Networks \cite{Chen2'16} and Long  Short-Term  Memory  (LSTM) \cite{Palangi'16,Hochreiter'97}.

% \subsection{Deep Learning-based Approaches}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{pics/autoencoders} \\
% 	\caption{(a) A simple deep learning neural network; (b) a 3-stage auto encoder.}
% 	\label{fig:autoencoder}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % \textcolor{red}{Lacks from some basic papers from Lecun}

% Previously presented techniques such as 
% neural networks, SVMs, and kernels are efficient as long as 
% the data set is small and has low levels of noise. But, the presence of 
% noise and large data sets  adversely affect the 
% performance of traditional machine learning techniques. 
% Deep learning has been introduced to address these issues.

% Deep learning \cite{Goodfellow'16} can be seen as an of extension traditional machine learning
% with abstractions and processing at multiple levels. Deep neural networks are an extended version of neural 
% networks with an increased number of processing layers (hidden layers), as shown in Figure \ref{fig:autoencoder}(a). 
% Different deep learning architectures \cite{Goodfellow'16,Heaton'15} including convolutional 
% neural networks \cite{Chen'16,Lawrence'97}, recursive neural networks \cite{Bianchini'01,Williams'89}, deep stacking networks \cite{Nie'14,Deng'13} 
% %\cajb{Add reference. Either a good reference for each of those types, or one reference that covers all types well.}
% and so  on are introduced depending on the application, with 
% architecture, i.e., the connectivity between and within layers, as the main differentiating factor. 




% For instance, deep stacking networks are a straight forward extension of traditional 3-layer networks. They contain a stack of hidden layers with the outputs of one layer forming the inputs to the succeeding. As such, the weights for the 
% individual hidden layer networks are calculated. Stacked auto-encoders have a set of single 
% hidden layer neural network providing inputs to the hidden layers in a 
% succeeding neural network, as shown in Figure \ref{fig:autoencoder}(b). 
% This hierarchical processing has the 
% advantages of abstracting the input data at different 
% levels. 

% As can be observed that the main principle of deep learning 
% is abstraction of input data in a hierarchical manner.  
% Deep learning techniques are widely used when the data to be processed 
% is of high dimensions, and widely demonstrated on image processing and speech processing rather than simple time-series analysis. 
% However, for completeness of the 
% survey, we include this as a part of high-dimensional time-series  analysis rather than confining 
% to traditional low-dimension time-series analysis. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Convolutional Neural Network}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{pics/NNs_Conv} \\
% 	\caption{Convolutional neural network architecture}
% 	\label{fig:trad_Conv}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% A Convolutional Neural Network (CNN) is a variant of feed-forward neural networks with deep-learning \cite{Lee'16,Li'16,Zhou'15,Ikhwantri'15}.
% The input provided for CNN will be tiled into several smaller segments, with two
% successive segments having an overlap. The amount of overlap can be 
% modified depending on the application and the input data size. 
% Each input neuron/node will be fed with this
% smaller segment of input data and convoluted with a mask. 
% A mask is a filter with which the convolution is performed. 
% Consider an object recognition example, the mask could be a small 
% matrix that represents a subset of the image. The main necessity of 
% masks is for extracting different levels of features in image processing 
% applications. 
% %\caj{The term "mask" should be explained better. Is it an activation function? Or are activation functions used to realize a particular mask? If so, how? Can you give an example how activation functions realize a particular mask? What is the purpose of a mask?} 
% A similar set of parallel layers are arranged with each layer having 
% specific masks i.e., different filters. 
% Further, the output from each layer is transferred to the next layer.
% Thus, the whole CNN comprises a set of parallel layers arranged 
% in a serial manner. 
% The output of each node is smaller in dimension compared to the input.
% %A few number of different activation functions are used.
% %A parallel set of such layers will be available at next layer.
% This dimension reduction continues. Finally, this reduced dimensional output
% is provided to a fully connected network i.e., a traditional neural network
% for final processing.
% CNN finds applications for multi-dimensional data classification and object recognition.

% A convolution based neural network implementation is shown in
% Figure \ref{fig:trad_Conv}. The input is convoluted with different masks
% at the beginning states and the convolution formed with different masks are
% concatenated. The yellow color rectangle represents the mask or 
% the activation function used in the layer. This procedure is 
% repeated and the output is finally obtained
% by providing the convoluted results to a fully connected neural network.
% In order to reduce the dimension, pooling stages are 
% used in between. For example, a moving average 
% filter applied to reduce the size of the data can 
% be seen as a Pooling stage. 
% CNNs are widely used in image processing applications where the amount of data 
% to be processed is often large. 

% \textbf{\textit{Example:}}
% In \cite{Huang'16}, a fine-grained vehicle recognition via deep Convolutional Neural Network (CNN) 
% is proposed. Vehicle and the corresponding parts are localized with the help 
% of Region-based Convolutional Neural Networks (RCNN) and their corresponding 
% features from a set of pre-trained CNNs are aggregated to train an SVM classifier. 
% Further, based on the trained CNNs and SVMs, a fine-grained vehicle classification is 
% performed. CNNs often suffer from large training time and vast amount of 
% resource requirements. 

% \subsubsection{Recurrent Neural Networks}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[height=0.35\textwidth]{pics/RNN} \\
% 	\caption{Recurrent neural network architecture}
% 	\label{fig:RNN}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Recurrent neural networks (RNNs) \cite{Chen2'16} are deep neural networks % ,RNN1,RNN2
% with the notion of memory, hence, they remember the previous state of the 
% network and can be be seen as a class of Elman networks. The state of a node is defined by the input weights 
% of the neuron. An RNN is modeled as 
% \begin{equation}
% \begin{aligned}
% h_t=f(h_{t-1},x_t)
% \end{aligned}
% \end{equation}
% where $h_t$ represents the state of the neural network at time $t$, $x_t$ is the input at time $t$. 
% $f(..)$ represents the next-state function. The state of a 
% neural network is defined as the weights in the 
% network.

% Figure \ref{fig:RNN} illustrates the RNN. The X-axis represents the 
% notion of time and Y axis represent the network. Each block can be 
% seen as a layer (or several layers) in the network i.e. a set of nodes. 
% The current state and the previous state of the hidden layers 
% determines the output at a time instant. In the following equation, 
% the hyperbolic tangent is considered as the activation function of 
% the hidden layer node and it takes the product of the previous state ($h_{t-1}$)
% and a weight vector
% %\cajb{What is the "weight for states"?? It is not explained!} 
% ($W_{hh}$) along with the input $x_t$ and the 
% weight vector $W_{xh}$. Based on the current state and the output 
% weight vector $W_{hy}$ the output $y_t$ is determined.
% %\cajb{Use a different font for tanh!!}
% \begin{equation}
% \begin{aligned}
% h_t=& \tanh(W_{hh}h_{t-1}+W_{xh}x_t) \\
% y_t=& W_{hy}h_t
% \end{aligned}
% \end{equation}

% Note, that the number of states that are considered 
% to determine $h_t$ is variable. In this example, only the previous state ($h_{t-1}$) is considered, but more history states $h_{t-1}\cdots h_{t-k}$ could be used. 
% If a large number of previous states is considered, the system may require significant amount of memory. 

% In general, the current state $h_t$ with $tanh()$ activation functions 
% can be given as 
% %\cajb{Is tanhW a function? Is this consistent with eq. (24)?}
% %\cpd{Tanh is the function W is a vector and so does the other two}
% \begin{equation}
% h_t^l=\tanh \left(W^l \begin{pmatrix}
% h_t^{l-i}\\ 
% h_{t-1}^{l}
% \end{pmatrix}\right)
% \end{equation}
% where $l$ represents the hidden layer number. $W^l$ is the weight vector of 
% the current layer ($W^l$ can be seen as $[W_{xh} W_{hh}]$, for this case,
% the $h_{t}^{l-1}$ is the input $x_t$, as only one hidden layer is used). This indicates that 
% the current state is derived based on the previous state of the current 
% layer and the current state of the one layer below the hidden layer in the hierarchy. It is not 
% necessary to consider the state of lower level hidden layers of all the times, which, however, depends on the application. 

% RNNs are employed widely in applications like image captioning,
% predicting strings, predicting words or characters, 
% language translation, with training set comprised of few words or characters,  
% \cite{Chien'16,Chen2'16} and so on.
% %\caj{This paragraph has several grammar errors and is not understandable!}

% \textbf{\textit{Example:}} A skin detection from images for dermatology applications 
% with a combination of CNN and RNN is proposed in \cite{Zuo'17}. 
% CNN layers are trained to capture the generic local features from the images, while 
% the RNN layers model the semantic contextual dependencies in images. As such, based on 
% the generic and contextual features extracted from the images, skin detection with 
% good accuracy, even in complex background situations is achieved. 

% \subsubsection{Long Short-Term Memory (LSTM)}
% Long short term-memory \cite{Palangi'16,Hochreiter'97} is an extension of RNNs. % ,RNN1
% The main issue in RNNs is the need for large storage to remember a 
% large number of states and computations performed on each of the 
% previous states. As a remedy, LSTM is activated with 
% forget and remember gates. During the training the network evaluates the 
% impact of the previous and current states. The current input 
% and the states, that have impact on the output are 
% kept while the rest is discarded. 
% % It can be mathematically given as 
% % \begin{equation}\label{eq:lstm}
% % \begin{aligned}
% % \begin{pmatrix}
% % i \\
% % f \\
% % o \\
% % g
% % \end{pmatrix} & = \begin{pmatrix}
% % sigm\\ 
% % sigm\\ 
% % sigm\\ 
% % tanh\\ 
% % \end{pmatrix} W^l
% % \begin{pmatrix}
% % h_t^{l-i}\\ 
% % h_{t-1}^{l}
% % \end{pmatrix} \\ 
% % c_t^l & =f \bigodot c_{t-1}^l+i \bigodot g \\ 
% % h_t^l & =o \bigodot tanh(c_t^l)
% % \end{aligned}
% % \end{equation}
% LSTMs are very popular in language processing.
% Similar to RNNs, LSTMs combined with CNNs are employed for 
% image captioning applications. % \cite{LSTM1} purposes. 


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.5em}
\subsection{Hybrid Approaches}
\vspace{-0.5em}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
So far, we have seen some of the individual approaches used for classification or prediction purposes. However, there exist approaches
that use combinations of techniques~\cite{Pazzouki'16,Romsdorfer'09,Alpaydin'09,Marsland'09}. The most common and widely used two-hybrid techniques are discussed below. 
% The following hybrid approaches are explained with the aid of examples. 


\subsubsection{RBF based Neural Networks}
Radial basis functions (RBF) have proven their efficiency in
many applications such as predictions, classifications, approximations,
system controls and many others
\cite{Pazzouki'16,Alpaydin'09,Marsland'09}. 
Work in \cite{Karayiannis'97} proposes a neural network 
with RBF as an activation function.
% Similar to traditional neural networks,
% the architecture consists of three kinds of layers.
% However, the activation functions
% in the hidden layers use RBF, and the 
% output layer simply can be seen as the linear
% combination of outputs from the last hidden layer i.e., RBFs and
% the neuron parameters such as bias.
Different applications of this hybrid technique can be seen as 
fault detection \cite{Li2'16,Meng'10}, control optimization \cite{Yali'08}, and so on. 

\subsubsection{Weighted Distance-based Neural Networks}
Weighted distance-based neural networks \cite{Romsdorfer'09} 
have a similar architecture of a 
traditional neural network. However, the activation functions make use of the weighted distance (Euclidean distance) metric to processes the data and provide the output. These kinds of neural networks are resource-constrained and can be utilized for lightweight applications such as pattern recognition on small scale data \cite{Alpaydin'09}.
% A weighted distance based neural network for pattern recognition is proposed in \cite{Alpaydin'09}.  
% This could also be utilized for finding anomalies in time-series 
% like ECGs, with training data of features like R-R interval 
% distances, QRS morphology and so on. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Other Techniques}
In addition to the above-discussed approaches, there exist approaches such as rule-based classifiers (JOne, JRip, J48), decision tree approaches, ensemble learning-based approaches, and so on. Some of these techniques are lightweight compared to the neural networks but have lower accuracy in classification and analysis \cite{Khaswneh'18}. Similarly, 
Ensemble learning can be seen as a mixture of classifiers but is costly in terms of the number of computations, power, and area. However, ensemble learning is useful when the amount of signal characteristics used for analysis is small in number \cite{Khaswneh'18}. In the case of classification 
of patterns or data in time-series signals, a technique such as clustering is widely employed. 
% Similarly, to detect the repeating patterns, techniques such as Motif discovery 
% are useful. 

\subsection{Discussion and Analysis regarding Techniques for Time-series Analysis}

In the previous subsections, we presented different time-series analysis techniques ranging from various stochastic based techniques to sophisticated machine learning methodologies. Based on the techniques and their characteristics, we target to provide a comprehensive analysis of different techniques and their suitability for various applications and data types in Table \ref{tab:tech_appl}. It needs to be noted that dimensionality refers to the number of independent variables or the number of channels depending on the application. 
For instance, in a 12-lead ECG signal, the number of channels are 
12 which is referred to as dimension in Table \ref{tab:tech_appl}. It needs to be noted that the analysis in Table \ref{tab:tech_appl} is based on the technique and suitability, and the hardware suitability and analysis will be discussed in the next section. 

% \caj{I think here we need a short discussion on how the different methods are applicable to time series signal analysis. Perhaps we can categorize the different methods, e.g. with respect to 

% - A large data set/small data set for learning

% - categorization tasks

% - on-line learning and abstraction

% - approximation and prediction tasks

% - noise resilient

% - resource efficient (for embedded HW/SW implementations)

% What do you think?
% }

% \begin{itemize}
% \item Fuzzy neural networks 
% \item Tree-based methods 
% \end{itemize}





%\section{Techniques for Time-series Analysis}
%\label{sec:tech_tsa}
%Time-series can be analyzed either in time-domain or 
%frequency-domain. For analyzing the series in time-domain, 
%the characteristics of the signal such as periodicity, variance, 
%amplitude and other raw information is utilized.  
%Similarly, time-series can be analyzed in the frequency-domain, 
%the series has to be converted into frequency-domain signal and the 
%respective characteristics such as
%energy, power spectrum density (PSD) have to evaluated.  
%These extracted characteristics can be analyzed using different techniques. 
%As such, we discuss some of the widely used techniques for analyzing 
%time-series signals with the aid of extracted characteristics below. 
%
%
%\subsection{Time-Series Analysis using Statistical Metrics}
%\label{subs:con_met}
%The time-series characteristics refer to the inherent properties of 
%time-series such as periodicity, amplitude, variance, and so on. 
%Statistical metrics derived on the time-series or signal characteristics 
%such as variance, mean, median, mode, and so on can be employed 
%to perform the times-series analysis. 
%The statistical metrics can be applied on both time-domain or frequency-domain characteristics 
%of the signal for analysis. 
%%extracted from
%%the raw signal or by converting the signal into frequency domain and further
%%derive these metrics to analyze the signal. 
%We discuss some of the commonly used %important
%statistical metrics based on the signal characteristics employed for 
%time-series analysis here  \cite{Guidelines'96}.
%
%\subsubsection{Time-Domain Characteristics}% Based Analysis}
%\label{subsubs:tdm} 
%Time-domain characteristics based analysis refer to employing the 
%derived statistical metrics on the time domain characteristics  
%of the signal for analysis. 
%The analysis is carried out
%based on the characteristics derived from the raw signal 
%i.e., in time-domain, such as time period, time-series motif, 
%construction of
%density function of time periods, and so on.
%For most of the signals, periodicity or the motif can be found by 
%%are periodic and the periodicity could be found by 
%auto-correlation. The motif in a time-series represents a pattern 
%that repeats. A time-series might have multiple motifs. 
%%\caj{This assumes a periodicity of the signal. Can this always be assumed? Or do we only cover periodic signals?}
%%\cpd{Motif is for aperiodic signals, motif represents the repeating patterns}
%Noise
%and other effects have to be filtered out 
%from the input signal, which calls for an efficient
%pre-processing stage.
%
%Throughout this article we use the term \emph{component} rather general to denote an identifiable part or an element  
%whose characteristics, like the amplitude, time period and so on, can be utilized for analyzing the signal. For instance it may be a periodically recurring maximum or minimum. 
%%\caj{Do we also mean components derived from principal component analysis?}
%%\cpd{It can also be}
%
%The time-domain characteristics widely used for signal analysis are: 
%time period,
%rate-norm (rate-norm indicates the percentage of components 
%having period higher than a threshold compared to normal period)
%%\cajb{What is meant by rate-norm?}
%for component(s),
%root-mean square difference between intervals of components, mode of the component, and 
%standard deviation. For instance, a component can be a 
%periodic maxima or minima characterized by period and amplitude, which however, may vary significantly. 
%Table \ref{tbl:td_metrics} 
%presents some of the commonly used statistical metrics on the time-domain characteristics for analyzing the 
%signal. 
%%\cpd{Component could be seen as a 
%%periodic maxima or minima, with slight variations 
%%in absolute amplitude and period.}
%
%We illustrate the use of time-domain characteristics based signal 
%analysis by considering a simple time-series 
%electrocardiogram (ECG) signal shown in 
%Figure \ref{fig:ecg_basic}. 
%%The terminology used regarding ECG signal is defined below: 
%%\textit{\textbf{Component}}: The components of the ECG signal are the P, Q, R, S and T peaks.
%%\textit{\textbf{Feature}}: Features of a component refer to its 
%%inherent characteristics such as time period, amplitude, width. For instance, R-R 
%%interval can be seen as a feature, similarly the width of the QRS complex, or the amplitude of the R peak.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[!htb]
%\centering
%\includegraphics[width=0.45\textwidth]{pics/ecg_mkd}
%\caption{A pseudo ECG signal and its components}
%\label{fig:ecg_basic}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The represented ECG signal (in time-domain) has mainly 5 components: 
%P, Q, R, S and T. These components are determined based on their 
%morphological structures, amplitude and periodicity. 
%However, the components can be differently determined for different 
%signals. For instance, in an Electroencephalography (EEG) the 
%components are determined based on the frequency bands such as 
%Alpha, Beta, Gamma, and Delta. 
%%\caj{All of the are either minima or maxima; so one would conclude that a component is always a local minimum or a local maximum. If that is so, let's say it explicit.}
%Some of the time-domain characteristics considered to 
%analyze the ECG signal using a component as reference are:  
%\begin{itemize}
%\item \textbf{Time period:} Time period of a periodic signal is the time after which the signal repeats.
%\item \textbf{$\text{pNN}50$}: It is the percentage of successive 
%component intervals which differ more than 50\% in duration. PNN(50) 
%stands for the proportion of intervals higher than 50\%. 
%This is given as 
%\begin{equation}
%\begin{aligned} \label{eq:pnn}
%\text{PNN50}(\%)=\frac{C}{N} \times 100
%\end{aligned}
%\end{equation}
%where, $C$ denotes the number of times the distance (in time) 
%between two 
%successive components differ by more than 50\% of its 
%normal value and $N$ is 
%the total number of considered components. %samples. 
%% \caj{The use of the term "interval" is confusing. Do you mean the time distance between two occurrences of the same component? If so, let's define this explicitly, but I am not sure that interval is the right term (in math interval is the set of numbers between two numbers). Is "delay" or "distance" a better term?
%
%% Is PNN50 only used for time distances between component occurrences? Or also for other metrics like amplitude? 
%
%% What does "PNN"  stand for?}
%
%Consider an ECG signal, with a mean of R-R intervals of  
%100ms. If the interval between successive R-R peaks is higher 
%than 150ms (50\%), $C$ is incremented by 1 and correspondingly the PNN50 is updated. 
%The higher the PNN, the more abnormal the signal is. 
%
%%\caj{I made some changes; please check.}
%%As such the number of intervals having more than 
%% difference 
%% For instance, if the R-R intervals of the ECG signal are $RT_1, RT_2, ..., RT_N$, if $RT_{i+1}-RT_i>50ms$,
%% then the value of PNN50 is increased by 1 and corresponding percentage value is
%% calculated. 
%
%%\caj{This should be defined more precisely. (What is 50ms here? PNN50 is creased by 1?? PNN50 is a percentage, so is the percentage increased by 1? or the fraction, which is between 0 and 1?. I guess the mean of the interval must be computed first?)}
%\item \textbf{Mean:} Mean of a time series represents the average value of the time series. For a signal $X=\{x_1,x_2,..., x_N\}$, 
%mean is mathematically given as
%\begin{equation}
%\begin{aligned}
%    \text{Mean}=\mu=\frac{\sum_{i=1}^{N}x_i}{N}
%\end{aligned}
%\end{equation}
%For time series analysis, the mean over a time window is used as well. 
%%\caj{Is the "running mean" (the mean over a running window) also used?}
%
%\item \textbf{RMSD:} Root mean-square deviation (RMSD)
%measures the deviation between predicted or detected and the normal 
%values
%%\caj{What is the difference of measured and actual values in our context?} 
%%\cpd{It should be deviation between predicted and actual or detected and 
%%actual component or value}
%in the context of prediction; or the deviation between 
%detected and actual components in the context of detection. 
%RMSD for a signal
%$X=\{x_1,x_2,..., x_N\}$ is given by
%\begin{equation}
%\begin{aligned}
%    \text{RMSD}=\sqrt{\frac{\sum_{i=1}^N(x_i-\mu)}{N}}
%\end{aligned}
%\end{equation}
%%\caj{What is $0^n$?? }
%where $\mu$ represents the mean of the series $X$ 
%and $N$ denotes the number of samples.
%%\caj{Above we used $S$ to denote the number of samples. Is $n$ here the number of samples? Let's use one symbol for the number of samples, $N$ if you want, and use it throughout all formulas.}
%
%% \item \textbf{Mode:} Mode is the value in a sequence that occurs often.
%% %\caj{Why is that useful and what is the mode in an ECG signal? Perhaps it is useful only for certain types of signals which are dominated by one or a few values, but not relevant for other signals like ECG?}
%% Mode is helpful to have 
%% a quantitative analysis of individual components in the signal.
%% %For instance, in a series like \{13, 18, 13, 14, 13, 16, 14, 21, 13\},
%% %the mode is 13, as it has most often occurrence.
%% However, it is possible to have a multi-modal sequences i.e., have multiple
%% modes. As such, based on the modes, it is possible to see the distribution of
%% different components in the signal and further analyze it.
%% Mode can be utilized to analyze a time periodic signals, by carefully observing 
%% the histogram of individual mode values (if it is a multi-modal signal). 
%
%% For an ECG, the mode can be derived for individual components 
%% and depending on their variability the arrhythmias can be 
%% diagnosed. For instance, a lower mode for T component indicates 
%% Ischemia. The mode based analysis is primarily useful 
%% for sequences which have repeating patterns or components. 
%
%%\caj{What is the definition of mode?}
%\item \textbf{Standard Deviation:} Standard deviations SD1 
%represents the standard deviation of the distance (in time) between components and SD2 represents the standard deviation of the  distance between next consecutive components. The SD1 and SD2 considering an ECG signal as example can be given as 
%\begin{equation}
%\begin{aligned}
%    \text{SD1} & =\sqrt{\frac{1}{2}\text{Var}(RR_i - RR_{i+1})}; \ \forall i=1,2,...,N\\
%    \text{SD2} & =\sqrt{2\sigma^2-\frac{1}{2}\text{SD1}^2}
%\end{aligned}
%\end{equation}
%%\caj{What is SDNN in the equation?}
%%\caj{Make sure a symbols appears uniformly everywhere. Now SD1 appears differently in normal text and in an equation $SD1$. The best is to define a new command, which then is used and looks identical in all contexts. }
%%\cpd{They considered difference between successive RR intervals with next and put it in a vector i.e., \{$RR_1-RR_2$, $RR_2-RR_3$,...\} 
%%and further calculated variance for this differences} 
%here $RR_i$ represents the R-R interval of the $i^{th}$ beat, 
%$Var()$ represents the variance and $\sigma$ represents the 
%standard deviation of the component. As such the vector is 
%built with the differences of R-R intervals with the succeeding ones. 
%Variance and standard deviation are mathematically given as 
%\begin{equation}
%\begin{aligned}
%\text{Var}(X)=& \sigma^2=\sum_{i=1}^N\frac{(x_i-\mu)^2}{N} \\ 
%\sigma=& \sqrt{Var(X)} %=\sigma
%\end{aligned}
%\end{equation}
%Here, $X$ is the input series of length $N$; $\mu$ indicates the mean.
%Standard deviation is given by square root of variance.
%%\caj{There is some inconsistency. In (4) $Var$ takes one scalar value as argument, but in (5) it takes the whole sample set $X$.}
%%\cpd{I will cross check the formula}
%%\caj{Let's use standard terminology everywhere: $\sigma$ instead of $SDNN$, $\mu$ instead of $Mean$, etc.}
%%\caj{Multi-character symbols in math mode look ugly (e.g. $SDNN$), because Latex typesetting assumes that each of the characters is a separate symbol and these symbols are multiplied. It is better to use e.g. } \verb|$\text{SDNN}$|
%%\caj{which becomes $\text{SDNN}$, or}
%%\verb|$\mathit{SDNN}$}|
%
%%\caj{which becomes $\mathit{SDNN}$. This can be abbreviated in a command like}
%%\verb|\newcommand{\mySymbol}[1]{\ensuremath{\mathit{#1}}}|
%
%%\verb|\newcommand{\SDNN}{\mySymbol{SDNN}}|
%%\newcommand{\mySymbol}[1]{\ensuremath{\mathit{#1}}}
%%\newcommand{\SDNN}{\mySymbol{SDNN}}
%%\caj{This can be used inside and outside math mode. It has the advantage that all your symbols will look the same, and it is easy to change the font for all of them later on. It can then be used as }
%%\verb|$\SDNN = \sigma$|
%%\caj{which will display as $\SDNN = \sigma$.}
%\item \textbf{Auto-correlation:} Auto-correlation is one of the parametric methods utilized for
%time series analysis that also estimates the disturbances in the signal.
%The auto-correlation {\bf R} of a signal $x$ can be
%found as
%\begin{equation}
%\begin{aligned}
%{\bf R}_{xx}(\tau)=\int_{-\infty}^{\infty}x(t)x(t-\tau) dt
%\end{aligned}
%\end{equation}
%%\caj{What is §u§?}
%where $\tau$ indicates the lag and $x(t)$ indicates the signal on which the
%auto-correlation is carried out with $t$ representing the 
%time instant. This ACF indicates the energy of the signal.
%\item Some other time domain metrics are presented in Table \ref{tbl:td_metrics}.
%\end{itemize}
%
%%Similarly, calculating RMSD between intervals of component provides the
%%information on the variation of signal components. Lower RMSD indicates more uniform signal.
%%In similar manner, standard deviation of the signal, the standard deviation of mean of intervals
%%could be used for analysis.
%%
%%
%%Mode amplitude corresponds to number of samples in the signal that abide the
%%Mode value. Higher the Mode amplitude, lower the anomaly in the signal.
%%Variation range is a bound set by the user/system on particular metrics i.e., $Value_{Min}\leq Value \leq Value_{Max}$.
%%
%
%\begin{table}[!htb]
%\centering
%\caption{Time Domain Metrics}
%\label{tbl:td_metrics}
%% \caj{Let's be clearer in this table with the terms used:
%% What exactly is meant with PNN50?
%% What is rate-norm?
%% What is an interval? Is it the time between two occurrences of the same component? What then is the difference to period?
%% -- Interval is same as period for uni modal series, but there can be series with multi-modal (or multiple motifs) 
%% What exactly is Mode? The values that appear most often? Why is that interesting? Why is it called mode?
%% }
%%\scalebox{1}{
%\begin{tabular}{|l|p{10cm}|}
%%	\begin{tabular}{|p{1.3cm}|p{5.5cm}|}
%\hline
%PNN50(\%) & Rate-norm of a component which differ by more than  a threshold  \\
%\hline
%RMSD & Root mean square difference between consecutive interval  of a component \\
%\hline
%$\sigma$ & Standard deviation of average duration intervals \\
%\hline
%SDANN & Standard deviation of mean of interval length of a  component calculated for every  window (5min for ECG signal)\\
%\hline
%Mode (Mo) & Mode of a series i.e., most frequently recurring value(s) in a time series\\ %component, not very different from \\
%\hline
%%\multirow{2}{*}{Mode amplitude} & Number of intervals corresponding to the mode value, \\
%% & in \% to the amount of samples \\
%%\hline
%Variation range  & Variation of amplitude or interval of the component \\
%\hline
%SD1/SD2 & Ratio of standard deviations SD1 and SD2 \\
%\hline
%\end{tabular}
%%}
%\end{table}
%
%%\begin{table}[!t]
%%	\centering
%%	\scalebox{1}{
%%		\begin{tabular}{|p{2.7cm}|p{2.7cm}|}
%%			\hline
%%			\multirow{2}{*}{PNN50(\%)} & Rate norm of a component which differ by more than  a threshold  \\
%%			\hline
%%			\multirow{2}{*}{RMSD} & Root mean square difference between consecutive intervals \\
%%			& of a component \\
%%			\hline
%%			$\sigma$ & Standard deviation of average duration intervals \\
%%			\hline
%%			\multirow{2}{*}{SDANN} & Standard deviation of mean of interval length of a \\
%%			& component calculated for every  window (5min for ECG signal)\\
%%			\hline
%%			\multirow{2}{*}{Mode (Mo)} & Mode of a series i.e., most frequently recurring value(s) \\ %component, not very different from \\
%%			& in a time series \\ % mathematical expectation  \\
%%			\hline
%			%\multirow{2}{*}{Mode amplitude} & Number of intervals corresponding to the mode value, \\
%			% & in \% to the amount of samples \\
%			%\hline
%%			Variation range  & Variation of amplitude or interval of the component \\
%%			\hline
%%			SD1/SD2 & Ratio of standard deviations SD1 and SD2 \\
%%			\hline
%%		\end{tabular}
%%	}
%%	\caption{Time Domain Metrics}
%%	\label{tbl:td_metrics}
%%\end{table}
%
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Some of the time domain metrics like time period, RMSD, PNN50, SD1, 
%%SD2 and so on as described in Section \ref{subsubs:tdm} 
%%are used to analyze the time series signals such as ECG. 
%The above mentioned metrics are obtained or calculated from the  
%signal and any deviations from the standard values indicate 
%anomaly. In the Table \ref{tbl:td_metrics}, the interval is 
%same as period for univariate series, but there can be 
%series with multivariate (or multiple motifs) series. 
%%\hl{verified for any deviations and/or pre-defined values}.\cajb{What do you mean?}  
%
%\textbf{\textit{Example:}} For instance, consider the R component of an ECG signal. 
%If the time period (R-R interval) is $\sim$100ms, then for 
%each instance of the R component, the time-period (R-R interval) is 
%compared against 100ms and any significant deviation indicates an
%irregularity in the ECG signal i.e. arrhythmia. In a similar manner, 
%other metrics can be used. This idea is proposed in 
%\cite{Guidelines'96}. Similarly, the consecutive R-R intervals 
%between can be used calculate SD1, SD2, and also the pNN50. 
%
%%\caj{The example is a great idea, but let's compute most or all of the metrics, that we introduced, for one specific ECG signal.}
%
%Some other variants proposed in the literature that use time domain metrics include
%minimum-distance classifiers \cite{Chakraborty'14}, template 
%matching \cite{Robert'89}, which uses the obtained time domain metrics 
%for signal analysis. For instance, an Euclidean distance metric is 
%utilized in \cite{Chakraborty'14} for classification of beats 
%in an ECG signal using the extracted components and the time periods. 
%The main advantage of employing time-domain characteristics based analysis is its relative low-complexity for some of the time-domain based metrics such as mean, standard deviation, and pNN.
%%\caj{I guess auto-correlation is fairly complex. Can we give complexity numbers for the algorithms?}
%However, the basic drawback of the time-domain characteristics based analysis is 
%that the characteristics are derived from the signal's original state space,
%where the dimensionality is often high and
%some of the derived characteristics may be irrelevant for the classification 
%and signal analysis \cite{Strauss'01}. Consider a simple of ECG signal, 
%which will have 12-channels i.e., 12 different ECG leads generating data, analyzing which 
%altogether will lead to a high-dimensional data. Moreover, it is important to note that 
%all the 12-channels might not be relevant for detecting all arrhythmias. As such, the 
%time-domain analysis incur large processing overheads. 
%%and the quality of the analysis is not high and depends heavily on the impact of noise.
%
%%\caj{Perhaps we should elaborate these points more: why is the dimensionality of the state space a problem? Why are some characteristics irrelevant? Giving examples will illustrate theses things and provide an intuition for the reader.}
%
%
%
%
%
%\subsubsection{Frequency-Domain Characteristics}% Based Analysis}
%\label{subsub:fdm}
%%In addition to the time-domain characteristics, frequency-domain characteristics can as well be 
%%employed for signal analysis. 
%Fast Fourier Transform (FFT) is widely adopted to 
%transform the signal from the time domain to the frequency domain (eq. (\ref{eq:fft})). After converting the signal into frequency-domain, the energy of the whole signal or in different frequency bands 
%can be extracted. Based on the 
%energy or power spectrum i.e., distribution of energy or power 
%across different frequency regions by studying the variance, 
%the analysis of the signal is carried-out \cite{Shah'14}. 
%%The energy of a signal is obtained and the corresponding 
%%spectrum is used for analysis of the signal \cite{Shah'14}. 
%
%The Fast-Fourier Transform (FFT) is defined as
%\begin{equation}
%\begin{aligned}
%X_k=\sum_{n=0}^{N-1}x_ne^{-i2\pi kn/N}\;\;\;\;0\leq k\leq N-1
%\end{aligned} \label{eq:fft}
%\end{equation}
%where $x_n$ represent the $n^{th}$ element in time-series and $X_k$ represents the
%$k^{th}$ frequency component. $N$ represents the size of input series. This FFT can
%be used to obtain the energy or power spectrum density in specific frequency ranges
%(by modifying the limits in Equation (\ref{eq:fft})). As per the Parseval's theorem, \cite{Proakis'07} %\cajb{Add reference.}
%the energy of a signal can be given by the summation of all frequency components i.e.,
%\begin{equation}
%\begin{aligned}
%E_s=\sum|X_k|^2
%\end{aligned} \label{eq:energy}
%\end{equation}
%where $E_s$ represents the energy of the signal.
%
%
%\noindent\textbf{Power Spectral Density:} One of the most widely used frequency-domain characteristics is the
%power spectrum density (PSD) \cite{Acharya'04}, which indicates the severity of frequency components in
%different frequency ranges such as very low frequency (VLF), low frequency (LF), high frequency (HF) and very high frequency (VHF).
%Based on the power distribution in each or between different frequency 
%bands, the analysis of the signal is performed, as discussed in the example later. The power spectral density $PSD$ for a signal $x(t)$ 
%is defined as 
%\begin{equation}\label{eq:psd}
%\begin{aligned}
%\text{PSD}(\omega)=& \lim_{T\to\infty} \textbf{E}[|\hat{x_T}(\omega)|^2] \\
%\hat{x_T}(\omega)= & \frac{1}{\sqrt{T}} \int_{0}^{T} x(t)e^{-i\omega t} dt
%\end{aligned}
%\end{equation}
%
%
%
%%Furthermore, the power in each of the frequency bands can as well be employed for signal 
%%analysis.
%
%\noindent\textbf{Spectral Entropy:} Spectral entropy also called as power spectral entropy (PSE) is the entropy 
%of the power spectrum of a signal which is also used for signal analysis. This is 
%obtained by calculating the normalized power spectral density of the 
%signal, followed by calculating the corresponding entropy. 
%Spectral entropy is given by 
%\begin{equation}
%\begin{aligned}
%\text{PSE}=& -\sum_{i=1}^Np_i\ln p_i; 
%\end{aligned}
%\end{equation}
%where $p_i$ represents the power spectral density for the input $X$, as in (\ref{eq:psd}). 
%Spectral entropy basically quantifies the complexity of the time-series i.e., a low 
%spectral entropy indicates that the spectral power is concentrated in relatively small
%number of frequency bands. 
%
%
%Some of the most common frequency-domain characteristics used for analysis are listed in
%Table \ref{tbl:fd_metrics}. The basic frequency-domain characteristics spectral density of the signal, energy, 
%entropy, and so on. %Methods to obtain these metrics are presented in Section \ref{subsub:fdm}.
%
%
%
%
%\begin{table}[!htb]
%\centering
%\caption{Frequency Domain Metrics}\label{tbl:fd_metrics}
%\scalebox{1}{
%\begin{tabular}{|l|p{9cm}|}
%%	\begin{tabular}{|p{1cm}|p{6.5cm}|}
%\hline
%VLF & Power or energy in the very low frequency range \\
%\hline
%LF & Power or energy in the low frequency range \\
%\hline
%HF & Power or energy in the high frequency range \\
%\hline
%VHF & Power or energy in the very high frequency range \\
%\hline
%ApEn & Approximate entropy quantifying the unpredictability of fluctuations in a time series  \cite{Sun'14} \\
%\hline
%SpEn & Spectral entropy quantifies the complexity of the time series \\
%\hline
%C0, C1 & Correlation values without shift and with one shift \\
%\hline
%\end{tabular}
%}
%\end{table}
%VLF, LF and so on in Table \ref{tbl:fd_metrics} are obtained based on Auro-correlation or FFT based analysis depending
%on the method implemented.
%The power or energy in different frequency ranges are estimated and based on the characteristics
%of the signal. Based on the energy values in each of the frequency 
%domains signal analysis is performed based on the energy distribution 
%pattern in different frequency bands or by deriving statistical 
%metrics presented in Section \ref{subsubs:tdm}. 
%The frequency-domain characteristics based signal analysis is 
%described with an example below. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%Consider a simple case of analyzing an ECG signal based on the 
%%R component whose time period is 100ms i.e., 10Hz. The energy should be 
%%high close to 10Hz range, whereas an high energy for R component 
%%at 150Hz (say) indicates an irregularity in the R component in the signal. Similarly, 
%
%\textbf{\textit{Example:}} Consider an example of signal analysis in a system which is designed as 
%a high pass filter. The output of such a system 
%should have zero or low spectral energy in the 
%lower frequency range. Whereas the presence of energy at 
%low frequency range indicates 
%malfunction of the designed filter. In a similar manner, for most of the 
%signals, the %characteristics 
%energy density in frequency bands depend on the signal characteristics, 
%any abnormal 
%energy distribution is considered as an indication of presence of abnormal behavior. 
%It needs to be noted that, to analyze a signal using time domain or frequency domain metrics, 
%pre-processing of the signal is critical to avoid the impact of noise.
%The complexity of different time-domain and frequency-domain analysis are 
%presented in Section \ref{sec:cmplx}.
%
%
%%\caj{We should give an idea and discuss briefly the complexity of the algorithms used for both the time domain and the frequency domain analysis. Or, alternatively, if we cover this in the later section 4, we just refer there.}
%
%
%
%\subsection{Regression Techniques}
%\label{subs:regression}
%In the previous section we have discussed time-series analysis by deriving statistical metrics. In addition, 
%the signal analysis is performed by exploiting 
%the relationship between the independent
%and dependent variables of the signal. 
%For example,
%in a time varying series, time is an independent variable and the
%value of the series is a dependent variable.
%%The number of dependent and independent variables can be different.
%This can 
%be done by performing regression and building the model for the 
%time-series or signal under experimentation. 
%Regression exploits the relationship between dependent and independent variables of the 
%signal, based on which the analysis for new inputs 
%is carried out and validated whether the relationship holds or not.
%Regression is mainly employed to 
%forecast and predict the signal by exploiting the 
%dependency between dependent and independent variables. 
%
%
%
%Consider a series with independent variable $X$ and dependent variable
%$Y$ ($X$, $Y$ are matrices or vectors). The regression analysis \cite{Harrell'15,Alpaydin'09,Marsland'09} can be mathematically defined as
%\[
%Y=f(X,\beta)
%\]
%where $\beta$ indicates the set of unknown parameters.
%
%In general, $\beta$ is calculated based on minimizing the error in
%least-square sense. For a particular case of linear regression, 
%$\beta$ is derived based on the input $X$
%and the output $Y$, and can be given as
%\begin{equation}
%\begin{aligned}
%\beta=(X^TX)^{-1}X^TY
%\end{aligned}\label{eq:beta_reg}
%\end{equation}
%%\cajb{Shouldn't the derivation of $\beta$ depend on $f$?}
%
%For a multi-variable dependent regression, the function can be given as
%\[
%Y=f(X_1, X_2, ...,X_n, \beta_1, \beta_2,...\beta_n)
%\]
%The function $f(...)$ could be linear or a polynomial, depending on the class of Regression considered. This regression analysis is widely
%adopted for interpolation, extrapolation and prediction of the time-series sequences.  
%%\caj{Please add a good reference for regression techniques.}
%
%\textbf{\textit{Example:}} For instance, consider a simple prediction in which the output 
%can be given as weighted sum of previous $N$ inputs. Once this regression 
%model is built, any deviations in the output from the model i.e., predicted value can be 
%seen as anomaly or noise. The same regression can be applied to predict the sequence of 
%ECG signal discussed in the previous Subsection. In such a case, the input will be 
%a set of samples obtained from previous time window, which will be weighted to 
%predict the ECG signal at the next time-instant. 
%%\caj{Can we compute the regression for a specific ECG signal, perhaps the same that we used in the section above?}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Various regression techniques exist, which are 
%employed depending on the application. Some of the widely used 
%regression techniques for time series 
%signal analysis are described below. 
%
%\subsubsection{Multi-variable Linear Regression}
%The most commonly used linear regression is multi-variable linear 
%regression. Multi-variable linear regression \cite{Kumar'16,Wang'16,MLR1},
%also known as multivariate regression, exploits the relation between 
%dependent and independent variables, with more than 2 independent variables:
%\begin{equation}
%\begin{aligned}
%y=\beta_0+\beta_1x_1+\beta_2x_2+...+\beta_Nx_N
%\end{aligned}
%\end{equation}
%where $y$ is the output i.e., the dependent variable with dependence 
%on $N$ input variables $x_i$, $i=1,2,...,N$. The weights are denoted 
%by $\beta$. 
%
%\paragraph{Example:} For instance, consider a simple example of predicting the ECG signal 
%w.r.t time. In this case the ECG values are the dependent variables, and other conditions including time, altitude, physical position (standing, running, walking, sitting, and so on) 
%are some of the examples of independent variables. The dependent variable is 
%dependent on each of these variables. 
%%\caj{Can you give an example of multiple independent variables in time series signals?}
%
%
%
%
%\subsubsection{Multi-variable Adaptive Regression Splines (MARS)}
%Multi-variable Adaptive Regression Splines (MARS) \cite{Marinho'16,Crino'07} 
%is an extension of 
%linear regression, but with added capabilities to effectively 
%capture non-linearities and 
%interactions between dependent and independent variables. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.65\textwidth]{pics/mars} \\
%\caption{Regression with: (a) Linear regression; (b) MARS}
%\label{fig:mars}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%As a simple example, consider a univariate linear regression with $x$, $x\in R$ being the independent 
%variable and $y$, $y\in R$ being the dependent variable. A linear 
%regression will model the behavior as 
%\[
%\widehat{y}=ax+b
%\]
%where $a$ and $b$ are constants and $\widehat{y}$ is the estimated value of $y$. 
%Figure \ref{fig:mars}(a) shows the solution of a linear regression as a
%line passing through most of the data points (indicated by boxes).
%In contrast to linear regression, MARS builds the model considering the
%non-linearities in the data. As such, a model built with MARS looks like 
%%\cajb{$x$ is not in the equation??}
%\[
%\widehat{y}=a\ \max(0,x-c)+b
%\]
%where $a$, $c$ and $b$ are constants. Note, that this
%formula is a simple example of MARS. Hwever, the hinge function
%$\max(0,x-c)$ could be in a different form or could be the sum of multiple hinge functions, as discussed below. 
%Thus, any deviations from perfect linearities %non-linearities
%are captured effectively, as shown in Figure \ref{fig:mars}(b).
%%\caj{Fig 2b does not really illustrate that a non-linearity is effectively dealt with.}
%
%In general, the model of a MARS is given as follows:
%\begin{equation}
%\begin{aligned}\label{eq:y_mars}
%\widehat{y}=\sum_{i=1}^k a_iB_i(x)
%\end{aligned}
%\end{equation}
%where $a_i$ is a constant and $B_i(x)$ is a basis function, dependent on $x$. The basis function can be a constant or a hinge 
%function, or a product of two or more hinge functions. A \emph{hinge function} 
%is a function defined by a variable and a knot, and takes the 
%following possible forms: $max(0,x-c)$ or $max(0,c-x)$, where 
%$x$ is the variable and $c$ is a constant called \emph{knot}. 
%
%Building this MARS model is performed in two steps: forward pass step and 
%backward pass step. In forward pass, the modeling starts with an initial 
%intercept term i.e., a constant (which is the mean of the response values). 
%Further, it keeps adding new basis functions based on the input. New basis 
%functions that give a maximum reduction in sum-of-squares of residual 
%error are often added. This is done in a brute force manner. This forward pass is followed by backward pass step. In order to avoid over-fitting, 
%the least effective basis functions are found and removed from the model. The user can limit 
%the number of terms in the forward pass and the total number of basis 
%functions i.e., $k$ in (\ref{eq:y_mars}). 
%
%\textbf{\textit{Example:}} In \cite{Marinho'16}, MARS is deployed to explore the non-linear 
%relationships between real and the desired responses in antenna arrays' received signal. 
%Further, these values are utilized to determine the direction of arrival (DoA) of the 
%signal for further signal processing. This method enjoys the benefits of efficient 
%modeling of the non-linear data compared to other methods. However, MARS is computationally 
%expensive compared to other techniques \cite{Marinho'16}. 
%
%%\caj{At the end of each of these subsections, we could give an example of time series, or discuss briefly, for which kinds of time series this analysis is applied with benefit.}
%
%\subsubsection{AutoRegressive Moving Average}
%Autoregressive Moving Average (ARMA) \cite{Barbe'16,ARMA1}
%models the time series data to analyze the data and/or predict the future series. 
%ARMA is mostly applied especially when the data is non-stationary (a series whose probability 
%distribution changes when shifted in time). The autoregressive moving 
%average (ARMA) models are built basically from autoregressive (AR) and 
%moving average (MA) models. For better understanding, AR and MA 
%models are individually presented, followed by the ARMA model. 
%
%\noindent\textbf{Autoregressive model:} Autoregressive (AR) models are utilized 
%for predicting or forecasting univariate time series 
%data (i.e., one variable, excluding time), purely based on its 
%previous values. An autoregression is expressed as 
%%\cajb{OK?}
%%\cpd{Yes}
%\begin{equation}
%\begin{aligned} \label{eq:ar_model}
%y_{t} & =f(y_{t-1},y_{t-2},...,y_{t-p},\epsilon_t) \\
%      & =c+\sum_{i=1}^p\phi_iy_{t-i}+\epsilon_t
%\end{aligned}
%\end{equation}
%where $y_t$ represents value of variable $y$ at time instant $t$;
%$\epsilon_t$ is the prediction error at time instant $t$; 
%$p$ represents the order of AR model and $\phi_i$ represents 
%the AR parameters i.e., weights for the model; 
%%\cajb{WHat is $\phi$; what is $p$?}
%$c$ is a constant and $f(...)$ represents the model that fits the 
%time series. 
%
%\noindent\textbf{Moving average:} Moving average (MA) modeling is another regression technique efficient 
%for univariate time-series or signal prediction. 
%%\cajb{What do you mean?}
%The model for moving average (MA($q$)) regression, with order $q$ is 
%given by 
%%\cajb{Why don't you write this also as a sum as above?}
%\begin{equation}
%\begin{aligned}
%y_{t} & =g(\epsilon_t,\epsilon_{t-1},...,\epsilon_{t-q}) \\
%      & =\gamma+\epsilon_t+\sum_{i=1}^q \theta_i\epsilon_{t-i} \\  %+...+\theta_q\epsilon_{t-q} \\
%\end{aligned}
%\end{equation}
%where $\theta_1$, $\theta_{1}$, ..., $\theta_{q}$ are the 
%parameters for the moving average model, $\gamma$ is a constant, $q$ denotes the order
%of the moving average model, and $\epsilon_t$ denotes 
%the error, as in (\ref{eq:ar_model}). The order of the MA model 
%indicates the number of error terms considered from the previous 
%predictions. Thus, moving average 
%can be seen as a linear regression of present 
%and previous error terms. 
%
%\noindent\textbf{Autoregressive Moving average:} Based on the above presented autoregression and moving average models, 
%ARMA can be given as %ARMA combines AR and MA models and can be given as  
%\begin{equation}
%\begin{aligned}\label{eq:arma_model}
%y_{t} & =\gamma+\epsilon_t+\sum_{i=1}^p \phi_i y_{t-i}+ \sum_{i=1}^q \theta_i \epsilon_{t-i} \\
%\end{aligned}
%\end{equation}
%ARMA is generally represented as ARMA$(p,q)$ with $p$ and 
%$q$ representing the orders of AR and MA, respectively. 
%ARMA has an advantage of capturing the impacts  of 
%noise from previous predictions 
%effectively, resulting in an improved prediction accuracy. 
%This method is useful especially for lower order polynomials. 
%%as the computing time becomes negligible. 
%%\cajb{Why so few?}
%
%To build ARMA regression, the time series signal is 
%initially modeled to estimate the AR and MA models based on the 
%previous values and errors, and then 
%%\cajb{Why not in one go?} 
%%\cpd{Individual terms i.e., errors and weights are computed to form the whole model}
%an ARMA model is 
%%\cajb{Don't use "could be"! What would that mean? Under which conditions could it be and under which conditions could it not be? Write "is" instead.} 
%formed. Further, based on the differences in 
%predicted signal and the actual signal, the signal can 
%be evaluated. The major drawback of ARMA is the amount of computation 
%increases proportional with the selected order, though the prediction accuracy might not 
%increase at same scale. 
%
%\textbf{\textit{Example:}} In \cite{Barbe'16}, ARMA is utilized for time series analysis in fractional 
%order systems. 
%In the presence of a diffusion or dispersion component, the fractional behavior 
%forces the estimated poles and zeros of the ARMA model to form an alternating chain. 
%This chain can be detected and consecutively be compressed to finally result 
%in a fractional order version of the ARMA model. 
%
%
%\subsubsection{Bayesian Linear Regression}
%\label{sec:bayesian_lr}
%Bayesian linear regression (in short referred as Bayesian regression) \cite{Saha'07,BLR1,BLR2} is a
%multivariate linear regression, where the output presents the 
%probability of the regression value for a particular point based on 
%the given data. Other similar approaches such as maximum likelihood estimation (MLE) suffer 
%from over-fitting, especially when the amount of trained data has a large variance and 
%biasing when the variance in the dataset is too less \cite{Montgomery'10}. 
%%\caj{Can this be really state in such general terms? Do you have a reference? }
%The basic principle of Bayesian regression is to provide an 
%inference of how good or bad (in 
%terms of probability) the predicted or estimated values are. 
%
%Consider a simple linear regression case, given by 
%\begin{equation}
%\begin{aligned}\label{eq:bay}
%y_i=x_i^T\beta+\epsilon_i
%\end{aligned}
%\end{equation}
%here $x_i$ and $\beta$ are vectors of size $k \times 1$, and output is $y_i$. 
%%The input and output vectors are $x_i$, $y_i$, respectively with 
%$\beta$ represents the model fitting parameter vector. 
%$\epsilon_i$ values are independent and normally distributed random 
%variables i.e., it follows a Gaussian distribution with 0 mean ($\epsilon_i \sim N(0,\sigma^2)$). 
%The likelihood function for the output at an input with a given variance 
%(variance is set by user or already known) is given by 
%\begin{equation}
%\begin{aligned}\label{eq:bays_prob}
%p(\bf{y}|\bf{X},\beta,\sigma^2) \propto (\sigma^2)exp(-\frac{1}{2\sigma^2}(\bf{y}-\bf{X}\beta)^T(\bf{y}-\bf{X}\beta))
%\end{aligned}
%\end{equation}
%where $\bf{X}$ is a $n \times k$ matrix and each row is a vector $x_i^T$. 
%$\bf{y}$ is the column $n$-vector ($[y_1,y_2,...,y_n]^T$) with 
%variance $\sigma$.
%$\beta$, denoting the weights, can be derived similar to that 
%in (\ref{eq:beta_reg}).
%For more in-depth analysis of how these are derived, please refer to \cite{Wakefield'13,BLR1,BLR2}. 
%
%In practice, the objective of Bayesian linear regression is to maximize 
%$\beta$ (\ref{eq:bays_prob}) for the given 
%data. Hence, it is often desired to have higher probability 
%for the estimated 
%output for given input. % is often desired. % when 
%%the probability to have a particular output is high for given 
%%input is maximum, it indicates it is more likely to have that output 
%%for the input. 
%A low probability indicates that the formed model does not fit the data, 
%hence needs to be further optimized. 
%
%In case of time-series or signal analysis, consider that a model is 
%formed as given in (\ref{eq:bay}) with output $y_i$. However, it is not known how good 
%the derived model is and how reliable the output is. In such cases, the Bayesian regression analysis 
%is carried out to estimate the quality of the derived model. 
%%The derived value i.e., $y_i$ represents the output value. 
%A low probability to have the $y_i$ based on the given data indicates that 
%the model is not accurate and needs to be improved. 
%
%\textbf{\textit{Example:}} Management of battery life with the aid of Bayesian linear regression 
%with regression and classification in the form of relevance vector machine (RVM), and to state estimation via particle filters (PF) is proposed in \cite{Saha'07}. 
%Accurate estimates of 
%the state-of-charge (SOC), the state-of-health (SOH) and state-of-life (SOL) 
%for batteries helps in scheduling and managing the involved operations effectively 
%to improve the overall system performance. 
%
%
%% Consider the data $D=\{((x_1,y_1),(x_2,y_2),...,(x_n,y_n)\}$, where 
%% $x_i \in R^d$ and $y_i \in R$. The objective or the output of 
%% Bayesian regression is to obtain $p(Y|X,D)$, where $p()$ represents 
%% probability. The basic assumptions for Bayesian regression is that 
%% the independent variable ($Y$)
%
%% \begin{itemize}
%% \item What is this and how is this related to previously described technique  in Section \ref{subs:regress_tech}
%% \item Involved complexity
%% \end{itemize}
%\subsubsection{Logistic Regression}
%In contrast to other discussed regression techniques, logistic regression 
%\cite{Prathibhamol'16,Dalvi'16,LR1,LR2} is used 
%for the purpose of classification only. The underlying basic 
%principle is similar to that of a regression. 
%A dependency among dependent 
%and independent variables are initially exploited, following
%the application of the logistic function (hence the name 
%logistic regression). 
%
%For given data $D=\{(X_1,y_1),(X_2,y_2),...,(X_n,y_n)\}$, 
%with $X_i \in R^N$ i.e., $N$-dimensional vector and $y_i$ represents 
%the class to which it belongs i.e., $y_i=\{0,1\}$ for the binary case. 
%The logistic function  
%\begin{equation}
%\begin{aligned}\label{eq:log_reg}
%\sigma(a)=\frac{1}{1+e^{-a}}
%\end{aligned}
%\end{equation}
%has an output between 0 and 1, depending on $a$.
%The logistic regression works for the given data  
%as follows: 
%\begin{eqnarray}
%\begin{aligned}
%Y_i \sim P_r(\sigma(\beta^T \cdot X_i)) \\ 
%\end{aligned}
%\end{eqnarray}
%where $P_r$ denotes the Bernoulli distribution 
%(i.e., $P(X=1)=1-P(X=0)$, where $P$ indicates the probability) and 
%$\beta$ indicates the weight vector, similar to that described in (\ref{eq:beta_reg}). Vectors $\beta$ and $X$ are of the same dimension.
%Based on the probability value, the class to which the input belongs 
%to can be determined. 
%The above mentioned example is for a simple binary classification, but it can be extended for multi-class classification.
%
%\textbf{\textit{Example:}}
%Logistic regression for a binary classification 
%with a simple example is explained here. 
%%\cajb{where below?} 
%Consider the process of classifying an ECG signal as normal or an anomaly. 
%The process considers different signal metrics such as periodicity ($T_p$), 
%amplitudes of individual components ($A_1$), QRS complex deviations ($Q$). 
%For instance, consider the weighted function is formulated as follows
%\[
%w_0+w_1 T_p+w_2 A_1+w_3 Q= W^T\cdot X 
%\]
%\[
%p(an|X)=\sigma(W^T \cdot X)
%\]
%In the above equation, $X$ is a set of parameters i.e., $X=\{T_p,Q,A_1\}$,
%$W=\{w_0,w_1,w_2,w_3\}$ is the set of weights, and $p(an|X)$
%represents the probability to have an anomaly for the observed $X$ in 
%the ECG signal. In this example, it can be clearly seen that 
%an increase in the QRS complex deviations ($Q$) increases the 
%probability to have anomaly. As such, logistic regression could be 
%implemented for classification purpose. 
%%The logistic regression builds a weighted function based on the above 
%%considered parameters and normalized further. 
%%Based on the parameters, the probability of signal to be normal or 
%%anomaly  derived. 
%
%%observing In this case, the function can be built using different 
%%metrics such as mean, standard deviation and so on. Further, 
%%the dot product of these metric values 
%%and weights is passed to the logistic function, as in
%%(\ref{eq:log_reg}), the signal is classified into one of the 
%%classes.\cajb{Can you give the equation for this example?}
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%\subsection{Machine Learning based Analysis}
%In the previous subsections, we presented the time-series
%signal analysis based on the extracted
%metrics and regression. Sometimes, a more efficient approach is to learn the signal characteristics and build a model. The advancement in machine learning has facilitated signal analysis efficiently even under adverse conditions. We discuss a few of them here, especially from the hardware implementation perspective. 
%
%\subsubsection{Neural Networks}
%
%Neural networks \cite{Reed'99,Anderson'95,Lipmann'87} are
%inspired by the mammalian brain architecture.
%A neural network comprises of at least three layers: an input layer, one or more hidden layers,
%and an output layer. In a fully connected neural network all nodes in a succeeding layer are 
%connected to all the nodes in the preceding layer. 
%Each node has inputs and outputs, and
%performs an operation based on its activation function. 
%Different layers could have different activation functions. 
%Learning in
%neural networks is the adaptation of weights between layers and
%the update of activation functions. 
%A traditional neural network with one 
%hidden layer is illustrated in 
%Figure \ref{fig:trad_neural}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.65\textwidth]{pics/neural} \\
%\caption{A single-hidden layer neural network with 2 inputs and 2 outputs}
%\label{fig:trad_neural}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The output of a neuron in a hidden or output layer can be given as
%\begin{equation}
%\begin{aligned}
%y_j=g(\sum_{i=1}^nw_ix_i+b_j)
%\end{aligned}
%\end{equation}
%where $y_j$ indicates the output of the $j$-th neuron with $n$ inputs,
%given by $x_i$, and $b_j$ denotes the bias. The activation function
%of the node is given by $g(\cdot)$.
%
%The main parameters to be tuned in neural networks are:
%%\cajb{Number of hidden layers?}
%% cpd{For traditional neural networks, 1 hidden layer is used}
%\begin{itemize}
%\item Number of hidden layers (if number of hidden layers is more than 1, it is usually classified under deep neural network, else as shallow neural network).
%\item Number of nodes in input, output and hidden layers.
%\item Activation functions in hidden and output layers.
%%\caj{Is there never an activation function for the input layer neurons?}
%%\cpd{No. There is ideally no input layer, it is just inputs, but for differentiation they use term input layer. But, they do pre-processing in some applications}
%\item Update procedure for the weights between different layers (learning methodology).
%\end{itemize}
%
%The number of nodes in the output layer denotes the number of outputs the
%user expects from the signal analysis. For instance, to classify an input series into one of the five categories, the neural network architecture will have five nodes in the output layer. The used activation functions and 
%the methodology to update the weights in neural network are discussed 
%here. 
%%indicate that the signal can be
%%classified effectively into one among the 5 possible categories.
%%As such, these are application specific.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\paragraph{Activation Functions}
%In neural networks, the activation function can be seen as an abstraction representing the
%rate of action potential firing in the cell, i.e. the activation function
%indicates the effectiveness with which the presented data will be helpful
%in determining final output. Different activation functions are
%used in the literature. Some of the most widely used are presented in Table \ref{tbl:nn_acf}.
%Most widely used activation functions are $tanh(x)$ and step functions.
%In Table \ref{tbl:nn_acf}, $x_0$ is the x-value of sigmoid's midpoint, $L$ is the curve's 
%maximum value and $k$ represents the steepness of the curve. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[!htb]
%\centering
%\includegraphics[width=0.45\textwidth]{pics/Activation_Functions} \\
%\caption{Activation functions: (a) identity; (b) binary step; (c) sigmoid; (d) hyperbolic tangent; (e) exponential linear unit; (f) soft plus; (g) sinusoid; (h) Gaussian}
%\label{fig:act_func}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%\begin{table}[!t]
%\caption{Activation Functions in a Neural Network}
%\centering
%\scalebox{1}{
%\begin{tabular}{|l|l|}
%\hline
%Name & Formula \\
%\hline
%Identity & $f(x)=x$  \\
%\hline
%Binary step & $f(x)= \begin{cases} 0, & \text{if}\ \text{$x < 0$} \\ 1, & \text{otherwise} \end{cases} $ \\
%\hline
%Logistic & $f(x)=\frac{L}{1+e^{-k(x-x_0)}}$\\ 
%\hline
%Sigmoid & $f(x)=\frac{1}{1+e^{-x}}$  \\
%\hline
%Hyperbolic tangent & $f(x)=\tanh(x)=\frac{2}{1+e^{-2x}}-1$  \\
%\hline
%ArcTan & $f(x)=\tan^{-1}(x)$ \\
%\hline
%Softsign & $f(x)=\frac{x}{1+|x|}$ \\
%\hline
%Exponential linear unit & $f(x)= \begin{cases} \alpha(e^x-1), & \text{if}\ \text{$x < 0$} \\ x, & \text{otherwise} \end{cases} $ \\
%\hline
%SoftPlus & $f(x)=\ln(1+e^x)$ \\
%\hline
%Sinusoid & $f(x)=\sin(x)$ \\
%\hline
%Gaussian & $f(x)=e^{-x^2}$ \\
%\hline
%\end{tabular}
%}
%\label{tbl:nn_acf}
%%\caj{Should it not be $x\leq 0$?}
%\end{table}
%
%
%The graphs for the activation functions presented in Table \ref{tbl:nn_acf} are
%shown in Figure \ref{fig:act_func}. The shapes of logistic and sigmoid functions look 
%similar, except the change in the bounds of the function. Similarly, from the perspective 
%of shapes, the hyperbolic tangent, arctan and softsign look similar with differences 
%in the slope of the curves and the bounds of the functions. 
%It needs to be noted that the graphs shown are 
%a simpler representation of their corresponding shapes, not drawn to the scale. 
%
%Activation functions are often the most computationally expensive  part in neural networks. 
%Reducing the implementation complexity of these functions often reduce the overall
%computational complexity. These activation functions could be implemented in 
%different manners, such as using look-up-tables (LUTs), BRAMs, utilizing CORDIC 
%algorithms to compute the hyperbolic and trigonometric functions \cite{Qian'06,Gisthuam'00}, and 
%approximate 
%computations \cite{Bian'14,Liu'08} such as piecewise-linear-approximations (PLAs). 
%
%
%\paragraph{Updating of Weights}
%\label{sec:update_nn}
%Weights in a neural network can be updated in multiple ways.
%One of the most widely used rule is the Delta rule \cite{Wiki_Delta}:
%%\caj{Let's add a reference here; perhaps to the wikipedia page: {https://en.wikipedia.org/wiki/Delta\_rule ?}}
%
%\begin{equation}
%\begin{aligned}\label{eq:wt_update}
%\Delta w_{ij}=\alpha (t_j-y_j)x_i
%\end{aligned}
%\end{equation}
%where $i$ indicates the index of input $x_i$ and $j$ represents the
%index of the $j$-th neuron with $t_j$ and $y_j$ as target and actual
%outputs. $\alpha$ denotes the learning rate.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% We have described the basic functionality of a neural network in 
%% Section \ref{subs:nn}. In addition to the number of neurons and the type of activation functions, various other architecture parameters influence the functionality and performance 
%% of the neural network. 
%We present some of the popular neural network 
%architectures for signal analysis, targeting resource constrained systems. 
%
%\subsubsection{Back Propagation Neural Network}
%\label{sec:bpnn}
%Back propagation means updating the weights in the network architecture. In Back propagation neural networks (BPNN) \cite{Marsland'09,Heerman'92,Gent'91,BPNN1,BPNN2}, 
%the input data is fed from the input layer to the hidden layer and then to the output layer. 
%However, the weights are updated in the reverse manner. One popular method to update the 
%weights of individual nodes is the Delta rule (eq. (\ref{eq:wt_update})). 
%The weights between the hidden layer and the output layer are 
%updated first based on the target outputs of the system, followed 
%by updating the weights between the hidden layer and the input layer.  
%The overall architecture is also termed popularly as feedforward neural network. 
%%\caj{Please give the formula that updates the weights based on the error.}
%
%\textbf{\textit{Example:}} In \cite{Asl'06}, a combination
%of linear and non-linear features of ECG, especially, heart-rate variability (HRV) is provided
%as input for feedforward ANN with back propagation for ECG classification. Time domain and frequency domain based nonlinear
%methods are applied in \cite{Asl'06} to extract the features of ECG and are fed to an ANN classifier
%for ECG arrhythmia detection. The NN architecture comprises of 11 inputs, one hidden layer with
%20 neurons and 5 outputs. This indicates that the implementation in \cite{Asl'06} can detect 
%and classify up to 5 arrhythmias. The paper claims that the implementation can be effective even when the 
%training dataset is small.
%% The output at each neuron is a real number in the  interval range [0, 1]. 
%This architecture utilizes the features of the ECG and 
%HRV metrics to 
%derive conclusions on arrhythmias, which makes the system prone to noise, unless the neural network itself  
%offsets the effects of noise. 
%
%
%\subsubsection{Elman Neural Network}
%Elman neural networks \cite{Deng'16,Lin'15} have explicit feedback 
%from the succeeding layer i.e., there exists a feedback from the 
%output layer to the hidden layer and from the hidden layer to the 
%input layer. It is a BPNN (as in Section \ref{sec:bpnn}) but 
%with explicit feedback from output layer to hidden layer. 
%The feedback provides the error, depending on the application. 
%For instance, when the neural network is used for 
%prediction, the prediction error is used as feedback signal. 
%As a result, the Elman neural network learns faster and more efficiently,
%even when the signal quality is poor. 
%However, inconsistent data such as random or noisy signals 
%lead to convergence issues. 
%
%\textbf{\textit{Example:}} An Elman neural network implementation for ECG anomaly detection is proposed in \cite{Mohamad'13}.
%In \cite{Mohamad'13}, for ECG anomaly detection,
%a three step process: pre-processing, processing and classification is followed. For pre-processing,
%median filter and moving average filters are used to remove high frequency noises, smooth the signal
%and eliminate the jagged edges. This is followed by principal component analysis for reducing the features
%to save the computation costs. The reduced feature set is provided as input to the Elman neural network,
%which is trained with the data. The results have shown a satisfactory results of more than 95\% accuracy.
%The major bottleneck in the Elman neural networks are the amount of 
%required memory resources, especially when the number of nodes and the 
%states to be utilized in the process are high. 
%
%\subsubsection{Block-based Neural Network}
%For an efficient hardware implementation, block-based neural networks (BbNN) \cite{Merchant'06,Kong'04,Moon'01}
%are often chosen. Their implementations can be seen as 2 dimensional arrays of blocks.
%Each block is a four input/output feed-forward neural network.
%The number of inputs and outputs are configurable.
%Each block connects to its neighboring blocks similar to
%a mesh network. The signal flow uniquely specifies the internal
%configuration of the block as well as the overall network structure.
%The number of inputs and outputs for different blocks do not have to be the same. 
%A feed-forward NN based BbNN can be seen as a data flow from the top block
%to the bottom block in a 2D array. A BbNN
%architecture with inputs provided at the top and outputs at the bottom
%is shown in Figure \ref{fig:trad_Bb}.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.5\textwidth]{pics/NNs_Bb} \\
%\caption{Block based neural network architecture}
%\label{fig:trad_Bb}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\textbf{\textit{Example:}} A BbNN with morphological features and temporal properties of ECG 
%i.e., Hermite expansion coefficients and RR intervals
%as inputs is proposed for ECG arrhythmia detection and classification 
%in \cite{Jewajinda'10}. However, in \cite{Jewajinda'10}, an online 
%updating mechanism for weights is incorporated.
%
%
%\subsubsection{Probabilistic Neural Networks}
%A probabilistic neural network (PNN) \cite{Perera'11,PNN1,PNN2} 
%is a feed forward neural network \cite{Marsland'09,Alpaydin'09} 
%which uses Bayesian statistics i.e., probabilistic evaluations 
%as in Section \ref{sec:bayesian_lr}, and Kernels to perform 
%pattern analysis. A PNN comprises of an input layer, a pattern layer, 
%a summation layer and an output layer.  
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.5\textwidth]{pics/pnn} \\
%\caption{Probabilistic Neural Network Architecture}
%\label{fig:trad_pnn}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%\textbf{\textit{Example:}}
%The input layer in the probabilistic neural networks 
%normalizes the raw input data, such that the range of input 
%becomes 0 to 1. For instance, consider a series $X=\{4,5,7,6,7\}$, 
%this could be normalized as $X_p=\{0.57,0.71,1.00,0.86,1.00\}$ 
%(all the values are divided by 7). However, it does not need to be divided by the maximum value in series, could also some other 
%function which will normalizes the input data to be in the range of 0 
%to 1, such as (\ref{eq:log_reg}). This normalized data will be sent 
%to other layers i.e., passed to pattern layer. 
%%\caj{what is normalized? The number of neurons in the input layer? Or the input signals to the input layer neurons?} 
%%and this is input is given to the 
%%pattern layer. 
%The pattern layer is built based on the number of 
%training samples i.e., for instance if for class A the network is 
%trained with 3 samples, one can see three nodes corresponding to 
%class A. As such, the number of 
%nodes in the pattern layer corresponds to the total number of 
%training samples. 
%In case of larger data sets, an optimal number of data sets 
%that cover most of the cases are considered and based on that the 
%number of nodes are formed. 
%%\cajb{Is this scalable to large training sets?} 
%The outputs of nodes that belong to a particular 
%class are summed up in the summation layer. In the output layer, 
%the summed up values received from the 
%summation layer for each class are compared and the class with 
%highest accumulated value is 
%voted as the class to which the input data belongs to. 
%
%% For instance, consider a simple case of differentiating 3 symbols 
%% i.e., 3 classes, as shown in Figure \ref{fig:trad_pnn}. 
%% The input is initially normalized. The nodes in the pattern layer 
%% are often built for each of the individual training samples. 
%% Further, the outputs from nodes in pattern 
%% layer that belongs to same class are summed (In this example, two training 
%% samples are provided for each class, hence 2 nodes for each class in
%% pattern layer, different colors inside the node indicate different 
%% class). In the
%% output layer, the summed values in the summation layer are compared and the class with the highest 
%% value is considered to be the class to which the input relates to.
%
%Probabilistic neural networks are more suitable for small scale and 
%medium scale input data based applications. On the other hand, for large 
%and (sometimes) even for medium scale data applications, the input 
%training data needs to be optimized. PNNs are widely used for object 
%recognition, pattern recognition, and so on, especially when the training 
%data set is smaller. However, PNNs are not preferred especially on 
%hardware constrained systems, as the number of nodes in the pattern layer 
%scales up proportionately with the training data sets. 
%
%%\caj{Please add a sentence about the suitability of this network for hardware implementation. It seems the network is very dynamic with large number of nodes for large training sets, which seems very difficult to accommodate in HW. On the other hand we write that we focus on resource constrained implementations.}
%
%
%\subsubsection{Wavelet Neural Networks}
%Wavelet neural networks \cite{Alexandridis'13,Chen'10,Pan'08,WNN1} 
%constitute a class of feed forward neural networks with 
%input, hidden and output 
%layers with backward propagation for updating the weights, 
%as in Section \ref{sec:bpnn}. 
%However, there is only one neuron in the output layer (Figure \ref{fig:trad_wnn}). 
%
%Wavelet neural networks make use of wavelet as an activation function. 
%Wavelets have the benefit of high compression ability as well as 
%an updating function that involves only a subset of coefficients. 
%Wavelet is a specific pattern or a mathematical function that is 
%intended to possess certain properties. Some of the widely used 
%wavelet functions are Gaussian derivation, second derivative of 
%Gaussian (also called ``Mexican Hat'') and Morlet wavelet. 
%In eq.~(\ref{eq:wnn}), a multi-dimensional wavelet function $\psi(...)$ is utilized.  
%Multidimensional wavelets are widely used, as they can preserve the 
%``universal approximation'' property
%%\caj{Can you briefly give an intuition of this property?}
%that characterizes neural networks 
%\cite{Alexandridis'13}. The universal approximation theorem says that the approximation 
%in the neural networks i.e., building the model happen as a result of neural network architecture rather than the 
%activation functions. The output of the wavelet neural network can be given as 
%follows
%\begin{equation}
%\begin{aligned}\label{eq:wnn}
%y=\sum_{i=1}^m x_iw_i^{[0]}+\sum_{j=1}^k w_j^{[2]}\prod_{i=1}^m\psi(\frac{x_i-w_{ijt}^{[1]}}{w_{ijd}^{[1]}}) +w_{k+1}^{[2]}
%\end{aligned}
%\end{equation}
%Here, $m$ represents the number of inputs, $k$ represents the number 
%of nodes in the hidden layer. The scaling factors (weights) between input 
%layer and output layer is given by $w_i^{[0]}$, $i=1,2,...,m$ and 
%the weights between hidden layer and the output layer is represented as 
%$w_j^{[2]}$, $j=1,2,...,k$. The weight vector between input and 
%hidden layer is given by $w_{ij}^{[1]}=(w_{ijt}^{[1]},w_{ijd}^{[1]})$, 
%$i=1,2,...,m; \ j=1,2,...,k$. Translation and dilation factors are 
%represented by $w_{ijt}^{[1]},w_{ijd}^{[1]}$ respectively. 
%For instance, the ``Mexican Hat'' wavelet function can be given as 
%\begin{equation}
%\begin{aligned}
%\psi(x)=(1-x^2)e^{-\frac{1}{2}x^2}
%\end{aligned}
%\end{equation}
%
%The main idea of the 
%wavelet neural networks is to adapt the wavelet basis in the 
%hidden layers to the training data.  A simple example is to adapt the 
%variance of the Gaussian function based on the inputs. When testing, 
%any input that does not satisfy the adapted variance can be seen as 
%an outlier to the trained data. 
%
%\textbf{\textit{Example:}} A wavelet neural network (WNN) is proposed in \cite{Ceylan'11} with wavelets 
%as the activation functions. This work use
%wavelet functions as activation functions in the hidden layer nodes. Morlet and Mexican
%hat wavelet functions are widely selected for experimenting, and it has been shown that an NN with Mexican hat wavelet
%function outperforms a Morlet activation function based NN, in terms of classification
%accuracy \cite{Ceylan'11}. In \cite{Ceylan'11}, ECG signals are first filtered using low-pass and high-pass
%filters. Further, R peaks are detected. The RR intervals are provided as inputs and
%training data for the NN. This work can classify bundle branch blocks (BBB) and normal beats.
%
%%In the hidden layer, the inputs are transformed into dilated and 
%%translated version of the \hl{mother wavelet} 
%%\cajb{What is the mother wavelet?} 
%%used in the nodes in 
%%hidden layer (each node in the hidden layer is also called a hidden unit). Finally, in the output layer, the 
%%approximation of target values are estimated. 
%%\caj{The main idea should be explained better.}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.45\textwidth]{pics/wnn} \\
%\caption{Feed-forward Wavelet Neural Network Architecture}
%\label{fig:trad_wnn}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Other Signal Analysis Approaches based on Machine Learning}
%In addition to shallow and deep neural networks there are other machine learning approaches 
%for signal analysis. We discuss some of the popular approaches.
%
%\subsubsection{Kernel based Time-series Analysis}
%
%Kernel methods \cite{Taylor'04,Bernhard'02} are another useful set of techniques for pattern analysis and recognition. In contrast to other described techniques, kernel methods
%make use of user-specified kernels, i.e., similarity functions
%over pairs of data points in a raw distribution.
%The main intention behind 
%having kernels is to have similar output for similar inputs. 
%
%One of the most widely used Kernel functions is the Radial Basis
%Function kernel (RBF, also known as Gaussian Kernel), given by
%\begin{equation}
%K(x,\mu)=e^{-\frac{\|x-\mu\|^2}{2\sigma^2}}
%\end{equation}
%where $x$ represents the variable $x$ at a particular 
%time instant and $\mu$ denotes the mean
%%\cajb{$x'$ denotes the mean? Why not use $\mu$?} 
%of the corresponding series $X$ with a 
%variance of $\sigma$. 
%One can see the Kernel as a simple function correlating with a sequence or a window in 
%a time-series result in detecting the patters, resulting in either detecting anomalies or 
%finding the desired patterns in the time-series. 
%%\caj{Can you give an example how the kernel is used for analyzing the times series signal?}
%
%Other popular functions include String kernels, Graph kernels,
%Fisher kernels and polynomial kernel. In a broader sense, the underlying 
%operation is to obtain the similarity metric (distance) of the 
%data to the Kernel. However, different kernels are more specific for 
%particular applications, for instance, String kernels are used when performing string or text matching, graph kernels to find the 
%similarity between graphs by calculating the inner products and 
%Fisher kernels for image recognition and classification purposes. 
%%\caj{Add a sentence indicating what are the main differences between different kernels. E.g. Is it a different distance metric, or?}
%
%Consider a simple example of detecting a pattern which resembles Gaussian distribution curve 
%%\cajb{What is a Gaussian pattern?} 
%in a series of data. Application of a RBF, i.e. multiplying the input 
%series with the RBF kernel will result in a maximum output near the 
%existence of the Gaussian pattern and lower values elsewhere. Based 
%on the output of the kernel, corresponding patterns are identified.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Kernels \cite{Hastie'08,Silverman'86} are generally considered to be 
%a measure of similarity in the sense that the kernel function $K({\bf X}, {\bf Y})$ takes a larger value if ${\bf X}$ and ${\bf Y}$ are 
%similar \cite{Alpaydin'09}. 
%%pre-defined functions \hl{using which the patterns in a 
%%data or series can be analyzed}.\cajb{This is weird formulation which I do not understand.} 
%%As defined in Section \ref{subs:kernel}, 
%Kernels are widely applied for problem solving scenarios such as pattern matching, and 
%text recognition. In the case of 
%line detection, a kernel is a model of a line and a correlation  
%over the input data series (a set of input data points) which produces a
%maximum correlation or a minimal Euclidean distance 
%or a dot product that
%indicates the presence of a line at those points
%\cite{Garcia'13,Alpaydin'09,Marsland'09,Cruz'04}. In a similar manner, 
%different kernels are employed to perform pattern analysis. 
%The type of kernel depends on the application. %A kernel can be 
%%some of the 
%%existing standard functions like Gaussian functions depending 
%%on the application. 
%
%\textbf{\textit{Example:}} For arrhythmia detection in ECG signals, a kernel can be 
%a user defined mathematical model of the QRS complex, as provided in \cite{Amiri'15}. 
%This QRS modeled kernel is used for pattern matching i.e., to match the 
%QRS of the incoming signal with the kernel. In case of any mismatch, the arrhythmia 
%will be signaled to the user. 
%In case of classification, Kernel based optimization can be seen as 
%a convex optimization problem.
%
%\paragraph{Different Kernels}
%A variety of pre-defined standard Kernels exist and each of them 
%are utilized depending on the application. A few of the commonly 
%used Kernels are listed below. 
%
%\begin{table}[ht]
%\centering
%\caption{Common Kernel Functions}
%%\scalebox{1}{
%\begin{tabular}{|l|l|}
%\hline
%Name & Formula \\
%\hline
%\hline
%Uniform & $K(x)= \begin{cases} c, & \text{if}\ |x|\leq a \\ 0, & \text{otherwise} \end{cases} $   \\
%\hline
%Triangular & $K(x)= \begin{cases} (c-|x|), & \text{if}\ x \leq c \\ 1, & \text{otherwise} \end{cases} $  \\
%\hline
%Gaussian & $K(x)=\frac{1}{\sqrt{2\pi}}e^{-\frac{x^2}{2}}$ \\
%\hline
%Logistic & $K(x)=\frac{1}{e^x+2+e^{-x}}$  \\
%\hline
%Sigmoid & $K(x)=\frac{2}{\pi}\frac{1}{e^x+e^{-x}}$ \\
%\hline
%String$^1$ & $K({\bf X})= \sum_{i:u=s_i} \lambda^{l(i)}$ \\
%\hline
%\multirow{2}{*}{Fisher Score$^2$} & $K({\bf X}_i, {\bf X}_j)= U_{{\bf X}_i}^TI^{-1} U_{{\bf X}_j}$\\
% & $U_{{\bf X}} = \nabla_\theta log P({\bf X}|\theta) $  \\
%\hline
%Polynomial$^3$ & $K({\bf X},{\bf Y})=({\bf X}^T{\bf Y}+c)^d$ \\
%\hline
%Radial Basis Function & $K({\bf X},{\bf Y})=exp(-\frac{||{\bf X}-{\bf Y}||^2}{2\sigma^2})$  \\
%\hline
%\end{tabular}\\[1ex]
%\raggedright
%$^1$ $i$ represents the string index, ${\bf X}$ is the string with substring $u$ of length $n$, 
%$s$ represents the string with which the input is matched; 
%parameter $\lambda$ can be set to any value between 0 
%and 1.\\ 
%$^2$ ${\bf X}_i$, ${\bf X}_j$ are two matrices, $I$ is the fisher information matrix, $\theta$ represents the set of parameters and 
%$P({\bf X}|\theta)$ is the likelihood of the probabilistic model. \\ 
%$^3$ $d$ is degree of polynomial. \\
%\label{tbl:kernels}
%\end{table}
%
%In Table \ref{tbl:kernels}, $c$ and $a$ are constants; $x$ is a scalar 
%and $K()$ represents the kernel function. 
%Letters in bold (such as ${\bf X},{\bf Y}$) represent Vectors, 
%unless otherwise specified. % otherwise.
%%\todo{References for each of the kernels}
%Fisher Kernels \cite{Zhu'08,Roth'06} are mainly employed for image classification and
%retrieval applications. Graph kernels \cite{Kim'14,Bleik'13} 
%compute inner products on graphs. Graph kernels are seen as 
%functions that measure the similarity between a pair of graphs. 
%Polynomial kernels \cite{Yaman'13,Meijering'99} are equivalent to polynomial regression models 
%but without any learning or updating. For  
%Radial Basis Function (RBF) Kernel (also called as Gaussian kernel) 
%\cite{Wang2'16,Jayasumana'15}, 
%$\sigma^2$ denotes the allowed variance as determined by the user. 
%A RBF kernel is an interpretation of similarity measure between 
%input vectors, with 1 denoting high similarity. 
%Kernel based recognition are widely employed in the field of image recognition 
%and classification.  
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
%\subsubsection{Support Vector Machines}
%
%Support Vector Machines (SVMs) \cite{Marsland'09,Steinwart'08,Vapnik'06} are used for classification and regression analysis.
%An SVM builds a model based on the input data with labels such
%that it could be classified as clear as possible (as provided in labels). 
%Here the label indicates the class or a group to which the 
%input data belongs to. For example, consider an ECG signal, 
%here the label could be name of the  
%component at a particular time instant. 
%%\cajb{What is a label? An example would illuminate the technique.}
%Every new input is mapped to the corresponding category.
%%SVMs make use of the Kernels to build the models and
%%mapping the input data to the category.
%%\cpd{Kernels are used to see if the data could be modeled as standard kernels based on the distance, but most often models are derived from data.}
%SVMs operate on vectors rather than individual
%points, making them robust. For estimating the
%distances, SVMs make use of dot products.
%%\caj{Isn't a kernel function used as distance metric?}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.55\textwidth]{pics/svm} \\
%\caption{Binary classification with (a) other classifiers; (b) SVM}
%\label{fig:svm}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%In SVMs, the objective is to find a hyper-plane that could separate 
%the positive and negative samples (considering a simple binary classification) with a clear boundary. Let us assume a sample space with 
%vector $w$ being normal to the hyper-plane that separates the data set, and a constant $b$. Then the following equation has to be satisfied
%\[
%t_i(w^T\cdot  x_i+b)\geq 1 \\ 
%\]
%where $x_i$ is a sample, and $t_i$ is the 
%%\caj{what is the target output?} 
%target output i.e., the class to which it should belong. $t_i = +$1 for the sample belonging to positive 
%class and $t_i=-1$ for the sample belonging to negative class. 
%%\caj{What is a positive sample and what is a negative sample?}
%
%The width of the hyper-plane is given by 
%
%\[
%max(\frac{1}{\|w\|})
%\]
%where $w$ represents the normal vector to the hyper-plane.
%
%%\caj{What is "max."? and what is $w$? If max is the Maximum function it should be written as $\max(\frac{1}{\|w\|})$}
%
%Considering all this, it boils down to optimizing the following equations which 
%could be performed using Karush-Kuhn-Tucker (KKT) conditions \cite{Boyd'04}. %\cajb{Add reference.} 
%\begin{equation}
%\begin{aligned}\label{eq:svm}
%\lambda_i(1-t_i(w^T\cdot x_i+b)) & = 0 \\
%1-t_i(w^T \cdot x_i+b) & \leq 0 \\ 
%\lambda_i & \geq 0
%\end{aligned}
%\end{equation}
%where $\lambda_i$ is a Lagrange multiplier. 
%%\cajb{Is the . in the equations (12) the Dot-product? It should be written as $\cdot$.}
%
%The main objective is to find $w$ and $b$, such that for any sample, 
%the classification can be carried out. 
%
%
%
%A simple example, explaining this SVM method is shown in Figure \ref{fig:svm}. 
%The goal is to perform classification of new input 
%based on the existing data. The positive samples are indicated by circles 
%and negative with squares. We first find the normal vector $w$ to the 
%median of the hyper-plane and the width of the hyper-plane. 
%Further, the hyper-plane is formed and the classification can be 
%easily performed by calculating the distance of the sample to the plane, 
%as given by constraint 1 in eq.~(\ref{eq:svm}). 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Support vector machines (SVMs) \cite{Xue'11,SVM1,SVM2} are employed in classification
%applications. The main objective of SVM is to compute the 
%hyper-plane based on KKT conditions as given in eq.~(\ref{eq:svm}). 
%The basic process of SVM starts with 
%training of labeled input data 
%%to basically data along with the labels 
%%\cajb{Not understandable!} 
%(labels represent the class to which the data belongs). 
%Further, based on the training data, 
%the normal vector $w$ is calculated. Once the normal vector is obtained, 
%the position of new input data (test data) relative to the obtained 
%hyper-plane has to be computed and based on the 
%relative position, the 
%class of the new input is determined. 
%
%%\subsection{Genetic Algorithms}
%%\begin{itemize}
%%\item How to use Genetic Algorithms for signal analysis
%%\item Complexity, advantages and limitations
%%\end{itemize}
%Consider a simple case of binary classification i.e., 
%the input data has two classes. A hyper-plane will 
%be formed in between those two classes. 
%Class A is on the left side of hyper-plane and 
%class B to the right side, similar to that in 
%Figure \ref{fig:svm}. Any new input data 
%whose distance is negative i.e., left side 
%of the hyper-plane belongs to class A and the 
%input data whose distance to the hyper-plane is 
%positive belongs to class B.
%
%\textbf{\textit{Example:}} Similar to neural networks, ECG morphological features can also be used as an input for 
%arrhythmia detection for SVMs. An ECG classification method based on dynamics and the morphological features is presented in
%\cite{Ye'12}. It applies wavelet transform and independent component analysis (ICA)
%separately to extract the morphological features. Additionally, RR interval information is
%utilized to compute dynamic information. All this information together is provided to SVM
%with radial basis function (RBF) to perform classification.
%
%
%
%\subsection{Deep Learning based Approaches}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.55\textwidth]{pics/autoencoders} \\
%\caption{(a) A simple deep learning neural network; (b) a 3-stage auto encoder.}
%\label{fig:autoencoder}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
%Previously presented techniques such as 
%neural networks, SVMs, and kernels are efficient as long as 
%the data set is small and has low levels of noise. But, the presence of 
%noise and large data sets  adversely affect the 
%performance of traditional machine learning techniques. 
%Deep learning has been introduced to address these issues.
%
%Deep learning \cite{Goodfellow'16} can be seen as an of extension traditional machine learning
%with abstractions and processing at multiple levels. Deep neural networks are an extended version of neural 
%networks with an increased number of processing layers (hidden layers), as shown in Figure \ref{fig:autoencoder}(a). 
%Different deep learning architectures \cite{Goodfellow'16,Heaton'15} including convolutional 
%neural networks \cite{Chen'16,Lawrence'97}, recursive neural networks \cite{Bianchini'01,Williams'89}, deep stacking networks \cite{Nie'14,Deng'13} 
%%\cajb{Add reference. Either a good reference for each of those types, or one reference that covers all types well.}
%and so  on are introduced depending on the application, with 
%architecture, i.e., the connectivity between and within layers, as the main differentiating factor. 
%
%
%
%
%For instance, deep stacking networks are a straight forward extension of traditional 3-layer networks. They contain a stack of hidden layers with the outputs of one layer forming the inputs to the succeeding. As such, the weights for the 
%individual hidden layer networks are calculated. Stacked auto-encoders have a set of single 
%hidden layer neural network providing inputs to the hidden layers in a 
%succeeding neural network, as shown in Figure \ref{fig:autoencoder}(b). 
%This hierarchical processing has the 
%advantages of abstracting the input data at different 
%levels. 
%
%As can be observed that the main principle of deep learning 
%is abstraction of input data in a hierarchical manner. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Convolutional Neural Network}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.45\textwidth]{pics/NNs_Conv} (a) \label{fig:trad_Conv}
%\includegraphics[height=0.45\textwidth]{pics/RNN}  (b) \label{fig:RNN}
%\caption{(a) Convolutional neural network architecture; (b) Recurrent neural network architecture}
%\label{fig:trad_Conv1}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%A Convolutional Neural Network (CNN) is a variant of feed-forward neural networks with deep-learning \cite{Lee'16,Li'16,Zhou'15,Ikhwantri'15}.
%The input provided for CNN will be tiled into several smaller segments, with two
%successive segments having an overlap. The amount of overlap can be 
%modified depending on the application and the input data size. 
%Each input neuron/node will be fed with this
%smaller segment of input data and convoluted with a mask. 
%A mask is a filter with which the convolution is performed. 
%Consider an object recognition example, the mask could be a small 
%matrix that represents a subset of the image. The main necessity of 
%masks is for extracting different levels of features in image processing 
%applications. 
%%\caj{The term "mask" should be explained better. Is it an activation function? Or are activation functions used to realize a particular mask? If so, how? Can you give an example how activation functions realize a particular mask? What is the purpose of a mask?} 
%A similar set of parallel layers are arranged with each layer having 
%specific masks i.e., different filters. 
%Further, the output from each layer is transferred to the next layer.
%Thus, the whole CNN comprises a set of parallel layers arranged 
%in a serial manner. 
%The output of each node is smaller in dimension compared to the input.
%%A few number of different activation functions are used.
%%A parallel set of such layers will be available at next layer.
%This dimension reduction continues. Finally, this reduced dimensional output
%is provided to a fully connected network i.e., a traditional neural network
%for final processing.
%CNN finds applications for multi-dimensional data classification and object recognition.
%
%A convolution based neural network implementation is shown in
%Figure \ref{fig:trad_Conv1}(a). The input is convoluted with different masks
%at the beginning states and the convolution formed with different masks are
%concatenated. The yellow color rectangle represents the mask or 
%the activation function used in the layer. This procedure is 
%repeated and the output is finally obtained
%by providing the convoluted results to a fully connected neural network.
%In order to reduce the dimension, pooling stages are 
%used in between. For example, a moving average 
%filter applied to reduce the size of the data can 
%be seen as a Pooling stage. 
%CNNs are widely used in image processing applications where the amount of data 
%to be processed is often large. 
%
%\textbf{\textit{Example:}}
%In \cite{Huang'16}, a fine-grained vehicle recognition via deep Convolutional Neural Network (CNN) 
%is proposed. Vehicle and the corresponding parts are localized with the help 
%of Region-based Convolutional Neural Networks (RCNN) and their corresponding 
%features from a set of pre-trained CNNs are aggregated to train an SVM classifier. 
%Further, based on the trained CNNs and SVMs, a fine-grained vehicle classification is 
%performed. CNNs often suffer from large training time and vast amount of 
%resource requirements. 
%
%\subsubsection{Recurrent Neural Networks}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\begin{figure}[!t]
%%\centering
%%\includegraphics[height=0.55\textwidth]{pics/RNN} \\
%%\caption{Recurrent neural network architecture}
%%\label{fig:RNN}
%%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%Recurrent neural networks (RNNs) \cite{Chen2'16,RNN1,RNN2} are deep neural networks 
%with the notion of memory, hence, they remember the previous state of the 
%network and can be be seen as a class of Elman networks. The state of a node is defined by the input weights 
%of the neuron. An RNN is modeled as 
%\begin{equation}
%\begin{aligned}
%h_t=f(h_{t-1},x_t)
%\end{aligned}
%\end{equation}
%where $h_t$ represents the state of the neural network at time $t$, $x_t$ is the input at time $t$. 
%$f(..)$ represents the next-state function. The state of a 
%neural network is defined as the weights in the 
%network.
%
%Figure \ref{fig:trad_Conv1}(b) illustrates the RNN. The X-axis represents the 
%notion of time and Y axis represent the network. Each block can be 
%seen as a layer (or several layers) in the network i.e. a set of nodes. 
%The current state and the previous state of the hidden layers 
%determines the output at a time instant. In the following equation, 
%the hyperbolic tangent is considered as the activation function of 
%the hidden layer node and it takes the product of the previous state ($h_{t-1}$)
%and a weight vector
%%\cajb{What is the "weight for states"?? It is not explained!} 
%($W_{hh}$) along with the input $x_t$ and the 
%weight vector $W_{xh}$. Based on the current state and the output 
%weight vector $W_{hy}$ the output $y_t$ is determined.
%%\cajb{Use a different font for tanh!!}
%\begin{equation}
%\begin{aligned}
%h_t=& \tanh(W_{hh}h_{t-1}+W_{xh}x_t) \\
%y_t=& W_{hy}h_t
%\end{aligned}
%\end{equation}
%
%Note, that the number of states that are considered 
%to determine $h_t$ is variable. In this example, only the previous state ($h_{t-1}$) is considered, but more history states $h_{t-1}\cdots h_{t-k}$ could be used. 
%If a large number of previous states is considered, the system may require significant amount of memory. 
%
%In general, the current state $h_t$ with $tanh()$ activation functions 
%can be given as 
%%\cajb{Is tanhW a function? Is this consistent with eq. (24)?}
%%\cpd{Tanh is the function W is a vector and so does the other two}
%\begin{equation}
%h_t^l=\tanh \left(W^l \begin{pmatrix}
%h_t^{l-i}\\ 
%h_{t-1}^{l}
%\end{pmatrix}\right)
%\end{equation}
%where $l$ represents the hidden layer number. $W^l$ is the weight vector of 
%the current layer ($W^l$ can be seen as $[W_{xh} W_{hh}]$, for this case,
%the $h_{t}^{l-1}$ is the input $x_t$, as only one hidden layer is used). This indicates that 
%the current state is derived based on the previous state of the current 
%layer and the current state of the one layer below the hidden layer in the hierarchy. It is not 
%necessary to consider the state of lower level hidden layers of all the times, which, however, depends on the application. 
%
%RNNs are employed widely in applications like image captioning,
%predicting strings, predicting words or characters, 
%language translation, with training set comprised of few words or characters,  
%\cite{Chien'16,Chen2'16} and so on.
%%\caj{This paragraph has several grammar errors and is not understandable!}
%
%\textbf{\textit{Example:}} A skin detection from images for dermatology applications 
%with a combination of CNN and RNN is proposed in \cite{Zuo'17}. 
%CNN layers are trained to capture the generic local features from the images, while 
%the RNN layers model the semantic contextual dependencies in images. As such, based on 
%the generic and contextual features extracted from the images, skin detection with 
%good accuracy, even in complex background situations is achieved. 
%
%\subsubsection{Long Short-Term Memory (LSTM)}
%Long short term-memory \cite{Palangi'16,Hochreiter'97,RNN1} is an extension of RNNs. 
%The main issue in RNNs is the need for large storage to remember a 
%large number of states and computations performed on each of the 
%previous states. As a remedy, LSTM is activated with 
%forget and remember gates. During the training the network evaluates the 
%impact of the previous and current states. The current input 
%and the states, that have impact on the output are 
%kept while the rest is discarded. 
%% It can be mathematically given as 
%% \begin{equation}\label{eq:lstm}
%% \begin{aligned}
%% \begin{pmatrix}
%% i \\
%% f \\
%% o \\
%% g
%% \end{pmatrix} & = \begin{pmatrix}
%% sigm\\ 
%% sigm\\ 
%% sigm\\ 
%% tanh\\ 
%% \end{pmatrix} W^l
%% \begin{pmatrix}
%% h_t^{l-i}\\ 
%% h_{t-1}^{l}
%% \end{pmatrix} \\ 
%% c_t^l & =f \bigodot c_{t-1}^l+i \bigodot g \\ 
%% h_t^l & =o \bigodot tanh(c_t^l)
%% \end{aligned}
%% \end{equation}
%LSTMs are very popular in language processing.
%Similar to RNNs, LSTMs combined with CNNs are employed for 
%image captioning \cite{LSTM1} purposes. 
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsection{Hybrid Approaches}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Till now we have seen some of the individual approaches that are used 
%for classification and/or prediction purposes. However, there exist approaches
%that use combinations of techniques~\cite{Pazzouki'16,Lee'08,Romsdorfer'09,Alpaydin'09,Marsland'09,Ceylan'07}. The most common and widely used two hybrid techniques are 
%discussed below. 
%The following hybrid approaches are explained with the aid of examples. 
%
%
%\subsubsection{RBF based Neural Networks}
%Radial basis functions (RBF) have proven their efficiency in
%many applications such as predictions, classifications, approximations,
%system controls and many others
%\cite{Pazzouki'16,Lee'08,Romsdorfer'09,Alpaydin'09,Marsland'09}. 
%\cite{Karayiannis'97} proposes a neural network 
%with RBF as activation functions. Similar to traditional neural networks,
%the architecture consists of three kinds of layers.
%However, the activation functions
%in the hidden layers use RBF, and the 
%output layer simply can be seen as the linear
%combination of outputs from the last hidden layer i.e., RBFs and
%the neuron parameters such as bias.
%Different applications of this hybrid technique can be seen as 
%fault detection \cite{Li2'16,Meng'10}, control optimization \cite{Yali'08}, and so on. 
%
%\subsubsection{Weighted Distance based Neural Networks}
%Weighted distance based neural networks \cite{Romsdorfer'09} 
%have a similar architecture of a 
%traditional neural network. However, the activation functions make 
%use of the weighted distance (Euclidean distance) metric to 
%processes the data and provide the output. This kind of neural networks 
%are resource constrained and can be utilized for lightweight 
%applications such as pattern recognition on small scale data \cite{Alpaydin'09}. A weighted distance based neural network for pattern recognition is proposed in \cite{Alpaydin'09}.  
%This could also be utilized for finding anomalies in time series 
%like ECGs, with training data of features like R-R interval 
%distances, QRS morphology and so on. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Other Techniques}
%In addition to above discussed approaches, there exists approaches  
%such as rule-based classifiers (JOne, JRip, J48), decision tree approaches, 
%Ensemble learning based approaches, and so on. Some of these techniques 
%are lightweight compared to the neural networks, but have lower accuracy 
%in terms of classification and analysis \cite{Khaswneh'18}. Similarly, 
%Ensemble learning can be seen as a mixture of classifiers, but is costly 
%in terms of number of computations, power, and area. However, ensemble learning 
%is useful when the amount of signal characteristics that can be used 
%for analysis is small in number \cite{Khaswneh'18}. In the case of classification 
%of patterns or data in time-series signals, techniques such as clustering are widely employed. 
%Similarly, to detect the repeating patterns, techniques such as Motif discovery 
%are useful. 
%
%\subsection{Discussion and Analysis regarding Techniques for Time-series Analysis}
%
%In the previous subsections, we presented different time-series analysis 
%techniques ranging from various stochastic based techniques to some of the 
%sophisticated machine learning methodologies. Based on the techniques and their 
%characteristics, we target to provide a comprehensive analysis in terms of 
%different techniques and its suitability for various applications and 
%data types in Table \ref{tab:tech_appl}. It needs to be noted that the dimensionality 
%refers to number of independent variables or number of channels depending on the 
%application. For instance, in a 12-lead ECG signal the number of channels are 
%12 which is referred to as dimension in Table \ref{tab:tech_appl}. It needs to be noted 
%that the analysis in Table \ref{tab:tech_appl} is based on the technique and suitability, and 
%the hardware suitability and analysis will be discussed in the next section. 
%
%\begin{table}[!htb] \small
%\caption{Machine Learning Techniques and their suitability to applications}\label{tab:tech_appl}
%\scalebox{0.9}{
%\begin{tabular}{|p{2.5cm}|p{4cm}|p{7.5cm}|}
%%	\begin{tabular}{|p{2cm}||p{2cm}||p{3.5cm}|}
%\hline
%Method & Purpose & Note \\
%\hline
%Time-domain characteristics	& Prediction, anomaly detection	& Low complex, but not efficient for large dimensional data, has impact of noise\\
%\hline
%Frequency-domain characteristics	& classification, anomaly detection, DSP applications (such as voice processing) & widely used in DSP, noise impact is less, suitable for small datasets\\
%\hline
%MARS & Prediction, Data mining & Beneficial for (limited) non-linear data modeling, suitable for small dimensional time-series \\
%\hline
%ARMA & Prediction, Data mining & Time series prediction even considering multiple independent variables, efficient even under the impact of noise, but can lead to over fitting \\ 
%\hline
%Bayesian Regression & Classification & Good for data classification, evaluate the model and prediction\\ 
%\hline
%Logistic Regression & Binary classification & Suitable for signals with correlations \\ 
%\hline
%Neural Networks & Prediction, classification & Suitable for data with large and small dimensions; complex in terms of processing and high processing overhead\\ 
%\hline
%Kernel-based analysis & Pattern matching & To determine existence of a pattern; limited applicability \\ 
%\hline
%Support vector machines & Classification, Prediction & Relatively slower compared to stochastic techniques, and complex, but efficient\\
%\hline 
%Deep learning & Prediction, classification & Efficient for large dimensional data, generally an overkill for time series analysis \\ 
%\hline
%Clustering & Classification & Unsupervised, and highly dependent on the number of clusters chosen\\ 
%\hline
%Motif discovery & Pattern detection & Detect sub-pattern(s) in a time-series\\ 
%\hline
%\end{tabular}
%}
%\end{table}
%
%% \caj{I think here we need a short discussion on how the different methods are applicable to time series signal analysis. Perhaps we can categorize the different methods, e.g. with respect to 
%
%% - A large data set/small data set for learning
%
%% - categorization tasks
%
%% - on-line learning and abstraction
%
%% - approximation and prediction tasks
%
%% - noise resilient
%
%% - resource efficient (for embedded HW/SW implementations)
%
%% What do you think?
%% }
%
%% \begin{itemize}
%% \item Fuzzy neural networks 
%% \item Tree-based methods 
%% \end{itemize}
%

\section{Hardware Implementation}
\label{sec:hw_impl}
Hardware implementation of the presented time-series analysis techniques and their variants, 
especially on FPGAs and ASICs, are discussed in this section. FPGAs are often preferred over other hardware platforms due to their reconfigurability and reprogrammability. 
Though existing hardware implementations of different 
signal analysis techniques are presented, special attention is 
provided to neural network (NN) implementations, 
due to their better learning capabilities, broader application domain 
and higher achievable accuracy. 
The key advantages for implementation in FPGAs are less time to market, 
easy to reprogram, re-deploy and test, cost of the devices compared to ASICs,  
and the ease in designing compared to other options. 

Parallelism, modularity, and dynamic adaptation are three 
essential features that make neural networks 
efficient. 
Neural networks can be implemented using digital or analog systems. 
Due to the advantages such as higher accuracy, 
better repeatability, low noise sensitivity, better 
testability and flexibility, digital implementation 
is often preferred over analog implementation \cite{Indiveri'94}. 
These implementations can be done on digital 
signal processors (DSPs), FPGAs, or ASICs. 
DSPs are sequential in 
nature~\cite{Jung'07}, hence cannot preserve the parallel implementation notion of NNs, which is an important aspect of NNs. The array of DSPs can help implement neural networks but are costly in terms of area. 
%\caj{Is this a good argument? What about arrays of DSP cores (multiply-accumulate blocks)? Would they be suitable for NN implementations? }
ASIC implementations 
limit the flexibility. FPGA based implementations are 
highly suitable for NNs. FPGAs support modular designs, 
parallel computing and are reconfigurable. 
%An extension of neural networks in terms of hierarchy results in deep neural networks. 
To implement deep neural networks, especially convolutional neural networks (CNNs), which constitute one of the 
widely employed techniques for processing large amounts of input data, 
different implementation 
parameters are chosen based on the 
the size of input data, such as  
stride (overlap between inputs to two consecutive input nodes in CNN), 
depth, etc.
Further, the corresponding masks and sizes 
have to be chosen. 

The hardware implementation 
of the masks will be done using filters. Once the activation 
functions and the number of hidden layers are decided, 
the performance evaluation will be first performed 
in software (say Matlab or Python), and once the results are 
satisfactory, the corresponding neural network will be 
built-in hardware using simple neuron structures. 
However, the weights are often 
obtained by training performed in software. 
Due to longer deployment times of CNNs on FPGAs, special design 
flow techniques are as well provided \cite{Qiu'16}.


% \begin{table}
% \tableSpace
% 	\label{tab:tech_appl}
% 	\centering
% 	\caption{Machine Learning Techniques and their suitability to applications}

% \scalebox{1}{
% 		\begin{tabular}{|p{1.5cm}||p{2.5cm}||p{4.3cm}|}
% 			\hline
% 			Method & Purpose & Note \\
% 			\hline
% 			Time-domain characteristics	& Prediction, anomaly detection	& Low complex, but not efficient for large dimensional data, has impact of noise\\
% 			\hline
% 			Frequency-domain characteristics	& classification, anomaly detection, DSP applications (such as voice processing) & widely used in DSP, noise impact is less, suitable for small datasets\\
% 			\hline
% 			MARS & Prediction, Data mining & Beneficial for (limited) non-linear data modeling, suitable for small dimensional time-series \\
% 			\hline
% 			ARMA & Prediction, Data mining & Time-series prediction even considering multiple independent variables, efficient even under the impact of noise, but can lead to over fitting \\ 
% 			\hline
% 			Bayesian Regression & Classification & Good for data classification, evaluate the model and prediction\\ 
% 			\hline
% 			Logistic Regression & Binary classification & Suitable for signals with correlations \\ 
% 			\hline
% 			Neural Networks & Prediction, classification & Suitable for data with large and small dimensions; complex in terms of processing and high processing overhead\\ 
% 			\hline
% 			Kernel-based analysis & Pattern matching & To determine existence of a pattern; limited applicability \\ 
% 			\hline
% 			Support vector machines & Classification, Prediction & Relatively slower compared to stochastic techniques, and complex, but efficient\\
% 			\hline 
% 			Deep learning & Prediction, classification & Efficient for large dimensional data, generally an overkill for time series-analysis \\ 
% 			\hline
% 			Clustering & Classification & Unsupervised, and highly dependent on the number of clusters chosen\\ 
% 			\hline
% 			Motif discovery & Pattern detection & Detect sub-pattern(s) in a time-series
% 			\hline
% \end{tabular}}
% \tableSpace
% \end{table}


\subsection{Hurdles in Implementation}

The design of ASIC hardware for machine learning or any generic applications requires a large amount of time, IPs, or different vendors' tools. This might not be viable for many research institutes and small-scale industries. Hence, FPGA based designs are widely deployed. In small-scale industries and large enterprises such as Google, IBM, Intel is deploying FPGAs for different purposes. We present some of the significant hurdles in implementing 
the above discussed time-series techniques in FPGAs, focusing on neural network (NN) implementation due to its wide adaptability and applicability. 

%\caj{Do we focus exclusively on FPGA implementation? It could be okay but we have to motivate it a bit more.}

The main challenges in FPGA based implementation are 
the limited available resources, i.e., the hardware on 
FPGAs are limited \cite{ Muthuramalingam'08,Reyneri'03}, and the NNs are `multiplication-rich.' Rounding of floating-point weights' numbers can significantly save resources while trading off accuracy. Which trade-off should be chosen depends highly on the requirements.

One of the main major hurdles in NN implementations on FPGA is the difficulty to select the
design parameters such as the number of hidden layers (in case of deep learning),
activation functions for each layer, the number of neurons, connectivity between layers, the precision of data, and so on. 
These parameters affect the performance as well as hardware resources. For example, many hidden layers might improve accuracy but might not fit on a given FPGA. 
Similarly, the use of different activation functions results in varying accuracy levels for various applications; hence, the activation function needs to be selected carefully. Data representation with higher precision may produce an accurate result, but it demands large bandwidth and more resources on the downside. 
Further, a direct mapping of deep learning algorithms from software to hardware
often results in inefficient resource usage and high latency, large memory requirements, 
and high power consumption. 
Hence there is a need to find suitable implementation 
parameters to achieve 
best performance. 

% \subsection{Evaluation Parameters}
% As evaluation parameters, we use accuracy (fraction of correct predictions, classifications and recognition),
% %\cajb{Correct?} 
% %\cpd{Yes, I added recognition}
% latency, 
% power consumption, and
% hardware resource usage (area, number of LUTs, registers, 
% RAMs, and other components). In the course of this project, 
% we will study the trade-offs of these parameters for hardware implementations and accelerations of signal prediction and categorization algorithms.


\subsection{Existing Hardware Implementations} 
%Here, we present the hardware implementations of 
%different signal analysis techniques, application for which it 
%is used, evaluation metrics (if provided). 
%for that particular implementation. 

In the following, we present some of the existing hardware implementations of signal processing techniques
%ranging from statistical metric based analysis to deep neural networks 
on FPGAs and ASICs for various applications.  
The practical resource usage and performance numbers offer some understanding of which techniques are suitable. They provide hints for a room for improvement and the possibility of developing hybrid techniques. We have presented the hardware implementation details for each broad category of techniques discussed previously in Tables \ref{tbl:hw_stat}, \ref{tbl:hw-nn}, \ref{tbl:hw_reg}, \ref{tbl:hw-dl} and \ref{tbl:hw-svm} for signal analysis algorithms based on statistical parameters, implementations of neural networks, regression techniques, deep learning, and support vector machines, respectively. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[!htb]
% \caption{Hardware implementations of signal analysis algorithms based on  statistical parameters}
% \label{tbl:hw_stat}
% \centering
% \scalebox{0.86}{
% \begin{tabular}{|p{2.1cm}|p{4cm}|p{2cm}|}
% % \begin{tabular}{|p{4cm}|p{7cm}|p{3cm}|}
% \hline
% Technique & Implementation Details & Note \\
% \hline
% Periodicity (1998) \cite{Weber'98} & Periodicity based inference detection in radio astronomy applications & Flex 10K50 FPGA - 50k logic gates   \\
% %     &   & \\
% %     & Flex 10K50 FPGA - 50k logic gates & \\ 
%      % In radio astronomy 
% \hline
% Autocorrelation (2003) \cite{Hsueh'15}& Power supply noise analyzer based on autocorrelation function   & Accuracy $\sim$ 1mV \\
% %  & & \\ 
% \hline
% Correlation (2003) \cite{Mohammad'03} & QRS Correlation for ECG Analysis & - \\
% % No performance metrics given, it just uses a QRS template for matching 
% % input sequence, but none of the performance metrics are listed 
% \hline
% Mean (2008)\cite{Shukla'08}  & Amplitude thresholding based on mean of previous 8 QRS amplitudes for QRS detection & Accuracy $>$96\% \\ 
% \hline
% Spectrum Analysis (2004) \cite{Goldberg'04} & Periodicity analysis and correlation & power $<$1$\mu$W\\
% \hline
% Spectrum analysis (2015) \cite{Hsueh'15} & Energy spectrum analyzed in different frequency bands for noise filtering & \\
% \hline
% Wavelet detector (2006) \cite{Hoang'06} & QRS detection in ECG based on wavelet transform & ASIC - 318.4nW (0.18$\mu$m node) \\
% \hline
% Wavelet Fuzzy network (1998) \cite{Nambakhsh'08}& TDM filter with Wavelet transform for QRS detection and Fuzzy network for classification& Accuracy - 92\%\\ 
% \hline
% \end{tabular}
% } \vspace{-1.6em}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[!htb]
% \centering
% \caption{Hardware Implementation of Neural Network}
% \scalebox{0.86}{
% \begin{tabular}{|p{2.1cm}|p{4cm}|p{2cm}|}
% % \begin{tabular}{|p{4cm}|p{7cm}|p{4cm}|}
% %	\begin{tabular}{|p{2cm}|p{4cm}|p{2cm}|}
% \hline
% Technique & Implementation Details & Note \\
% \hline
% Feedforward NN (2019) \cite{FFNN_1} & 
% FPGA-based system to detect epilepsy in real-time with neural network & Hardware detection accuracy is 89.88\% \\

% \hline

% Feedforward NN (2019) \cite{FFNN_2} & 
% EEG classification scheme based on neural network implemented on FPGA & Hardware implementation realized using Artix-7, Kintex35 and Kintex115\\

% \hline

% Spiking NN  
% (2019) \cite{FFNN_3} & 
% Provides a scalable and tunable platform based on NN to facilitate the study of neurological diseases & Xilinx Kintex-7  XC7k325tffg900\\


% \hline
% Feedforward NN (2015) \cite{Geoffroy'15} & Identify true line of response (LOR) for multiple event detection in positron emission tomography (PET) & Virtex-2 FPGA, $\sim$39.7\% better detection efficiency compared to others\\
% \hline
% Feedforward NN (2010) \cite{Le'10} & Low-speed damping controller for stepper motor; & XC2V8000 FPGA module from Xilinx \\
% % As this is control loop application, max. vibration 2000-18000 pps 
% % 3.2 rounds per second = 32000 pps
% \hline
% Feedforward NN (2007) \cite{Himavathi'07} & Flux estimation using NN with minimal resource utilization & Xilinx FPGA XCV400hq240 - $\sim$50\% saving in resources \\
% % & for 8-5-5-2 NN (two hidden layers with 5 nodes in each) & \\
% \hline
% Elman NN (2009) \cite{Lin'09,Lin2'09} & Force is computed to control the mover position of linear ultrasonic motor & Virtex-II FPGA, tracking error of 1.78$\mu$m \\
% % As this is control operation, they plotted graphs showing damping, 
% %did not quantify tracking errors! 
% \hline
% Block-based NN (2008) \cite{Jewajinda'08} & An integrated FPGA design for evolvable adaptive hardware with XOR based classification & Xilinx Virtex-5 FPGA\\
% % Its an architecture design paper, no accuracy metrics quantified 
% \hline
% Block-based NN (2012) \cite{Tran'12} & BbNN for network intrusion detection with structure and weights generated by genetic algorithms & Altera Cyclone III FPGA with 100\% detection rate maintained, 2.22\% false alarm rate \\ 
% \hline
% %Block-based NN (2010) \cite{Jewajinda'10} & Genetic algorithm based optimization for BbNN learning; & no real FPGA implementation, but synthesized in ISE; 97.7\% accuracy in Arrhythmia detection \\
% % \hline
% Probabilistic NN (2010) \cite{Zhu'10} & Improve PNN FPGA implementation with mixed data size precision and CORDIC based activation function implementation for neural decoding & Virtex-5 FPGA - Less number of resources \\
%  % &  & \\
%  %(2010)  & ;   & \\
% % https://en.wikipedia.org/wiki/CORDIC - CORDIC is a special technique for hyperbolic 
% % and trigonometric functions 
% \hline
% Probabilistic NN (2010)  \cite{Zhu2'10}& Spike sorting using PNN, 32-bit data, more DSPs used for 32-bit than 16-bit & Xilinx Virtex-5 FPGA implementation 44$\times$ compared to MATLAB implementation \\ 
% \hline 
% Probabilistic NN (2007) \cite{Shima'07}  & Delta-sigma Modulation (for weight calculations) based PNN for Electromyogram (EMG) pattern discrimination & XtremeDSP Development Kit-II, up to 96.98\% accuracy \\
% \hline 
% \end{tabular}
% }
% \label{tbl:hw-nn}
% \vspace{-2em}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[htb]
% \centering
% \caption{Hardware implementations of regression techniques}
% \scalebox{0.86}{
% \begin{tabular}{|p{2.1cm}|p{4cm}|p{2cm}|}
% % \begin{tabular}{|p{4cm}|p{7cm}|p{4cm}|}
% %	\begin{tabular}{|p{2cm}|p{4cm}|p{2cm}|}
% \hline
% Technique & Implementation Details & Note \\

% \hline
% Regression (2020) \cite{Regression_Gao_2020} & Framework to implement Stochastic Configuration Network (SCN) model adapted to regression analysis & SCN-based model on FPGA performs 56.37\% and 17.35\% better than the extreme learning machine (ELM)\\

% \hline
% Regression (2018) \cite{Shrivastwa_Regression} & Proposed a combination of compressive sensing and neural network for the compression and reconstruction of ECoG signals & Compression ratio of 50\% and reconstruction accuracy of 89.85\%. Target FPGA: Virtex-7 (XC7VX485T-2FFG1761C)   \\

% \hline
% %Logistic regression & Biometric identification of individual & \\
% %& based on ECG signal & \\ 
% % This is software implementation, states its for hardware efficient, but no substantial  proof
% %\hline
% Multivariate Regression (2014) \cite{Khan'14} & Imaging based regression for Anemia detection &  Altera FPGA board implementation\\
% % comparison of Hemoglobin count between matlab and fpga provided, but no final comparison in terms of accuracy or something provided 
% \hline
% Linear Regression (2011) \cite{Pablo'11} & Different hardware architecture proposed for linear regression for automated modulation and classification & Xilinx Virtex FPGA (89 logic slices and 5 DSPs) \\
% \hline
% Logistic regression (LR) (2015) \cite{Page'15} & EEG feature extraction and classification; LR outperforms SVM, Naive Bayes &  ASIC - 65nm, 0.008mm$^2$, 37nW\\
% \hline
% Linear Regression (2012) \cite{Kalali'12} & Prediction of intra-frames in HVEC considering a reference frame along with current frames & Xilinx Virtex-6, 30fps, 44.60mW power (max.) \\
% \hline
% Linear Regression (2013) \cite{Belhadj'13} & Pixels are predicted based on the adjacent pixels instead of previous frames &  Altera Stratix IV FPGA- 68 MHz, 14\% resource utilization\\ 
% \hline
% \end{tabular}
% }
% \label{tbl:hw_reg}
% \vspace{-1.5em}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

% \begin{table}[!htb]
% \centering
% \caption{Hardware Implementation of Deep Learning}
% \scalebox{0.86}{
% \begin{tabular}{|p{2cm}|p{3.6cm}|p{2.5cm}|}
% % \begin{tabular}{|p{4cm}|p{7cm}|p{4cm}|}
% %	\begin{tabular}{|p{1.8cm}|p{4cm}|p{2.2cm}|}
% \hline
% Technique & Implementation Details & Note \\

% \hline
% Deep NN (2017) \cite{DNN_Zamorano_1} & Back-propagation learning algorithm is implemented in FPGA to reduce high computation time & Design on VIRTEX-5 XC5VLX110T  much faster than C and Matlab-based implementation\\


% \hline
% Deep NN (2015) \cite{Yu'15} & Feedforward neural network accelerator for prediction & Zedboard - speedup up to 30$\times$\\
% \hline
% Deep NN (2011) \cite{Orlowska'11} & Two hidden layers feedforward NN for speed estimation Implemented in LabView & Max. estimation error of 5.43\% \\
% % No information on FPGA implementation provided 
% \hline
% Deep NN (2016) \cite{Han'16} & CNN with memory hierarchy for data allocation, data flow optimization for image classification & Throughput of 1244GFlop/s with Xilinx Vertex UltraScale XCVU440, 5.48$\times$ than state-of-the-art FPGA works \\

% \hline
% CNN (2019) \cite{CNN_Nguyen} & YOLO CNN implemented on FPGA for real-time object detection with high throughput effeciency & VC707 FPGA - 1.877 TOPS throughput @200MHz; mean average of 64.16\% for the PASCAL VOC 2007 dataset  \\

%  \hline
% CNN (2016) \cite{Ma'16} & A compiler that analyses CNN structure and parameters, and generates a set of modular and scalable primitives to accelerate various deep learning techniques on Altera Stratix-V FPGA &  Achieve up to 117.3 GOPS; 48\% logic utilization and all 256 DSPs used  \\
% \hline
% CNN (2016) \cite{Wang3'16} & A dynamic quantization method to reduce precision while maintaining same or similar accuracy, achieving low power consumption with less resources is proposed & Xilinx ZynQ board used, 14.22 GOPS/J efficiency \\

% \hline
% RNN (LSTM) (2019, 2020) \cite{Rakib_1, Rakib_2} & RNN implementation proposed to generate SAT-hard clauses  as an alternative, providing low area and power overheads & 160.95$\times$, 2.06$\times$, and 6.26$\times$ area savings and 63.46\%, 91.65\%, and 96.53\% power savings on average compared to LUT+LUT, SARLock+SLL, and SLJI+TI based techniques, respectively\\
% \hline
% \end{tabular}
% }
% \label{tbl:hw-dl}
% \vspace{-1.6em}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{table}[htb]
% \centering
% \caption{Hardware Implementation of Support Vector Machines}
% \scalebox{0.86}{
% \begin{tabular}{|p{1.5cm}|p{3.4cm}|p{3.2cm}|}
% % \begin{tabular}{|p{3cm}|p{7cm}|p{4.5cm}|}
% %	\begin{tabular}{|p{1.5cm}|p{4.1cm}|p{2.4cm}|}
% \hline
% Technique & Implementation Details & Note \\

% \hline
% SVM (2020) \cite{SVM_Bassoli_2020} & SVM architecture as a solution for high computational power kernel function & Xilinx Artix-7 XC7A100T FPGA and Altera Cyclone 10 LP 10CL010. 95\% reduction in both area and time \\

% \hline
% SVM (2019) \cite{SVM_Lopes'19} & Parallel implementation of SVM on FPGA using Stochastic Gradient Descent (SGD) as a superior alternative to Sequential Minimal Optimization (SMO) for big data analysis & 10,000$\times$ speedup relative to software implementations running on a quad-core processor; 319$\times$ speedup compared to state-of-the-art FPGA implementations\\

% \hline
% SVM (2016) \cite{SVM_Tinoosh_1} & SVM for anomaly detection in NoC-based many-core architecture & Detection accuracy range between 94\% - 97\%. Power overhead range is 3\% to 1\% for 16-core implementation; 65\% reduction in area overhead, and 3$\times$ faster than previous works \\

% \hline
% SVM (2010) \cite{Llata'10} & SVM for Image classification and sinc$(x)$ regression & Cyclone II FPGA - max. classification error is 3.5\% \\
%  % no performance metric provided on regression 
% \hline
% SVM (2013) \cite{Li'13} & SVM based image classification is implemented  & Training time onf FPGA Virtex II is $\sim$4$\times$ faster than Matlab; max. accuracy 98.22\%  \\
% % &   & \\
% % (2013) & FPGA of Virtex - II Pro series -  & \\
% \hline
% SVM (2013) \cite{Hussain'13}  & SVM based microarray classification with SVM using  systolic multiplier array & Xilinx XC4VSX35 FPGA implementation is $\sim$85$\times$ faster in image classification compared to general purpose processor  \\
% %(2013) &  & \\
% \hline
% SVM (2012) \cite{Kryjak'12} & A local binary pattern based thresholding for feature extraction followed by SVM for pedestrian detection is proposed & Xilinx Virtex 6 FPGA implementation with 15\% logic slices and 66 DSP\_48s are used, 7.44W power consumption and achieves 97\% detection accuracy \\
% %  & ; Real time video stream  & \\
% %   & with 640$\times$480@60fps resolution is processed on ; & \\
% %   &  for & \\
% % (2012)  & FPGA and  & \\
%  \hline
% % SVM & Indirect matrix converter (IMC, also referred to as 2-stage direct power  & \cite{Hamouda'11} \\
% % & converter) is proposed with DSP to build specified pulses at PWM and  & \\
% %  & FPGA to synthesize suitable gate pulses for semiconductor controlled devices & \\
% SVM (2006) \cite{Fazakas'06} & To classify gray-scale noisy images based on presence of human face structure in image; BRAM used instead of LUT-based RAMs; Multipliers placed close to BRAM have lower propagation time compared to LUT-RAM & SPARTAN 3 FPGA implementation takes 1.58$\mu$s to classify 1 image, 45.2$\mu$s on Pentium IV \\
% %  &  & \\
% %  & ;   & \\
% % (2006) &  & \\
%  \hline
% SVM (2016) \cite{Bourrasset'16}  & Histograms are computed for gradients and SVM for object classification; CAPH based hardware description is used & Altera Cyclone III FPGA; 17\% of Logic elements used and 1 DSP for SVM with 1280$\times$1024@50fps resolution, 90\% true positive rate over INRIA pedestrian data set \\
% %& ;  & \\ % CAPH is a programming language used to generate HDL script in this work, similar to C in Vivado HLS
% %& & \\
% %(2016) &  & \\
% \hline
% \end{tabular}
% }
% \label{tbl:hw-svm}
% \vspace{-2em}
% \end{table}


\section{Complexity Analysis}
\label{sec:cmplx}
This chapter provides the computational complexity for each of the techniques discussed and the number of computations required in terms of additions, subtractions, multiplications, and divisions. The numbers given should be considered as first-order estimates to outline roughly the computational complexity. Specific implementations can deviate significantly from these estimates.

The notations provided in Table \ref{tbl:ind_cmplx} are given below: 
\begin{itemize}
\item $N$ - size of input data 
\item $s$ - number of iterations to obtain the square root
%\item $l$ - length of correlation window (in a discrete process)
% R(l)=\frac{1}{(n-l)\sigma^2} \sum_{t=1}^{n-l} (X_t-\mu)(X_{t+l}-\mu)
\item $M$ - number of nodes in the hidden layer in a neural network 
\item $K$ - number of neurons in the output layer of neural network 
\item $A_1$ - computational complexity of activation function in hidden layer(s) of neural network 
\item $A_2$ - computational complexity of activation function in output layer of neural network 
\item $D$ - number of hidden layers in deep neural networks 
\end{itemize}

%the input size of the data is represented by $N$. 
%For a neural network, $M$ represents the , 

% layer and . 
%Similarly, for the deep learning case, $D$ denotes the number of hidden layers. 
Note that we assume that the complexity of activation functions in all 
hidden layers are the same for the deep learning neural network and further the 
complexity is provided. 
Division and multiplication are hard to be classified individually, hence provided as `Mul/Div.' 
%can be realized using shift operation, hence 
%we provided the operation count for division and multiplication as `shift.' 
%in Table \ref{tbl:ind_cmplx}. Similarly 
Addition and subtraction provided as `Add'.
Comparison operation is provided by `Comp'. The computation numbers provided do not include training, as training could be 
done off-line.

% \begin{table}[t]
% \centering
% \caption{Complexity of Different Techniques}
% \scalebox{0.77}{
% \begin{tabular}{|l|l|l|}
% \hline
% Name & Complexity & Num of Operations\\
% \hline
% \hline
% Mean & O($N$)  & ($N-1$) Add; 1 Div \\
% % Assume there are N numbers for which mean needs to be determined
% % Then number of computations is N additions 
% \hline
% RMSD & O($N$) & ($N-1+s$) Add; ($1+2s$) Mul/Div \\
% % Calculating RMSD is similar as mean, except with additional 
% % squaring and having a square root 
% % Regarding square-root, it could be decomposed into sum and division and 
% % done iteratively . See for instance Babylonian method: 
% % https://en.wikipedia.org/wiki/Methods_of_computing_square_roots#Babylonian_method 
% % Hence 1 square root involves (1 add, 2 shift)*s, s ->iterations 
% \hline
% Mode & O($N$)  & $N$ Add, $N$ Comp\\
% % Consider a series of N elements, so to find mode i.e., most 
% % repeating element, the whole series needs to be traversed and 
% % number of times each element is repeated needs to be counted, hence N 
% \hline
% Standard Deviation & O$(N)$ & ($N-1+s$) Add; ($1+2s$) Mul/Div \\ 
% %$(2N+s)$ - Add, $(N+1+2s)$ - shift\\
% % similar to finding RMSD 
% \hline
% \multirow{2}{*}{FFT} & O($N \log(N)$) & $N\log(N)$ Add, $N\log(N)$ Mul/Div \\ 
% \cline{2-3}
% & O($N^2$) & $N(N-1)$ Add, $N^2$ Mul/Div \\ 
% % check below reference 
% % Look at following link to understand it: https://en.wikipedia.org/wiki/Fast_Fourier_transform \\ 
% % DFT and FFT have similar mathematical formulas, hence similar complexity. The best complexity is presented here 
% % https://en.wikipedia.org/wiki/Fast_Fourier_transform
% % The radix-2 Cooley–Tukey algorithm, for N a power of 2, can compute the same result with only (N/2)log2(N) complex multiplications (again, ignoring simplifications of multiplications by 1 and similar) and N log2(N) complex additions. In practice, actual performance on modern computers is usually dominated by factors other than the speed of arithmetic operations and the analysis is a complicated subject (see, e.g., Frigo & Johnson, 2005), but the overall improvement from O(N2) to O(N log N) remains.
% \hline
% Auto-correlation & O($N \log(N)$) & $(N\log(N)$) Add, ($N\log(N)$) Mul/Div\\ 
% %Auto-correlation & O($N \log(N)$) & $(N * l$) Add, ($N *(l+1$) ) Mul/Div\\ 
% % check below reference
% % Please check page 83 of  https://engineering.purdue.edu/~ipollak/ee438/FALL04/notes/Section1.4.pdf
% % https://en.wikipedia.org/wiki/Autocorrelation
% % l is the window size of discrete correlation 
% \hline
% Linear Regression & O($N$) & $(N-1)$ Add, $N$ Mul/Div\\ 
% % Please see following 
% % https://www.quora.com/What-algorithms-can-perform-classification-and-or-regression-on-n-observations-with-space-and-time-complexity-O-n
% % linear regression - does not include training phase, as ideally training is not 
% % considered in industrial scale applications 
% \hline
% \multirow{3}{*}{Neural Network} &  & $ ((N-1)* M + (M-1)* K)$  Add, \\
%  & O($N M$)+O($M A_1$)+ & $ (N * M + M * K)$ Mul/Div,  \\
%  & O($K M$)+O($K A_2$) & Operations for activation functions \\
% % consider there are N inputs, and neural network is fully connected. 
% % Each node in the hidden layer takes the N inputs, assume that the 
% % computations in hidden layer node has complexity of A_1, as such 
% % the complexity becomes N.A_1, further if there are M neurons in 
% % hidden layer, hence first term. For 2nd term, a similar explanation 
% % could be assumed, but the number of nodes is K and since it uses 
% % M inputs from hidden layer neurons, they are multiplied, and the 
% % computational complexity of activation function is given by A_2 
% % NN indicates here - fully connected 
% % updating weights is not given because it done during training phase, operations 
% % count given for testing phase 
% \hline
% SVM & O($N^3$) & ($N^2(N-1)$) Add, $N^3$ Mul/Div \\
% % Computation count not given for optimization phase, it is only given for 
% % testing phase : N additions for distance value from individual points, N-1 for 
% % their sum and N shift because we have N multiplication terms i.e., $x^2$
% % Please look at https://www.quora.com/What-is-the-computational-complexity-of-an-SVM - without any decomposition 
% %http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.139.2112&rep=rep1&type=pdf
% \hline
% \multirow{4}{*}{Deep Neural Network} &   & $ ((N-1)* M +(M-1)* M * D +$  \\
%  & O($N M$)+O($M A_1 D$)+ &  $(M-1)* K)$ Add, $ (N * M + $  \\
%   & O($K M$)+O($K A_2$) & $M * M * D +M * K)$ Mul/Div,  \\
%   & & Operations for activation functions \\ 
% % Computational complexity is given similar to traditional neural
% % network, except, the number of hidden layers are different hence 
% % the first term has $D$ 
% \hline
% \end{tabular}
% }
% \label{tbl:ind_cmplx}

% \end{table}



\section{Discussion and Analysis}
\label{sec:analysis}
Here we discuss the suitability of different time-series analysis techniques presented 
above in terms of their applicability, pros, cons considering various aspects such 
as for performance, hardware footprint, suitability to data size, and so on. 

\begin{itemize}
\item \textbf{Statistical Metrics based Analysis}: The advantage of this technique compared to different other techniques is their complexity and hardware footprint area. However, they lack in terms of performance and often require pre-processing of data. These techniques are suitable for smaller datasets. The main applications are periodicity detection, anomaly detection, and spectrum analysis.  
\item \textbf{Regression based Analysis}: The regression techniques are somewhat area-efficient compared to some of the machine learning techniques, and some works can be offloaded to DSPs in FPGAs for throughput improvement. This is prone to noise and may overfit or underfit the data depending on the training data. They are hardware suitable, even if implemented as ASIC. The main applications of regression are prediction, time-series feature extraction, and anomaly detection. 
\item \textbf{Neural Network (NN) based Analysis}: The advantage of NNs is their ability to learn and model the data efficiently. In terms of hardware footprint and processing, they are complex compared to statistical metrics and regression-based analysis. However, in terms of performance, they are often found to be efficient. Additionally, NNs are found to be efficient in terms of prediction, even when the amount of data to train is small compared to regression-based techniques. The NNs have a wide range of applicability ranging from simple prediction to classification and recognition of images, predicting captions, speaker bots, and so on. 
\item \textbf{Deep Learning-based Analysis}: The deep learning is advantageous when the data is large and complex to extract patterns out of it. Furthermore, they are more robust to noise compared to regression and statistical metrics-based analysis. However, in terms of area overheads, they have a bigger footprint compared to neural networks. As mentioned previously, deep learning techniques are widely used when the data is large such as voice processing, natural language processing, image processing for classification, and recognition of objects. 
\item \textbf{SVM based Analysis}: Support vector machines efficiently model even the non-linearities and extract the correlations in the patterns. In terms of processing and hardware footprints, they have higher processing costs than regression, 
but smaller footprint than neural networks. In terms of accuracy, they sometimes perform in-par with neural networks, as observed from existing works. 
\end{itemize}

Based on the above-presented analysis, the following conclusions can be derived: 
when the number of resources is small, data is little with fewer irregularities, and high accuracy or performance is not a requirement, statistical-metrics-based analysis is a viable option. When the amount of data is sufficient with appropriate computing resources available, and performance is one of the requirements, the techniques like regression and SVM are feasible. When the accuracy requirements are high, the resources are available, data available for learning is sufficient (or insufficient) and limited in size, SVM, neural networks, and their variants are a good choice. However, when the data to be processed is large, 
the deep learning techniques will be a viable option but at the expense of large amount of resources and memory. 


\section{Conclusion}
\label{sec:conc}
As the domains of cyber-physical systems and Internet-of-Things grow at a breath-taking pace, the need for devices that monitor, analyze, and classify time-series signals increases rapidly. 
This review illustrates a wide variety of techniques at our disposal, but we have no methodology to select the best strategy for a 
given application and a set of requirements. An engineer that is challenged 
to design a system for analysis of a time-series signal in a particular application is faced with an impossible problem. To make a sensible and well-informed choice, he or she must be an expert in half a dozen disciplines, from statistics to machine learning to hardware and software design. In practice, this means that the choice of algorithm and implementation platform is more driven by the expertise and the tools that happen to be available, rather than by a deliberate analysis of trade-offs.

We provide a comprehensive 
% Although this review will not fundamentally change this situation, we hope to provide an 
overview of multiple techniques available and present its benefits and applicability for different kinds of applications along with 
its complexity. Furthermore, an evaluation of its hardware implementations is presented for fair comparison and the impact on the performance. 
% is available and which techniques are worth studying in-depth before committing significant engineering resources. We also have shown that there is no single best approach. 
It has been observed that choosing an analysis technique requires careful study of the data, algorithm, and available resources on the implementation platform. This work presents and analyzes the application vs. algorithm mapping and outlines the resource consumption for different techniques.

% \begin{table*}[!htb] \small
% \centering
% \tableSpace
% \caption{Impact of adversarial attack on HMD}
% \label{tbl:adv_res}
% \scalebox{1.2}{
% \begin{tabular}{lllll}
% \hline
%  & Accuracy & Precision & F1-score & Recall \\ 
% \hline
% \hline 
% Before & 82.7\% & 80.0\% & 80.0\% & 83.0\% \\
% After & 18.3\% & 45.0\% & 10.0\% & 18.0\% \\
% \hline
% \end{tabular}
% }
% \end{table*}


==> content.tex <==
\section{Introduction} \label{sec:intro}
% Introduction to h/w security, cache-bases SCAs, and physical SCAs. What defense strategies we have proposed in the past, currently working, etc. 
The hardware security domain in recent years has experienced a
plethora of threats like the Side-Channel Attacks \cite{Yarom_usenix_'14,Gruss_dimva_'16}, Malware attacks \cite{Dhavlle_DATE'21, Dhavlle_ISCAS'21, Meraj_ISCAS'21, SMPD_DAC'19, Sanket_CASES'19, Sanket_ICMLA'19, Sanket_ICTAI'19,Sanket_DAC'21}, Hardware Trojan attacks \cite{Meraj_AsianHOST'20}, reverse engineering threats \cite{Kolhe_GLSVLSI'19, Kolhe_ICCAD'19, Hassan_ISQED'20} and so on. Among multiple threats, the side-channel attacks (SCAs) is one of the pivotal threats due to it's capability to exploit the design despite being introduced in the market post-validation. These SCAs function by exploiting
the side-channels, which invariably leak important data during
an application’s execution. The information leaked through side-channels are inherent characteristics of the system and are often unintentional. 
The side-channel information can be device's
microarchitectural or physical information such as 
power consumption, thermal maps, the timing of the operations, acoustics, 
and cache access traces. Some of the attacks are reported in \cite{report_1, report_3, report_4} with vulnerabilities in Linux been reported in \cite{report_5}. The work in \cite{report_2} lists and reports the common vulnerabilities in the computing systems discovered so far, while some newer threats to a CPU have been reported and described in \cite{report_6}. It is quite evident by looking at the mentioned reports that the side-channel attacks have proven a major threat to system security, and developing novel mechanisms to mitigate them becomes inevitable. 

Snooping on co-located programs' cache trace is performed by cache-based SCAs and is prominently explored in the domain of SCAs. A part of my thesis work focuses on timing-based cache attacks, which exploit the time required to flush/reload an instruction from the cache subsystem as a covert channel\cite{Abhijitt_isqed'20,Dhavlle_TCAD'21}. Some of the popular cache targeted SCAs are the Flush+Reload\cite{Yarom_usenix_'14} and Flush+Flush attack\cite{Gruss_dimva_'16}.
Intercepting secret information based on the study of power signature is a subdivision of SCAs where power consumption information serves as a covert channel leaking crucial information about the executed operations. 
Such physical and cache-based SCAs are known to be a significant threat to cryptosystems such as AES (Advanced Encryption Standard) and RSA and can reveal the encryption key efficiently. Yet these attacks are not limited to the cryptographic algorithms, and they can be extended to snoop on other applications as well. 
One can argue to have a 
% That being said, an obvious 
solution that can simply shut the covert channels and hence prevent such threats in the first place. It is not as straightforward as it seems to be because shutting down covert channels that originated due to vulnerability is not feasible due to the cost and performance constraints. Hence, in this report, we introduce the reader to primarily cache-targeted and physical SCAs, discuss the proposed solution, existing works, and how it compares with our solution, along with current ongoing and future projects. 

The rest of this report is organized as follows: Section \ref{sec:cache_based} enumerates and describes the existing works on cache-targeted attacks and defenses, and our proposed defense; Section \ref{sec:physical_based} mentions previous works on physical SCAs and the ongoing research in the domain; Section \ref{sec:conclusion} concludes this report with the anticipated results and contributions considering the current ongoing research.
% and Section \ref{sec:list_publications} list all the accepted publications, under review works, WiP work and accepted poster presentations.
% \vspace{-1em}



% \begin{figure}[tb!]
%     \centering
%     \includegraphics[width=0.35\textwidth]{figures/cache_system.pdf}
%     \caption{Block Diagram of the Cache Sub-system}
%      \label{fig:cache_system}
%      \vspace{-1em}
% \end{figure}

% \begin{figure}[tb!]
%     \centering
%     \includegraphics[width=0.20\textwidth]{figures/flush_reload.pdf}
%     \caption{Flush+Reload Attack Principle}
%      \label{fig:flush_reload}
%         \vspace{-1.6em}
% \end{figure}
%   \vspace{-1em}
   

\section{Cache-Targeted Side-Channel Attacks/Defenses} \label{sec:cache_based}

Cache-targeted attacks primarily rely on the timing information to successfully probe the intended process/data. The idea is to co-locate 
with a victim and snoop on its private data over the covert channel. 
Intel CPUs use \textit{cflush} instruction to evict a specified cache line from the cache subsystem. Intel uses inclusive caches, meaning a line evicted from the cache using the \textit{cflush} command does evict it from all the levels of cache. The block diagram of the cache subsystem is shown in Figure \ref{fig:cache_system}(b). The attackers time the \textit{cflush} instruction after evicting a cache line belonging to the victim. Depending on the access time, 
the attacker deduces if the victim accessed the data. Flush+Flush\cite{Gruss_dimva_'16} and Flush+Reload\cite{Yarom_usenix_'14} are some of the most popular cache-targeted SCAs exploiting the timing information to steal private data. 

% \textbf{Flush+Reload Attack:} A quick background on the Flush+Reload attack has been discussed here. Figure \ref{fig:cache_system}(a) demonstrates the attack process: 
% \begin{enumerate}
%     \item The attacker flushes the victim's cache line that corresponds to a line/function in victim's code.
%     \item The attacker waits for the victim to access its data.
%     \item The attacker again reloads the same data and times this access.
%     \item If the time happens to be greater than the threshold, it means the victim did not access the data. This event corresponds to a cache miss.
%     \item If the access time is less than the threshold, the victim accessed the data. This corresponds to a cache hit.
% \end{enumerate}
In this section, we discuss the existing cache-targeted SCAs, defenses, and our proposed \shield\ as a defense against cache-targeted attacks. 
% \vspace{-1.2em}
\subsection{Existing Attacks Targeting Cache} 
\textbf{Flush+Flush}: Flush+Flush\cite{Gruss_dimva_'16} is a passive type of an attack unlike its sibling, Flush+Reload\cite{Yarom_usenix_'14}, in the sense that it does not reload the data again to check a hit/miss. This attack depends on the time it takes for the \textit{cflush} instruction to complete. Because the system has to flush all the copies of the flushed data, it requires some time to do so, and hence, flushing a data that is present in the cache takes more time as against missing data. Hence, Flush+Flush can silently attack a victim and steal its secret data. 

\textbf{Prime+Probe}: The Prime+Probe\cite{Liu_prime_probe} attack targets the LLC. The attacker 'primes' or prepares its cache by loading a chunk of data. It then waits for the victim to execute. If the victim's data is mapped to the same area as the attacker's data, the attacker data is evicted given the replacement policy. When the attacker reaccesses its data, it deduces if the victim's data was present, depending on whether the 'probe' was a hit or a miss.

\textbf{}
\textbf{Flush+Reload}: 
A quick background on the Flush+Reload attack is discussed here. Figure \ref{fig:cache_system}(a) demonstrates the attack process: 
\begin{enumerate}
    \item The attacker flushes the victim's cache line, which corresponds to a line/function in victim's code.
    \item The attacker waits for the victim to access its data.
    \item The attacker again reloads the same data and times this access.
    \item If the time happens to be greater than the threshold, it means the victim did not access the data. This event corresponds to a cache miss.
    \item If the access time is less than the threshold, the victim accessed the data. This corresponds to a cache hit.
\end{enumerate}

% This attack was already discussed in Section \ref{sec:intro}. 

\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{figures/combined.pdf}
    \caption{(a)Flush+Reload Attack Principle; (b)Block Diagram of the Cache Sub-system}
     \label{fig:cache_system}
    %  \vspace{-2em}
\end{figure}

\subsection{Existing Defenses for Cache-Targeted SCAs} 
% Here, we will discuss different categories of defenses and refer to some existing works. 
The existing defenses against cache-targeted SCAs can be broadly categorized into five categories, as discussed below. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Randomization based} 
Cases where modifying the hardware is not feasible, randomizing the memory accesses has been proposed in \cite{Wang_isca_'07}. The work in \cite{He_micro_'17} proposed the use of random memory-to-cache mappings to make the attack difficult. A permutation table for each process causes dynamic memory address to cache set maps. The attacker relies on evicting 
a specific cache line to perform the attack, dynamic memory address 
mapping prevents the attacker from evicting the targeted cache line. 
This comes for a price though, as maintaining the table during runtime 
affects performance. 
A dynamic random control flow by exploiting software diversity is introduced in 
\cite{Crane_ndsss"15}. 
% Authors in \cite{Crane_ndsss"15} propose software diversity by dynamically randomizing the control flow\footnote{Taken as it is from \cite{Abhijitt_isqed'20}}. 
The main idea is to transform the program trace of each application into a unique trace. The technique dynamically randomizes the control flow of the program during runtime. Replicas of functions within the code are created, and the dynamic program flow chooses one of them in runtime to randomize the overall control flow. 

\subsubsection{Partition based}
DAWG by Kiriansky\cite{Kiriansky_micro'18} proposes a Dynamically Allocated Way Guard (DAWG) to protect way partitions in a set-associative cache. Secure isolation is provided by giving a notion of protected domains within the cache. DAWG is capable of isolating cache miss, hit, and other metadata across the protected domains. DAWG can protect against attacks that depend on timing behaviors. The defense mechanism can be extended to branch history tables or the TLBs. However, DAWG would need supplemental techniques to block covert channels, and this defense leads to performance overhead. Another partitioning based technique is proposed in \cite{He_micro_'17}, which promises to protect sensitive data from attack by reserving dedicated cache sets. The sensitive process, in this way, would map to the protected cache area, thereby reducing the interference caused by other programs. But, this method requires the intervention of the operating system to separate cache into a reserved and non-reserved area, all of which must be non-overlapping. This brings overhead and inefficient cache utilization, along with security. 

\subsubsection{Intel Cache Allocation Technology (CAT)}
Work in \cite{Liu_hpca'16} utilized Intel's CAT technology to protect SCAs on shared last-level cache. CAT is a way partitioning mechanism that ensures efficient utilization of the cache space/occupancy. Another work in \cite{Dong_usenix'18} proposes to use CAT in addition to the mechanism that can partition the LLC to thwart SCAs. CAT cannot by itself securely partition the cache. The attack launches on a compromised operating system. Hence, by preventing cache line sharing with applications or OS, the authors propose to defend against SCAs. 

\subsubsection{Detection based defenses}
Cloudradar\cite{Zhang_raid_'16} proposes to detect SCAs using hardware performance counters (HPCs). Specialized cores are employed to detect SCAs based on either signature detection technique or anomaly-based detection established on HPCs. The system constantly monitors the HPCs. These traces are then compared with pre-stored attack signatures to detect the presence of an attack. Another technique used is the anomaly detection technique, which alerts the system based on the drift of the program flow from its normal flow. Stealthmem\cite{Kim_usenix'12} provides a system-level protection against cache SCAs. It protects the cache from unauthorized accesses by providing a set of locked cache lines per core. These cache lines are never evicted. Authors in \cite{Shi_dsnw'11} develop a technique, titled as dynamic cache coloring. This technique cautions the virtual machine when a security-sensitive operation is being processed. This swaps the data to a safe, isolated cache line that has limited access, thus preventing the attack.  

\subsubsection{SGX Enclave based}
Varys\cite{Oleksenko_usenix'18} proposes to protect the system from timing based and page-table attacks. The main idea is to prevent shared resources. During the execution of secure-sensitive operations in the enclave, strict reservation of physical cores is enforced. 
These previous works have been summarized in Table \ref{tbl:cache_summary}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[!htb]
\centering
\caption{Cache Targeted Defenses Summarized} 
\label{tbl:cache_summary} 
% \vspace{-1em}
\scalebox{0.63}{
\begin{tabular}{|c|c|}
\hline
Title/Reference & Technique \\
\hline
``New Cache" \cite{Wang_isca_'07} & Randomize memory maps. \\
\hline
``How secure is your cache?" \cite{He_micro_'17} & Use permutation tables to randomize cache mapping to make it harder to evict specific targeted cache line. \\
\hline
``How secure is your cache?" \cite{He_micro_'17} & Sensitive process access dedicated non-overlapping cache set. \\
\hline
``Varys" \cite{Oleksenko_usenix'18} & Protects programs in SGX enclaves from cache attacks.Strict reservation of physical cores to threads.\\
\hline 
``Cloudradar" \cite{Zhang_raid_'16} & Cores  (processors)  equipped  with specialized signature detection. Detects  SCAs  based  on  the  hardware  performance  counters(HPCs). \\

\hline
``Stealthmem" \cite{Kim_usenix'12} & Protects cache  from unauthorized access by creating set  of  locked  cache lines  per  core. Lines are never evicted  from  the  cache.  
\\

\hline

``Dynamic Cache Coloring" \cite{Shi_dsnw'11} & Notifies VM when application executing secure-sensitive operations.\ Swaps associated data to safe and isolated cache line, limiting its access. \\

\hline
``Partition Locked (PL) Cache" \cite{Wang_isca_'07} & Protected cache line cannot be evicted by an attacker’s miss. \\

\hline
``Non-monopolizable Cache" \cite{Domnister_nomo'12} & Sensitive process assigned reserved ways in each cache set. Disallow attacker from occupying whole cache set. \\
\hline
\end{tabular}
}
\end{table*}



\subsection{Proposed Entropy-Shield}
In this subsection, we discuss the vulnerability in the GnuPG RSA encryption algorithm and propose a defense mechanism to thwart attacks. 
\subsubsection{Vulnerability in RSA}
The vulnerabilities in the existing RSA algorithms is described in \cite{Yarom_usenix_'14} and also demonstrates how Flush+Reload can successfully retrieve all the secret key bits. Referring to Table \ref{tbl:rsa}, bit `0' in a secret key would translate to RSA executing a square operation followed by a modulo operation. Likewise, square-modulo-multiply-modulo operations are called for a bit `1'. Table \ref{tbl:rsa_sequence} shows the sequence of operations corresponding to different key bit combinations. By observing the functions calls to the square, reduce or modulo lines of code, the attacker can deduce the secret key bits. Not all the bits need to be retrieved at once, but the attacker has to execute the attack for several hundreds of thousands iteratively to guess the correct key. 

\subsubsection{Entropy-Shield} 
Earlier, we discussed different attacks and defense strategies. With the defenses discussed, it is evident that some of them require software level changes to the operating system or the hypervisor, while others require hardware modifications, causing inefficient utilization of the cache or severe overheads. Hence, we propose \shield\ as a defense against timing-based SCAs, shown in Figure \ref{fig:full_diagram}. 
% \footnote{Figure taken from published work \cite{Abhijitt_isqed'20}}. for the overview diagram of the \shield\. 
In Figure \ref{fig:full_diagram}(a), we can see that the attacker can sniff the covert channel and hence, retrieve secure-sensitive data. With \shield\, the attacker is misled to an incorrect key. This is achieved using fake/dummy calls to the square, reduce, or multiply functions. We call this as adding perturbations to the signal/channel observed by the attacker. For example, if a bit `0' is processed by the victim, the \shield\ calls dummy Multiply-Modulo operations following the original Square-Modulo operations, thus giving the notion of bit `1' processed by the victim when bit `0' was processed. Refer to Table \ref{tbl:fake_sequence} for the fake operations corresponding to key bits. 
Referring to Figure \ref{fig:full_diagram}(b), with \shield\, dummy operations are called to mislead the attacker. The \shield\ offers \textit{Uniform} and \textit{Deceptive} mode of operation. \textit{Uniform} mode adds maximum noise to the channel by flipping all 0's to 1's, while \textit{Deceptive} mode cognitively perturbs the sequence by randomly calling dummy operations, the position of the bits perturbed change every run. The results of the \shield\ from \cite{Abhijitt_isqed'20} is presented in in Tables \ref{tbl:shield_results_uniform}
% \footnote{Figure taken from published work \cite{Abhijitt_isqed'20}} 
and \ref{tbl:shield_results_deceptive}. 
% \footnote{Figure taken from published work \cite{Abhijitt_isqed'20}}.




\begin{table}[!htb]
\centering
\caption{Operations Corresponding to Key Bits} 
% \vspace{-0.5em}
\label{tbl:rsa} 
\scalebox{1}{
\begin{tabular}{|c|c|}
\hline
Secret Key Bit & Corresponding Operations \\
\hline
Bit `0' & Square-Modulo \\        
\hline
Bit `1' & Square-Modulo-Multiply-Modulo \\ 
\hline
\end{tabular}
}
\end{table}
%   \vspace{-1em}
\begin{table}[!htb]
\centering
\caption{Sequence of Key Bits to Corresponding Operations} 
% \vspace{-0.5em}
\label{tbl:rsa_sequence} 
\scalebox{1.2}{
\begin{tabular}{|c|c|}
\hline
Bit Sequence & Corresponding Operations \\
\hline
``0010" &  SR-SR-SRMR-SR\\        
\hline
``1100" &  SRMR-SRMR-SR-SR\\
\hline
\end{tabular}
}
\end{table}

\begin{table}[!htb]
\centering
\caption{Sequence of Key Bits to Corresponding Operations} 
% \vspace{-0.5em}
\label{tbl:fake_sequence} 
\scalebox{1}{
\begin{tabular}{|c|c|}
\hline
Secret Key Bit & Corresponding Fake Operations \\
\hline
Bit `0' &  Square-Modulo\\        
\hline
Bit `1'  &  Square-Modulo-\textcolor{red}{Multiply-Modulo} \\
\hline
\end{tabular}
 } 
%  \vspace{-1em}
\end{table}


\begin{figure*}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{figures/full_figure.pdf}
    \caption{(a) Traditional side-channel attack on encryption algorithm where the data leaked via covert channel is accessible to the attacker; (b) Victim wrapped with Entropy-Shield that injects perturbation during run-time to perturb the sensitive information leaked thereby making SCAs laborious and time-consuming. *Only Uniform mode results have been shown* \cite{Abhijitt_isqed'20}}
    % \vspace{-1em}
     \label{fig:full_diagram}
    %  \vspace{-0.5em}
\end{figure*}

\begin{table*}[htb!]
\centering
\caption{Key as visible to the attacker and the victim with \shield\ - Uniform mode of operation} 
\label{tbl:shield_results_uniform} 
\scalebox{1}{
\begin{tabular}{|c||c|c|c|c|c|}
\hline
Attack Type & Encryption & Key  &  Original Key & Victim seen key & Key seen by the attacker \\

\hline

% \parbox[t]{3mm}{\multirow{6}{*}{\multicolumn{1}{|c}{} \rotatebox[origin=c]{90}{Adv. training with}}}
\multirow{2}{6em}{Flush+Reload}  & RSA-RSA & key\_1 & 0FCFFF & 0FCFFF & FFFFFF \\        
\cline{2-6}
& DSA-Elgamal & key\_2 & 587BFA & 587BFA &  FFFFFF\\
\cline{1-6}
\multirow{2}{6em}{Flush+Flush }& RSA-RSA & key\_3 & 54FF0B & 54FF0B & FFFFFF \\
\cline{2-6}
& DSA-Elgamal & key\_4 & 89DE00 & 89DE00 & FFFFFF \\
\hline

\end{tabular} 
}
\end{table*}

\begin{table*}[htb!]
\centering
\caption{Key as visible to the attacker and the victim with \shield\ - Deceptive mode of operation} 
\label{tbl:shield_results_deceptive} 
\scalebox{1}{
\begin{tabular}{|c||c|c|c|c||c|c|}
\hline
Attack Type & Encryption & Key  &  Original Key & Victim seen key & \multicolumn{2}{c|}{Key seen by the attacker}  \\
\hline
 & & & & & Iteration 1 & Iteration 100th \\
 \hline
% \parbox[t]{3mm}{\multirow{6}{*}{\multicolumn{1}{|c}{} \rotatebox[origin=c]{90}{Adv. training with}}}
\multirow{2}{6em}{Flush+Reload}  & RSA-RSA & key\_1 & 0FCFFF & 0FCFFF & \textcolor{red}{5}F\textcolor{red}{D}FFF & \textcolor{red}{0}F\textcolor{red}{E}FFF \\        
\cline{2-7}
& DSA-Elgamal & key\_2 & 587BFA & 587BFA &  5\textcolor{red}{9F}BF\textcolor{red}{B} & \textcolor{red}{7}8\textcolor{red}{FF}F\textcolor{red}{E} \\
\cline{1-7}
\multirow{2}{6em}{Flush+Flush }& RSA-RSA & key\_3 & 54FF0B & 54FF0B & \textcolor{red}{75}FF\textcolor{red}{1}B & 5\textcolor{red}{5}FF\textcolor{red}{1F} \\
\cline{2-7}
& DSA-Elgamal & key\_4 & 89DE00 & 89DE00 & \textcolor{red}{CB}D\textcolor{red}{F}0\textcolor{red}{2} & 8\textcolor{red}{B}D\textcolor{red}{F}0\textcolor{red}{1} \\
\hline

\end{tabular}
} 
% \vspace{-2em}
\end{table*}

\section{Physical Side-Channel Attacks} \label{sec:physical_based}
Physical side-channel attacks are those that require proximity to a victim device - an FPGA or a CPU. The attack principle is to target data-dependent power traces/signatures of the victim device. Crypto algorithm like the AES demonstrates data-dependent power consumption which serves as a covert channel. The attacker attaches a probe to measure the power traces by executing the application iteratively. By applying methods such as Correlation Power Analysis (CPA), Differential Power Analysis (DPA), or the Simple Power Analysis (SPA), the attacker can reveal the entire secret key. This data-dependent behavior can be extended to other non-cryptographic applications as well to snoop on the private data. 
In this section, we discuss the physical side-channel attacks, those that require proximity to the target hardware, as well as the remote physical side-channel attacks. 
% are also discussed here.
We review the existing attacks, defenses, and our ongoing work in this domain. % In the Section \ref{sec:future}, we will take a look in to our anticipated projects we want to work and publish papers on.

\subsection{Existing Power-based Physical Side-Channel Attacks} 
Work in \cite{Zhao_remote_fpga'18} exploits a new vulnerability in the power-sharing within FPGA to snoop on other entity's power consumption. The power rails are shared across all the components. The attack employs ring oscillator (RO) -based design to convert voltage drops to figures, representing power consumption of co-located applications on the same FPGA. The attack describes the successful recovery of the RSA key. Authors in \cite{Ramesh_without_access'18} bring to light yet another type of vulnerability. The work discusses how an RO-based spy can read the relative delay in the wire, a delay caused by logic values on the adjacent victim wire. The crosstalk between two wires - transmitter (victim) and the receiver (spy) - is exploited in this type of attack. Hardware designs have a strict power budget, which causes one component to power throttle while another power-hungry component is operating. This power budget has been exploited as a covert channel in \cite{Khatamifard_powert_19}. The source entity is assumed to have access to sensitive data while the sink has access to a third party application that reads the data. Using power viruses, the attack causes other known (spy) entity to power throttle, thus utilizing this reduced performance factor to correspond to logical values `0' or `1'. Simple Power Analyis (SPA)\cite{SPA'07,Mangard_spa'03} , Difference-of-Means Power Analysis (DPA)\cite{Lo_dpa_cpa'17} and Correlation Power Analysis(CPA)\cite{Lo_dpa_cpa'17} are analysis methodologies used to extract secret data from the observed power traces of an application. Simple Power Analysis is the most simple type of them. It requires manual observation of the power traces to extract the key. DPA requires the collection of a large number of traces. These traces are processed statistically to find the mean of differences observed in the traces, to derive the secret information. While in CPA, the correlation between the measured power traces and the guesses (from a hypothetical power model) is calculated to conclude the secret key.  

\subsection{Existing Defenses} 
Nele Mentens in \cite{Mentens_randomization'17} proposed to utilize hardware components of the FPGA to thwart attacks. The reconfigurations to prevent leakage are performed in runtime. The author discusses the addition of random noise, irregular clock cycles, and scrambling S-Box in the hardware to thwart attacks. Work in \cite{Yu_codes'07} proposed an intelligent place-and-route technique to perform symmetrical routing. This approach is explained to defense against power analysis SCAs. Authors in \cite{Kocher_crypto'99} explain the algorithmic countermeasures that minimize the correlation between power and processed data. 

\subsection{Ongoing work in Physical Side-Channel Attacks domain}
The ongoing work in physical SCAs is to research on methods to secure FPGA implementation of crypto algorithms from attacks. We are working on CPA type attacks on power traces collected during the execution of the AES application. Once the attack is successful, securing the FPGA with approximate modules is what we plan to focus on in the future. Post power trace collection on the secure design, we would attack with CPA again to evaluate the resilience of the new security measure implemented.

\section{Research Progress:}
As described in the previous sections, I have been working and publishing papers on Malware Detection \cite{SMPD_DAC'19}, Side-Channels Analysis \cite{Abhijitt_isqed'20, Dhavlle_TCAD'21}, Hardware-based Trojan Attack and Detection \cite{Meraj_AsianHOST'20}, and Survey-based papers \cite{Brasser_CASES'18, Dhavlle_IGSC'20} published to conferences and journals. I intend to dive deeper into more of SCA based attacks and defenses in future and contribute my work to top tier conferences and journals. 
% \section{Works in Progress} \label{sec:future}

% This section describes our ongoing projects, what contribution they would make, and what the anticipated results would look. Some of the mentioned works are published as proceedings, while others are available on ArXiv. 

% \subsection{\shield\ for FPGA-based RSA (ES-FPGA)}
% As we have discussed previously that the square, reduce, and multiply operations are crucial for the cipher generation. But, the \shield\ we discussed so far is for software implementation of the RSA algorithm. Here, we plan to employ the same principle of cognitive perturbations to the hardware-based implementation of RSA. This is a plausible and valid approach as FPGAs are being deployed by various industry giants to accelerate performance by offloading compute-intensive tasks to re-configurable devices like the FPGAs \cite{report_7, report_8, report_9, report_10, report_11}. Like \shield\, the ES-FPGA would, in a similar manner, implement and execute dummy operations that would mislead the attacker. The attacks and defenses against physical SCAs have been discussed in Section \ref{sec:physical_based}. The novel contribution ES-FPGA would render is that it would not delay or halt computations to thwart an attack, but rather, continue computations (dummy operations) between primary operations. This approach renders the attack process very difficult to execute as there is no differentiation between the power consumption of a computation that contributes to the result and the one that does not - at least the gap is not significant to be detected. Again, the ES-FPGA does not alter the application's original functionality, yet would be capable of misleading the attacker. Refer to Figure \ref{fig:es_fpga}, which shows how the ES-FPGA can execute dummy modules (Multiply-Reduce in the Figure) to mislead the attacker to deduce bit `1' instead when the actual bit processes were `0'. A pseudorandom generator would ensure that the calls made are random. With such randomness, the power analysis attacks would be difficult to break. Considering the overhead and performance factors, this approach is sure to add little extra area overhead given the requirement of new modules. But as with every designed system for security, it would be a trade-off between security and little overhead. 

% \begin{figure}[tb!]
%     \centering
%     \includegraphics[width=0.42\textwidth]{figures/es_fpga.pdf}
%     \caption{\shield\cite{Abhijitt_isqed'20} as a Defense Against Physical Side-Channel Attacks}
%      \label{fig:es_fpga}
%         % \vspace{-2em}
% \end{figure}

% % \subsection{Secure AES with Approximate Modules}
% % Data-dependent power consumption renders the design vulnerable to power analysis attacks like the CPA, DPA, and SPA. Approximate modules with the resultant power traces have been shown in Figure \ref{fig:approx_aes}. Approximate modules are optimized modules of the same AES implemented on the FPGA fabric. These modules are similar in functionality but differ in power consumption due to optimizations. A runtime controller invokes the modules for crypto operation. Because each power trace corresponding to the set of input plaintext and the key are different - due to the fact they being processed by different modules - we anticipate that this approach could potentially thwart power analysis attacks. 

% % \begin{figure}[tb!]
% %     \centering
% %     \includegraphics[width=0.42\textwidth]{figures/approx_aes.pdf}
% %     \caption{Secure AES with Approximate Modules}
% %      \label{fig:approx_aes}
% %         % \vspace{-1em}
% % \end{figure}

% \subsection{Adversarial Operations to Secure Crypto Systems}
% As discussed previously, the power consumption corresponds to each functional module in the FPGA. This is vulnerable to attacks, as the attacker can correspond each power signature to its data-dependent block in the design. Hence, with adversarial operations, we can bring the power consumption of one module close to another functional module, thus thwarting the attack. This becomes possible because the observed traces would be non-differentiable during the attack phase. A preliminary part of this work was submitted and accepted at the Government Microcircuit Applications \& Critical Technology (GOMACTech) 2020 conference. But, due to COVID-19, the work could not undergo successful publication and distribution as the conference stood canceled. Figure \ref{fig:gomac} shows the adversarial operations to thwart attacks. The original unsecured design is shown in Figure \ref{fig:gomac}(a), the secured design in \ref{fig:gomac}(b), where multiple blocks of functions, like `multiply', `addition', `row/column shifters', etc. are placed, and the resultant power traces are shown in Figure \ref{fig:gomac}(c). These blocks perform similar functions as the original block, except for different power signatures. These blocks are chosen during runtime by a selection logic. In the Figure, OP-2 is performed by one functional block in an unsecured design. With security added to the design, the same OP-2 operation would be executed by blocks with different power signatures (although they might belong to the same group of `multipliers' or `adders'). With such an approach, the power trace is secured by generating different power signatures for the same function executed (as shown in green dashed lines), at the same time ensuring that the original purpose of the design remains unaltered. 


% \begin{figure*}[htb!]
%     \centering
%     \includegraphics[width=1\textwidth]{figures/gomac.pdf}
%     % \vspace{-1em}
%     \caption{(a)Conventional cryptosystem where the attacker can deduce secret information from the observed power traces that correspond to the operations;(b) Cryptosystem protected by \shield\ where the power trace does leak information but it leads to wrong information deduction by the attacker as standby modules aka approximate-modules add misleading information by leaking power traces, similar to other modules in magnitude, that are not known previously to the attacker; (c) Power signatures of the outputs of a conventional unprotected cryptosystem and a system protected by the proposed \shield. *The figure is shown for visualization purposes and should not be used as an accurate depiction of an AES cryptosystem's internal structure*}
%      \label{fig:gomac}
% % \vspace{-1.2em}
% \end{figure*}

% \subsection{Getting into the Attacker's Shoes}
% We also anticipate researching Neural Network-based attacks, which are currently being researched within the hardware community. Building attacks would help us evaluate our defense measures and, if need be, come up with even better defense strategies. Current traditional attacks require an attacker to obtain thousands to millions of traces to reverse engineer the key through neural networks. However, given the defenses in place, it is not feasible to obtain that many traces or the defense can change the key, making the obtained traces futile for reverse engineering. As such, we would like to take the help of one-shot learning \cite{Zotkin_shot'18, Thaler_shot'18, Batina_neural_shot'18}
% which require very few traces to learn the distribution and reverse engineer the key. 

\section{Conclusion} \label{sec:conclusion}
Utilizing traditional randomization is not the best solution -given the overhead, performance, and design requiring significant hardware modifications. As a panacea, we discussed our proposed \shield\ that would offer security with significantly less overhead. Our \shield\ incurs less overhead (2$\times$). With the positive results achieved so far, we would like to extend this work further in the hardware domain, thus enabling cognitive randomization based defense for FPGAs, which would secure them from side-channel attacks. Furthermore, working on approximate modules for AES, adversarial learning, and one-shot learning with neural networks, we want to contribute to the community by building attacks that would help us evaluate our defenses more accurately. 


